No Time for Downtime: Understanding Post-Attack Behaviors by Customers of Managed DNS Providers

We leverage large-scale DNS measurement data on authoritative name servers to study the reactions of domain owners affected by the 2016 DDoS attack on Dyn. We use industry sources of information about domain names to study the influence of factors such as industry sector and website popularity on the willingness of domain managers to invest in high availability of online services. Specifically, we correlate business characteristics of domain owners with their resilience strategies in the wake of DoS attacks affecting their domains. Our analysis revealed correlations between two properties of domains -- industry sector and popularity -- and post-attack strategies. Specifically, owners of more popular domains were more likely to re-act to increase the diversity of their authoritative DNS service for their domains. Similarly, domains in certain industry sectors were more likely to seek out such diversity in their DNS service. For example, domains categorized as General News were nearly 6 times more likely to re-act than domains categorized as Internet Services. Our results can inform managed DNS and other network service providers regarding the potential impact of downtime on their customer portfolio.

==> WTMC2022 - No Time for Downtime/section/conclusion.tex <==
\section{Conclusion and Implications}
\label{sec:conclusion}

% Managed DNS has become one important components in Internet ecosystem, following the rapid growth of digital business.
% It provides more reliable service in domain name translation to make sure that an online system is always available for the clients.
% An outage of managed DNS service provider can cause a huge impact on their customers: service unavailability that leads to downtime.
% However, businesses 

% so that the client can communicate with the right machine

% Situation:

Unplanned outages of managed DNS services can lead to financial losses for customers. Depending on how customers value online availability, outages could prompt customers to switch to a different DNS service provider or to add a (secondary) provider to add resilience.
We leveraged large-scale DNS measurement data to infer 168K Dyn customers at the time of the infamous 2016 DDoS attack and tracked the choices made by customers following the attack. We also used a publicly available URL categorization service and website popularity metrics to characterize customers. We demonstrated the impact of factors such as domain popularity, industry sector, risk level, and risk group on the adopted resilience strategy.

% Outages of managed DNS service could cause massive impact on their customers by causing service unavailability, disrupt customers' businesses and leads to losses. 
% However, downtime in online services affects businesses differently, depending on their business type and the importance of the unavailable online resource. 
% % % complication
% % The ability to understand the cost of DNS service unavailability from different business types would be a great advantage for many stakeholders.
% The ability to understand how domain owners will behave in response to an unplanned outage would be a great advantage for many stakeholders, especially in predicting and anticipating business impact of such outage.
% % %Answer
% We  use large-scale  DNS  measurement  data  to  investigate  the  behavior  of  customers of  Dyn after  the  DDoS  attack  in  2016. 
% We enrich the data using a URL categorization service and a website popularity rank to identify domain characteristics: domain popularity, industry sector, risk level, and risk group.

%We identified 168K customers of Dyn prior to the attack and tracked their use of DNS services for 20 days after the attack. 
%We define three possible \textit{domain statuses}: \textit{exclusive} (use only Dyn name servers), \textit{non-exclusive} (use name servers from Dyn and other providers), and \textit{unsubscribed} (stop using Dyn name servers).
%Using \textit{domain statuses} of two consecutive days we define \textit{domain reactions} as \textit{do nothing} (\textbf{R0}), \textit{become non-exclusive} (\textbf{R1}), \textit{unsubscribe then return} (\textbf{R2}), and \textit{unsubscribe then not return} (\textbf{R3}).
%Then, we enrich the data with domain characteristics from Alexa website popularity metrics and McAfee's URL categorization service.

\vspace{0.4em}
\noindent Our findings are as follows:
% 
\begin{itemize}
    % method
    \item 
    % key takeaway 1
    We confirmed the intuition that domains with a higher popularity (i.e., larger user base) are more likely to re-act (40\% of customers on the Alexa Top 100 in contrast to only 15\% in the Top 500K);
    % reference
    %(\S\ref{sec:domain_popularity}).
    \item 
    % method 
    % We use a multivariate logistic regression to model the correlation between industry sectors of Dyn customer domains and the probability to re-act to the outage.
    %Using a multivariate logistic regression,
    % result
    % key takeaway 2 - 3
    We inferred 94 industry sectors for customers and revealed that 34 sectors statistically significantly influenced post-attack customer behavior; 
    %while some other sectors do not, such as \textit{Religion} and \textit{Politics} 
    % reference
    %(\S\ref{sec:stat_analysis}).
    % method
    \item 
    %We further investigate the behavior of domains in 20 out of 34 industry sectors with significant influence on the decision to react (Table~\ref{tab:stat_result}). 
    % result
    % key takeaway 4
    We unveiled that customers in different sectors adopted different resilience strategies. For example, in some sectors customers typically stopped using Dyn altogether whereas in others they added an additional DNS provider to reduce the risk of unavailability;
    %some industry sectors prefer to become non-exclusive, such as \textit{General News} with 13\% became non-exclusive and 2\% unsubscribed.
    %Meanwhile, domains in some other sectors prefer to unsubscribe in response to the outage, such as \textit{Gambling} domains with 1\% became non-exclusive and 10\% unsubscribed
    % reference
    %(\S\ref{sec:stat_analysis}).
    
    % method 
    %\item 
    % By studying domains that returned after they unsubscribed,
    % result
    % key takeaway 5
    %Domains in Gambling sector also show preference to return later after they unsubscribed: only 20\% of unsubscribed domains in this sector that did not return.
    % We see that in some industry sectors, such as \textit{Gambling}, domains that unsubscribed prefer to re-subscribe later, 
    %Meanwhile, a high proportion of domains in some sectors do not return after they unsubscribed, e.g.,\ \textit{Travel} with more than 90\% of unsubscribed domains did not return.
    %These results indicate the dependence of observed post-attack domain reactions on industry sectors. 
    % reference
    %(\S\ref{sec:stat_analysis}).
    % method
    \item  We showed that the popularity of domain names is more tightly related to post-attack behaviors in some industry sectors over others;
    % We study the popularity of domains in each industry sector using the distribution of domain ranks -- where present -- in Alexa Top 1M website list.
    %Analyzing the Alexa ranks of re-active and non-reactive domains in 20 selected industry sectors, 
    % result
    % key takeaway 6
    % \textcolor{red}{
    %we see that the popularity of domains  has more influence on the decisions to re-act after the attack in some industry sectors (e.g.\ \textit{Job Search}) more than others (e.g.\ \textit{Travel}). %@@ what numbers to put?
    % reference
    %(\S\ref{sec:stat_analysis}).
    % }
    % method
    \item 
    % Using reputation score from McAfee grouped into different risk levels,
    %Considering risk level,
    % result
    % key takeaway 7-8
    A large proportion of domains categorized as `minimal risk' that unsubscribed from Dyn, did not return (more than 71\% did not return). We observe that domains categorized as medium or high risk prefer to become non-exclusive after the attack (9\% became non-exclusive while 1\% unsubscribed). %The ones who unsubscribe tend to return if they unsubscribe (none did not return).
    % reference
    %(\S\ref{sec:domain_risk_level}).
    % method
    % \item We investigate the reactions of domains that possess similar main risk
    % result
    % key takeaway 9
    We also see that domains in some risk groups such as \textit{Liability} (e.g., pirated movie portals) showed a slight preference to unsubscribe after the attack,  with 0.1\% becoming non-exclusive and 2\% unsubscribed.
    % \textcolor{red}{
    % In addition, we observe that the popularity might have a strong influence on the post attack reactions of domains in some risk groups, such as \textit{Productivity}\footnote{E.g., sites for entertainment purpose.}, but not in some others, such as domains with \textit{Bandwidth}\footnote{E.g., video streaming sites.} and \textit{Communication}\footnote{E.g., instant messaging platforms.} risks
    % reference
    %(\S\ref{sec:domain_risk_type}).
    % }
\end{itemize}




% The results show differences in behavior across industry sectors and intended uses, in terms of type of reaction, time of reaction, and the return movement after stop using the service.
% 1

% 2
% The result also indicates which sectors that have higher and more effective influences on the decision as summarized in Table~\ref{tab:stat_result}.
% 3
% We further analyze how each aspect of domain characteristics influence the domain behavior using data visualizations.
% On \textit{domain popularity}, we show that the proportion of domains that reacted is higher among highly ranked domains than among those with lower rank.
% 4
% On \textit{domain industry sector}, we show that malicious domains predominantly became non-exclusive following the incident, and all of those which unsubscribed later decided to return.
% 5
% This behavior is rather similar in \textit{General News} sector, but most of unsubscribed domains in this sector did not return.
% 6
% In addition, domains for adult audience show a significant behavior towards the decision to unsubscribe after the incident.
% 7
% We also show that domain popularity might or might not have a strong influence on behavior of domains in each sector, depends on how uniform their ranks are.
% 8
% On \textit{domain risk level}, we show that the proportion of domains with higher risk that became non-exclusive is much higher while all of them which unsubscribed later returned.
% 9
% Meanwhile, domains with minimal risk, which represent the majority of legitimate domains, have a relatively high tendency not to return once they unsubscribe.
% 10
% Lastly, on \textit{domain risk group}, we show that the behavior of domains in certain risk groups might be strongly influenced by their popularity.

The results of our study could help managed DNS providers to estimate the impact of an unplanned outage based on their customer portfolio. Businesses such as cloud service providers could make use of a methodology similar to ours to understand the impact of unplanned downtime on their customer portfolio~\cite{Yasir2021}. 

%\subsection{Implications of results for Stakeholders}
%\label{sec: Implications}
%We present possible implications of the results for different stakeholders, especially in managed DNS business.
% 
%\subsubsection{For Managed DNS Service Providers}
%\textcolor{red}{This should be a separate section and part of Discussion. Implications are very generic, we need examples from results for making them stronger.}

\comment{

We evaluate the impact of factors such as domain popularity, industry sectors, domain risk level and risk group on decision of domain managers in response to unavailability of Dyn services. We believe that our results can be insightful for both providers and users of network services. We discuss the implications of these results for four a number of stakeholders:

\noindent \textbf{Managed DNS Service Providers:}
The results of this work are most useful for managed DNS service providers, especially to develop resilient strategy related with their customer portfolios. 
\begin{itemize}
    \item 
        DNS providers could use this work to estimate the proportion of their existing customers which are more likely to stop using the service in case of an outage incident. 
        For example, they can start profiling their existing customers using URL categorization service and Alexa rank to indicate which of them have characteristics (e.g., industry sector and popularity) that suggest a higher probability to leave in case of an outage.
    \item
        Using data of their existing revenue, DNS providers can quantify financially the potential business impact of an unforeseen outage by calculating the potential revenue loss coming from the number of customers with higher probability to leave in case of an outage.
    \item 
        DNS providers could use this estimation of potential business impact to justify their strategy in outage prevention e.g., infrastructure redundancy, or to minimize the loss, e.g., use cyber insurance. 
    \item
        Moreover, using this method, DNS providers should consider to monitor their customer portfolio in order to minimize the proportion of customers with characteristics (e.g., domain popularity and industry sector) that reflect a high probability to re-act or leave in case of an outage to minimize the business impact.
    \item
        Further, DNS providers could base their marketing strategy on the results of this work, for example, to offer more premium DNS services, e.g., with more redundant PoP servers, to customers that are more probably to re-act since it indicates that the customers adopt a more resilient strategy.
        
\end{itemize}
% They could develop a formula to measure their current risk score based on the number and the industry sectors of their current customers. 
% \textit{Second}, 
% \textit{Third}, they 
% 
%\subsubsection{For Digital Businesses}

\noindent \textbf{Digital Businesses:\ }
\textcolor{red}{}
The results could be beneficial for businesses in terms of managing their risk of downtime.
\begin{itemize}
    \item 
        They could adjust their investment to prevent or to deal with downtime, e.g., insurance, SLA, or use of backup provider, by estimating the relative cost of downtime based on their characteristics.
    \item
        They could adjust their contingency plan in case of downtime, e.g., what reaction they could take based on most domains in similar sectors. However, it needs further study to evaluate the quality or the impact of different decisions taken by the Dyn customers, i.e., whether their reactions were appropriate.
\end{itemize}


%\subsubsection{}
\noindent \textbf{Cyber Insurance:\ }
The results can assist in cyber risk calculation for insurance purpose. 
\begin{itemize}
    \item 
        Insurers can use these results to find the optimum price and compensation, according to business characteristics of their (potential) customers and estimated business impact of downtime.
        For example, cyber insurers could estimate a higher business impact of downtime on customers with characteristics that suggest a higher likelihood to react.
    \item
        With this estimation, cyber insurers can adjust their strategy to offer more competitive pricing and compensation scheme, e.g., higher premiums for customers with high likelihood to react.
\end{itemize}

%\textcolor{red}{Example! DONE}

%\subsubsection{}
\noindent \textbf{Academic Researchers:\ }
The methodology and results presented in this paper have shown a novel direction for Internet measurement research to explore the Internet ecosystem resilience properties and dynamics. Rapid growth of digital business and use of Internet as business enabler requires more attention from the academic measurement community. 
\begin{itemize}
    \item 
        Our methodology provides business context on large-scale Internet network measurements. This approach can initiate ground breaking insights for academic research in both business and technical fields, such as digital business ecosystem, cyber risk, and centralization topic.
    \item
        Our methodology translates observations from measurement data into business insight which might accelerate strategic decision making related with digital resilience such as cyber security investment.
    \item
        The results from this work could help researchers analyze industry sectors regarding their concern about DNS service availability, and behavior against downtime in general, based on our statistical model.
        
\end{itemize}
}

% OLD VERSION ABOVE
% [UNDER RECONSTRUCTION]

% Structure:
% \begin{itemize}
%     \item Profiling managed DNS customers (who should practice? what aspect to consider?)
%     \item Implication of results from risk characteristics analysis
% \end{itemize}

% We now discuss the implication of our results in the previous sections.

% \textbf{Managed DNS customer profiling.}
% By observing the change in the \texttt{NS} records following a DoS-induced outage, we showed that customers of managed DNS service adopt different resilience strategy.
% Some customers responded to the attack by using additional providers for redundancy in name servers; some domains unsubscribed and switched to other providers; while some others did not show any re-action.
% From the perspective of the DNS service provider, each of these responses indicate a different business impact, e.g., the provider may suffer financial losses from customers that stopped using the service for a longer period, which could be catastrophic if the majority of customers show such response.

%DNS service providers could profile their current customers as a means to understand the resilient strategy adopted and further, to estimate the business impact of an unforeseen outage in the future. 

We show that \textit{domain popularity}, \textit{industry sector}, and -- to some extent -- \textit{risk groups} \& \textit{risk level}, are factors that can be used to understand the choice of resilience strategy. %These results can be used to estimate the proportion of customers that may leave the service in case of an unforeseen outage.
%DNS service providers can: 
%\begin{enumerate}
%    \item make use of publicly available website popularity metrics such as Alexa~\cite{noauthor_alexa_nodate} or Tranco\footnote{\url{https://tranco-list.eu/}}~\cite{le_pochat_tranco_2019} to indicate the popularity of domains operated by their customers;
 %   \item use URL categorization services 
    % from companies such as McAfee\footnote{\url{https://trustedsource.org/}}, FortiGuard\footnote{\url{https://www.fortiguard.com/webfilter}}, and Zvelo\footnote{\url{https://tools.zvelo.com/}}, 
  %  to obtain the industry sectors of the domains;
   % \item use our results especially in Fig.\ref{fig:by_popularity}, Table~\ref{tab:stat_result}, and Fig.\ref{fig:reactions_by_category} to estimate which customers that adopt a more resilient strategy, hence, more likely to re-act in case of an unforeseen outage.
%\end{enumerate}
% 
%\noindent The objective is to monitor and maintain the proportion of customers with a higher chance to re-act, especially those which prefer to stop using the service following an unplanned outage.
%That is because our results show that managed DNS customers are less likely to return if they stop using the service (Fig.\ref{fig:reaction_by_risk_type}).
%DNS service providers should avoid having large proportion of customers with such potential response to prevent financial loss in case of unplanned outages in the future.


\comment{
\textbf{Resilience strategy of cyber criminals.}
Our results indicate that domains potentially used by cyber criminals seem to adopt a more resilient strategy.
We observe some of Dyn customers were domains with malicious intent -- indicated by their industry sector labels (PUPs or Malicious Sites) and reputation scores (medium or high risk) from McAfee's URL categorization service --
implying their needs to improve reliability and performance for their operations.
The majority of these malicious domains even chose to use additional providers for redundancy in response to the outage (Fig.\ref{fig:reactions_by_category} and Fig.\ref{fig:reaction_by_risk_type}).

We suggest law enforcement to collaborate with DNS service providers to 

TBA \dots
}


\subsection{Limitations and future research}
%Based on the limitation of this research, we call for a further study regarding non-reactive domains. 
% As a result of our analysis we observe that interestingly the number of \textit{active domains}, especially \textit{exclusive domains}, that did not react following the incident are relatively high. It means that a large number of domains must have experienced downtime, since they did not have backup DNS service, but they did not do anything in response to that. Among them are domains that belong to \textit{large online companies} that provide rather critical services e.g., VoIP, ISP, and social network. One possible explanation is that the DNS service was already back in less than a day following the outage, and these companies have had a good relationship with Dyn for years. Hence, they tolerated this one time relatively short outage. In addition, it can be  that because the incident was due to a cyber attack instead of Dyn's own technical mistake, they blamed the attacker and not Dyn. We think that further research is required to explore why a large number of exclusive domains did not take action in response to this incident. 
The nature of our data sources and assumptions that we need to make lead to a few limitations.
% 1
\textit{First}, the URL categorization service we use in this study might exclude domains without hosted content.
Recall that the domain content is a feature in our categorization process. 
Moreover, one should be aware that all existing URL categorization services, including McAfee's, have accuracy concerns~\cite{vallina_mis-shapes_2020}.
\comment{TBD To account for this, we randomly sample 100 domain names labeled by McAfee to manually verify the given labels and yield that XX\% of them are correctly classified.}
% 2
\textit{Second}, Alexa does not rank non-website domains (i.e., other networked services), despite their high traffic. Moreover, Alexa ranks the Top 1 million most popular websites only. Consequentially, most Dyn customers that we infer ($\sim$163K out of $\sim$168K) do not have an associated rank.
In addition, Alexa Top 1M is prone to bias and a rigorous alternative exists, i.e., Tranco\cite{le_pochat_tranco_2019}. However, Tranco did not yet exist when the attack happened in 2016.
% 3
\textit{Last}, the insights we draw are based on the analysis of data connected to a single attack event. Hence, we understand that similar behavior may not be observed for another event. However, researchers could apply our methodology to other similar attacks and outages to improve the generalizability of our findings.  
%
% In some cases, multiple domains can be operated by a single party. For example, an enterprise such as Alphabet Inc. can operate multiple domains such as google.com and gmail.com.\ Currently, we do not view the impact that the concentration of domains among the parties that operate them has on our results. However, to further explore if there are multiple parties responsible for the reactions we observe, we measure the variety of reactions observed within each AS. 
% % \textcolor{red}{
% To do so, we extract the type of hosting that a domain was using during the incident by mapping IP address from domain's \texttt{A} record to its corresponding Autonomous System (AS) using IP prefix to AS dataset~\cite{the_caida_ucsd_routeviews_2008}
% % } 
% Using this data we calculate the percentage of IPs that react out of the total number of IPs related to the domains using Dyn name servers. Fig.~\ref{fig:AS_Size_Histogram} shows the distribution for the percentage of \texttt{IP} addresses within each AS that react. We observe that in the case of only the smaller ASes, all domains show the same behaviour. For, larger ASes, we see only a small fraction of domains showing reactions. This shows that the resilience strategy chosen by domains within each AS was not the same, except when these ASes were relatively small.
%
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figure/AS-and-Rank-histogram.pdf}
%     \caption{Histogram showing the variability in decisions within each AS and the average size (number of IPs) of ASes.}
%     \label{fig:AS_Size_Histogram}
% \end{figure}
%

As one area of future work, we plan to analyze the response following outages (attack related or otherwise) in other online services such as CDN or web hosting using a similar approach.
Even though these outages would also lead to downtime, the behavior observed may be different given that the operator/manager might need to employ greater effort to opt for a more resilient strategy. 
In addition, considering the development of the DNS ecosystem since 2016, we plan to analyze more recent incidents to gain updated insight into the topic and study what changed in the last six years.
%We also call for further research using other aspects of domain characteristic to explore other factors that might influence the post-outage decision.
% Our approach would also be useful in explaining the landscape of digital businesses using large scale measurement to expand our understanding from either business, technical, or security perspective.
% @@ What do you mean here?

%Moreover, we also call for further analysis on unreachable domains to understand the situation. Historical data, e.g., web archives, can be used to discover the characteristics of these domains.



==> WTMC2022 - No Time for Downtime/section/introduction-merged.tex <==
\section{Introduction}

The domain name system (DNS) is a core component of the Internet. Its primary function is to translate human-readable domain names to IP addresses. As such, e-commerce with a web site is no longer possible if the authoritative name servers for the web site's domain name fail to function. A managed DNS service provider offers premium services to manage DNS traffic~\cite{abhishta_measuring_2019}, improving reliability and performance, including potentially offering DDoS protection. 
%Domain name owners can delegate authority to such managed DNS services, which, among others, can provide greater resilience against denial-of-service (DoS) attacks. 
Failures of managed DNS services adversely affect parties that rely on these services~\cite{bolstridge2016dyn}, depending on their degree of reliance.

%The effects are not necessarily always earth-shattering: businesses will view unavailability based on its operational consequences.

Businesses that use a managed DNS service may adopt a more resilient strategy, i.e., use multiple DNS service providers, that ensures higher availability even when that managed DNS service provider may be unavailable. Previous studies  \cite{abhishta_measuring_2019,bates2018evidence} have shown that when services of Dyn, a large managed DNS service provider, became unavailable in 2016 \cite{bolstridge2016dyn}, many but not most domains adopted this more resilient strategy to counter the effects of downtime. 
Some businesses value continuous online availability enough to pay the premium charged by managed DNS service providers. It depends on the expected return on investment of such high availability of their online services. Different businesses value high  availability differently, but outages clearly sometimes directly induce a loss of revenue~\cite{akamai2018}.

%We study the influence of factors such as industry sector and website popularity on this willingness of domain managers to invest in high availability of online services.

%The technological impact of DNS unavailability in terms of interruption of %services to Internet users and consequences of centralization in this market is %discussed in the literature at great lengths. 
%We summarize these findings in Section~\ref{sec:related_work}. 
% this should be in related work
%A study using survey-based methodology to understand the perception of unplanned unavailability of network services to its customers report that the largest loss is due to the unavailability of customer facing services~\cite{akamai2018}. 
% this isn't really cybercrime, at least not the kind
% discussed in this survey, right?
% not convinced this cite is relevant
% \cite{florencio2013sex} argue that most cybercrime surveys provide limited insights as they use restricted sample size and selection criteria. In this paper, using an empirical methodology, we evaluate the influence of factors such as industry sector and website popularity on the decision of Dyn customers to follow the previously discussed more resilient strategy.

We perform an analysis of large-scale longitudinal active DNS measurement data to identify domains that responded to the Dyn DDoS-induced outage. We map these domains to their popularity rank using historical Alexa rankings. We also obtain industry-sourced data on industry sector and risk characteristics using McAfee's URL categorization service. 
\noindent Overall, we make the following contributions:
\begin{itemize}
    % methodology
    % \item 
    % We present a novel methodology @@what is novel methodology -- must 
    % summarize here. not convince the method is novel. just correlating
    % data sets.  if it is novel, must be specific about how.
    
    % a number @@say what number of 
    \item We characterize 106K domains under \texttt{.com}, \texttt{.net}, and \texttt{.org} affected by the Dyn outage based on four aspects: post-attack resilience strategy, popularity, industry sector, and risk characteristics.
    
    \item 
    We observe that domains with higher popularity (based on their Alexa ranks), more commonly adopted a more resilient strategy. We find that nearly 40\% of Dyn customers in the top 100 of Alexa 1M list re-acted after the attack while in the top 500K only $\approx$15\% re-acted.
    
    \item 
    Some industry sectors had a more significant correlation with post-attack response of domain managers. For example, the probability of a domain owner to adopt a more resilient strategy after the attack was nearly 9 times more if the domain belonged to \textit{General News} category (compared to categories which did not re-act). Some industry sectors (such as \textit{Religion}) did not have a statistically significant impact on the decision of domain owners.
    %Particularly, among Dyn customers serving general news, 13\% of them used additional DNS service providers after the attack, while despite the similar number of domains, the proportion is only 3\% among Dyn customers which provide job search.
    %@@need to say what the influence was.  was it in both directions? this sentence is awkward. 

    \item 
    We show differences in the post-attack responses across domains categorized by their risk characteristics, based on McAfee's URL categorization service. Nearly, 9\% of the domains categorized as malicious used an additional DNS service provider after the attack, while only 1\% of domains categorized as low risk took this strategy.
\end{itemize}

\noindent Our results empirically show that factors such as industry sector and popularity of domain name influence the resilience strategy adopted by domain managers in the face of unplanned unavailability of managed DNS services.
We believe that our results will be useful for managed DNS providers in understanding the possible aftermath of unforeseen downtime. 
% Other related stakeholders, such as insurance service providers, who are interested in measuring the cost of unplanned network downtime may use our results to understand network downtime implications for various industry sectors. @@feel this is assertion w/o substantiation

We first review related work (\S\ref{sec:related_work}), and then
present our data sets and analysis  methods (\S\ref{sec:methodology}), 
results (\S\ref{sec:Result_and_Discussion}), and discuss 
our conclusions and implications (\S\ref{sec:conclusion}). 

We use mostly open source data-sets: Alexa top 1M historical archives from TU M{\"u}nchen\footnote{\url{https://toplists.net.in.tum.de/archive/alexa/}} 
and URL categorization portal from McAfee~\cite{noauthor_mcafee_trustedsource}.
OpenINTEL data are available to academic researchers upon request~\cite{OpenINTEL-JSAC2016}. We use \texttt{statsmodels} package~\cite{seabold2010statsmodels} in python to implement logistic regression.
% @@something about
% availability of tools and data

==> WTMC2022 - No Time for Downtime/section/introduction.tex <==
\section{Introduction}

% Elaborate problem statements and previous works

% Situation

% REMOVED DUE TO REVIEW
% Rapid development in cloud technology has led to a move from on-premise solution to outsourced services \cite{hsu2014examining}. 
% With the increase in the number of businesses that consume and provide services through Internet, quality of service stands out as one of the competitive advantages in this emerging market \cite{alkhater2018empirical}. 
% Service quality determines and influences selection of cloud service providers. 
% Service outage frequency is a key factor that can diminish the quality of service by making online resources unavailable for businesses and their consumers for a period of time. 
% Downtime in service availability causes disruption in business and leads to a loss \cite{abhishta2019blind}. 
% However, the financial loss experienced by businesses due to unavailability of online resources may depend on their business type. 
% Each industry sector has its own cost of downtime, according to the nature of the business and the importance of the unavailable service. 
% For some business types, every second of Internet unavailability may cost millions of dollars, while for others, the cost can be negligible \cite{florencio2013sex}.

% Complication
Cloud-based infrastructure as a service (IaaS) providers offer premium services (e.g., managed DNS and Content Delivery Network (CDN)) that promise high availability and performance of customer services~\cite{mell_nist_2011}.
Businesses purchase these services to hedge the risk of accumulating losses from network downtime. Unplanned outages of these cloud providers might significantly disrupt businesses that depend on their infrastructure/services~\cite{dubendorfer_economic_2004}. For some business types, every second of Internet unavailability may cost millions of dollars, while for others, the cost can be negligible \cite{florencio2013sex}. 

Businesses that use a managed DNS service often have the opportunity to adopt a more resilient strategy (i.e.,\ use multiple DNS service providers) that ensures higher availability even when that managed DNS service provider may be unavailable. Previous studies \cite{abhishta_measuring_2019,bates2018evidence} have shown that when services of Dyn, a large managed DNS service provider, became unavailable in 2016 \cite{bolstridge2016dyn}, a considerable number of domains adopted this more resilient strategy to counter the effects of downtime. The same studies have also shown that the domains that adopted the more resilient strategy were not in majority. Different businesses value high  availability differently, but it clearly sometimes directly induces loss of revenue~\cite{akamai2018}.

@@make roadmap of paper.
Section\ref{sec:related_work} reviews related work.
Section~\ref{sec:mdns_business} discusses the relationship between various industry sectors and importance of Internet availability to them.

%The technological impact of DNS unavailability and consequences of centralization in this market has been discussed in the literature at great lengths. We summarize these findings in Section~\ref{sec:related_work}. A study using survey-based methodology to understand the perception of unplanned unavailability of network services to its customers report that the largest loss is due to the unavailability of customer facing services~\cite{akamai2018}. \cite{florencio2013sex} have argued that most cybercrime surveys provide limited insights as they use restricted sample size and selection criteria. In this paper, using an empirical methodology, we evaluate the influence of factors such as industry sector and website popularity on the decision of Dyn customers to follow the previously discussed more resilient strategy.


% \textcolor{red}{something on the real life implication of this outage. Why should we still care? Maybe, a short comparison with recent outages and their impact on network availability world wide.} 

%Our aim is to be able to predict how cloud service consumers, such as managed DNS consumers, would react upon an outage incident, so that different stakeholders can anticipate the business impact of such events. 

% Answer
We perform an analysis of large-scale longitudinal active DNS measurement data to identify domains that responded to the outage. We then map these domains to their popularity rank (using historical Alexa ranks), industry sector and risk characteristics such as level of maliciousness \& risk type (using McAfee URL categorization service). We discuss the datasets used for this analysis and their characterstics in Section~\ref{sec:methodology}. Further in Section~\ref{sec:Result_and_Discussion}, we analyze this mapped data to understand the influence of various factors such as industry sector and website popularity on the decision of Dyn customers to use of more resilient DNS strategy.

% Conclusion
% 
% Brief about conclusion here, needs update...
% 
% \textcolor{red}{ 
% [Still Working][CONTRIBUTION] We show that all following aspects do influence post-outage decisions of customers of Dyn:
% \begin{itemize}
%     \item \textit{Popularity} of the domain names
%     \item \textit{Industry sector} of the domain names
%     \item \textit{Risk level} of the domain names
%     \item \textit{Risk type} of the domain names
% \end{itemize}
% }

% \textcolor{red}{AVOID USING TERMS THAT NEED FORMAL DEFINITIONS!}
\ 

Overall, we make the following contributions:
\begin{itemize}
    % methodology
    \item 
    We present a novel methodology to analyze longitudinal Internet measurement data.
    % to estimate business impact of cyber attacks on DNS providers based on customer portfolio.
    We characterize domains affected by the Dyn outage based on a number of aspects, including responses after the outage, popularity, industry sectors, and risk characteristics.
    % domain popularity influence on reaction
    \item 
    % \textit{We demonstrate in Section~\ref{sec:domain_popularity} how popularity of domains correlate with the reactions after the attack and} 
    We observe that domains with higher popularity, indicated by Alexa rank, have a higher chance to adopt a more resilient strategy.
    % Later in Section~\ref{sec:stat_analysis}, \ref{sec:domain_risk_level}, and \ref{sec:domain_risk_type}, 
    % We show how to identify whether the popularity plays an important role on the reactions.
    % quantitative measure of industry sector influence
    \item 
    % We statistically model the correlation between domain industry sectors and the probability of reacting to outage in Section~\ref{sec:stat_analysis}. 
    We observe that some industry sectors have a higher and significant influence on the post-attack response of the domain managers, while some others do not.
    % risk and reaction
    \item 
    % We discuss the correlation between risk characteristics of domains and the reactions after the attack.
    We show different post-attack responses across domains with different levels of maliciousness and risk types, according to McAfee URL categorization service.
    % using data to validate prior known premise about value of availability for businesses
    \item 
    Our results confirm the notion about availability that certain aspects, such as industry sector and popularity of domain names,
    % indicate a higher concern about availability among managed DNS customers thus 
    influence the resilience strategy adopted by the domain managers.
    % \item \textit{We propose an approach to evaluate possible business impact of cyber risk on Cloud providers \textbf{based on their customer portfolio} which existing frameworks do not take into account~\cite{akinrolabu_csccra_2019,akinrolabu_cyber_2019}}. PUT THE CITATIONS IN THE FIRST POINT.
\end{itemize}

We believe that our results can be useful, not only for manage DNS industry to understand the possible aftermath of unforeseen downtime, but also for other stakeholders, such as insurance service providers, who are interested in measuring the cost of unplanned network downtime. We discuss this topic in Section~\ref{sec: Implications}.
% 
% i.e., popularity, industry sector, risk level, and risk type of domains, do have an influence on post-outage decision. They influence, in different ways, the decision
% (1) \textit{to react or not}, 
% (2) \textit{to become non-exclusive or unsubscribe}, and 
% (3) \textit{to return or not}. 
% \\
% Include contribution here and summarize conclusion.
% }

  

%how different domain owners/managers take decisions following a major downtime incident forced by a large denial of service attack. 
%We use large-scale DNS measurement data to investigate the change in behaviour of customers (categorised by domain characteristics) of Dyn after the DDoS attack in 2016. 
%We classified all active domains that used Dyn managed DNS service prior to the incident into different domain statuses after the incident: those who keep using and those who stop using the service. 
%We further consider the status change in these domains as reactions of the domain owners in response to the incident.

%\begin{description}
   % \item[The attack] The day, Oct. 21, 2016 (\textit{day 0}), in which Dyn suffered an outage of its managed DNS service from a DDoS attack.
    %\item[Dyn customers] Domains under \texttt{.com}, \texttt{.net}, and \texttt{.org} that used at least one of Dyn name servers (\texttt{*.dynect.*}) \textit{one day before} the attack i.e., Oct. 20, 2016 (\textit{day -1}).
    %\item[Domain status] The relationship between a Dyn customer and Dyn on a certain day in terms of use of Dyn name servers.
  %  \item[Exclusive domain] Domain status that indicates the use of \textit{only} name servers from Dyn.
  %  \item[Non-exclusive domain] Domain status that indicates the use of name servers from Dyn \textit{and at least one} name server \textit{other} than Dyn name servers.
    %\item[Unsubscribed domain] Domain status that indicates the use of \textit{only} name servers \textit{other} than Dyn name servers.
    %\item[Domain movement] Changes in domain status between adjacent days.
    %\item[Observation period] A period of 20 consecutive days after the attack, from Oct. 22, 2016 (\textit{day +1}), to Nov. 10, 2016 (\textit{day +20}), in which the daily domain status of Dyn customers were observed.
    %\item[Do nothing] Domain response following the attack in which no single change in domain status is observed within the observation period.
   % \item[Non-reactive domain] Dyn customers which \textit{did nothing} in response to the attack.
%    \item[Reactive domain] Dyn customers whose domain status changed at least once within the observation period in response to the attack.
 %   \item[Become non-exclusive] Domain response following the attack by changing its domain status from exclusive to non-exclusive, i.e., use redundant services.
  %  \item[Unsubscribe] Domain response following the attack by changing its domain status from exclusive or non-exclusive to unsubscribed, i.e., stop using Dyn DNS service.
%\end{description}


%To understand more about factors influencing domain owners, we study the characteristics of these domains from different aspects.
%We use ranks from Alexa Top 1M list to measure domain popularity and
%a URL categorization service to classify these domains into different industry sectors, risk types, and risk levels.
% In addition, we enriched the data with information about the type of hosting which the domains used from their AS number.

%We employ two main research questions to guide this study. 
%\begin{itemize}
%    \item \textit{How does each domain characteristic influence the decision made by %    \item \textit{How do owners of domains in the same category behave?}
%\end{itemize}
% Methodology
% We use two types of analysis to answer these questions.
% \textit{First}, we conduct statistical analysis to study how significantly important industry sector of the domains are in making a decision towards a decision to react.
% \textit{Second}, we conduct graphical analysis using plots and diagrams to study the behavior of domains in the same category.



% \textcolor{red}{
% CONCLUSION.
% We show the difference in behavior across industry sectors using three perspectives. 
% \textit{First}, what type of reaction i.e., whether a domain chose to keep using Dyn but became non-exclusive, or to stop using Dyn service. 
% \textit{Second}, how delayed was the reaction i.e., whether a domain reacted immediately after the incident or later.
% \textit{Third}, returning movement i.e., whether a domain returned after it stopped using Dyn or left for good.
% We observe differences in the behaviour among industry sectors and intended uses. 
% Specifically, most domains in Finance sector showed a distinct behavior that suggests sensitivity to reliability of the DNS provider, as they permanently stopped using the services a few days after the incident.
% In addition, using the Wilcoxon signed-rank test we check whether the differences we observed are statistically significant.
% }
% 
% 
% 


==> WTMC2022 - No Time for Downtime/section/mdns_business.tex <==
\section{Business of Managed DNS Service and Importance of Internet Availability for different Industry Sectors}
\label{sec:mdns_business}
% 
% DNS is one key component of Internet ecosystem.
% Its main role is to translate the domain name to its corresponding IP address. 
% The use of domain name is beneficial for multiple reasons, including ease of use and stable connectivity.
% Nowadays, almost all Internet-based services use domain name extensively and rely on it.

The domain name system (DNS) is a core component of the Internet. Its primary function is to translate human-readable domain names to IP addresses. Domain-destined communication (e.g., business website visits) may no longer be possible if the authoritative name servers for a domain name fail to function. 


A managed DNS service provider offers premium services to manage DNS traffic, especially for businesses which rely on it~\cite{abhishta_measuring_2019}. It offers better reliability and performance with better computing and network infrastructures, and may offer a DDoS protection. Domain name owners can delegate authority to managed DNS services, which, among others, can provide greater resilience against denial-of-service (DoS) attacks. If managed DNS services themselves however fall over, this can have adverse effects on many of the depending parties. The effects are not necessarily always earth-shattering: businesses will view unavailability based on its operational consequences.

%DNS resolves the domain name requested by the client through a DNS resolver into an IP address. 
%The resolver will locate the authoritative name server (ANS) for the domain name and query the ANS for the IP address of the domain name. 
%Once obtained, the IP address will be returned to the client, so the client can contact the corresponding machine using the IP address. 
% DNS makes use of caching mechanism in which a record is stored for a certain Time to Live (TTL) before it gets refreshed by a new record.


% Hence, their customers can expect higher availability for their online resource by using managed DNS service.


%\subsection{}
% 
% Explain why different business value and require availability differently and how managed DNS can be an important service
% 
% Reference: \cite{barua_empirical_2004}
% 
% Main idea: Availability as digital business capability and value \\
% 
% Main idea: Managed DNS offers premium service for higher availability \\
% 
% Historically businesses have been viewed either as brick \& mortar or as online or as a combination of the prior two based on the mode of delivery of service. 
Today, even most ``brick \& mortar" businesses have an online presence, either for e-commerce, marketing, or communication~\cite{pozzi2013effect}.
%The backbone services of the Internet such as the domain name system play a crucial role in making the digital business of firms available. 
% As discussed before managed DNS service providers offer additional resilience to availability as they are able to leverage their infrastructure to defend against attacks such as denial of service.
% Of-course, this resilience comes at an additional cost, hence, most 
Managed DNS providers charge a premium for using them as authoritative name servers. 
% As dependence of Industry varies per Industry sector, 
But, it is not profitable for all business types to bear this additional cost. It depends on the return on investment that is expected by the business by guaranteeing high up-times of their online services. To understand the influence of factors such as business sectors and website popularity on the willingness to spend additional cost to guarantee high availability of online services, we perform an analysis of Dyn customers (domains that use its services) that followed a resilience strategy of either using an additional DNS provider or switch to another provider after the attack. We empirically draw differences between the industry sectors that followed the above mentioned strategy and the one's that did not. Thus, giving us a peek into the the cost of unintended downtime anticipated by customers of Dyn.

%We hypothesise that industry sectors who value availability more are more likely to change their status. We observe the decisions taken by different industry sectors and empirically test the relationship between the type of business and the decision to change status.

%Importance of Internet for different firms.

%Dependence of industry sector on ICT.
% how mDNS affects it

% MIS Quarterly paper about An Empirical Investigation of Net-Enabled Business Value

% Digital Business Capability



==> WTMC2022 - No Time for Downtime/section/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Earlier work has shown that even large-scale DNS deployments, such as the root zone of the DNS, can be a victim of DDoS attacks. Moura et al.\ provided a detailed analysis of such an attack on the root in 2015, which not only affected operations of one root server family, but led to collateral damage to other DNS operators~\cite{MouraIMC2016}.

Allman~\cite{allman_comments_2018} reflected on the structural robustness of the DNS, and provided recommendations to improve operator practices, including a call to action to implement topological and geographical diversity in terms of authoritative name server deployment. Moura et al.\ studied how DNS caching and retry behavior by resolvers may hide up to 90\% of DDoS attacks on the DNS from the perspective of Internet users, but also noted that this resolver behavior may impose a significant additional load on servers under attack~\cite{MouraIMC2018}.

% Centralization of DNS services and resolution is increasing -- up to 30\% of queries to two ccTLDs originated from just five cloud providers in 2020~\cite{MouraIMC2020}.


 %Other infrastructures also show a similar trend, such as the e-mail ecosystem where mail is increasingly handled by a small number of large cloud operators~\cite{OpenINTEL-JSAC2016,HenzeTMA2017}.
% Other cloud infra: mail
% 
% RvRD: cut until here.


Centralization of DNS services and resolution is increasing -- up to 30\% of queries to two ccTLDs originated from just five cloud providers in 2020~\cite{MouraIMC2020}. Such
centralization enables economies of scale in
provisioning infrastructure, but can also
present a single point of failure~\cite{bates2018evidence}.

%On the one hand, centralization in these services may provide greater revenues to some organizations to be invested in future innovations; on the other hand, events causing unavailability can affect a large number of businesses. Bates et al.\ discuss the problems associated with market centralization in the case of DNS service providers and the change in market share as a result of the attack on Dyn ~\cite{bates2018evidence}.  @@need to say more about what Bates found if you include this .

%@@you have to say what that study found.



The technical and business implications of the attack on Dyn were discussed extensively\cite{antonakakis2017understanding,bates2018evidence}. Antonakakis et al.\ analyzed the emergence of Mirai, the botnet used for attacking Dyn, while also presenting the possibility that the attackers were targeting not only Dyn but also Sony Playstation infrastructure \cite{antonakakis2017understanding}. Bates et al.\ analyzed the market share of Dyn within the top 1000 Alexa rank domains (that belonged to \texttt{.com}/\texttt{.net}/\texttt{.org} TLDs) and found that its market share dropped from 10\% before the attack to 7.5\% within the month after the attack \cite{bates2018evidence}. 

In this paper, we extend on previous work in which we analyzed 
% Most closely related work by Abhishta et al.\ analyzed 
the immediate impact of the attack on Dyn, and an earlier attack on another managed DNS provider, NS1~\cite{abhishta_measuring_2019}. In the previous paper, we showed that in terms of risk management, using multiple DNS providers is a good strategy. In this paper, we extend and analyze factors that potentially drove the decision-making of Dyn customers and characterize the behavior of different types of customers when faced with the consequences of such a large-scale attack.

%@@are you sure prefix papers didn't do that? you need a sentence for each of those papers and what they found.. not just what they studied but what they discovered.. 

%Moura et al.\ evaluated the impact of mechanisms within DNS protocol help during DDoS attacks and found that DNS mechanisms of caching and retries provide significant resilience to the user during an attack \cite{MouraIMC2018}.

%too repeated from earlier
%In this paper, we analyze large-scale Internet measurement data by mapping it to data on website popularity and a URL categorization service to understand the decisions made by domain managers to counter the implications of the attack.

==> WTMC2022 - No Time for Downtime/section/result-edited.tex <==
 \section{Result and Discussion}
\label{sec:Result_and_Discussion}

We identify nearly 168K labeled domains with 94 unique industry categories from the categorization process that were Dyn customers on the day prior to the DDoS attack. Here we present the results of our analysis.

\subsection{Categorization of Dyn Customers}


We query category labels and reputation scores of the initial set of domains using a publicly available URL categorization service provided by McAfee ``Real-Time Database"~\cite{vallina_mis-shapes_2020}. \textbf{$\sim$62\% of the domains were categorized by McAfee.} 

Some domain names could not be categorized using McAfee; they are either no longer in operation or do not have enough features available for McAfee's classifier to make a deterministic classification. We refer to these domains as \textit{Un-categorized domains}. In this paper, we limit our analysis only to the domain names that McAfee successfully categorized, i.e., around 106K unique domains or nearly 62\% of all unique domains that used Dyn services one day prior to the attack (Fig.~\ref{fig:macro_flowchart}). 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/Flowchart-Domains.pdf}
    \caption{Dyn customer subdivision in category, domain status and reaction. We identify 169K customers and categorize them per our methodology. We distinguish exclusive and non-exclusive domains and subdivide them into reaction. $\sim$17K non-exclusive domains, 45 unsubscribed following the attack, and 24 out of 45 did not return to Dyn later.}
    \label{fig:macro_flowchart}
\end{figure}

Some domain names are mapped to multiple industry sectors and risk groups. We consider all retrieved category labels for our analysis. Hence, the total number of category labels retrieved for the domains exceeds the total number of unique domains.

We retrieve daily \textit{Domain Status} for all categorized domains from the measurement data for 20 days after the attack to observe status changes which we use to capture \textit{Domain Movements} as discussed in \S\ref{sec:methodology}.

\textbf{The number of \textit{Non-reactive Domains} is higher than \textit{Re-active Domains}.} The number of \textit{Non-reactive Domains} is significantly higher than those who became non-exclusive or unsubscribed (Fig.~\ref{fig:macro_flowchart}). We observed that more \textit{Exclusive Domains} either became non-exclusive or unsubscribed from Dyn services, as they had a greater probability of experiencing downtime due to the lack of redundancy in authoritative name servers.
Among non-exclusive domains, only 45 out of nearly 17K domains reacted. More than 85K out of $\sim$89K of \textit{Exclusive Domains} did not show any reaction (Fig.~\ref{fig:macro_flowchart}). This may be explained by the presence of cached \texttt{NS} records on DNS resolvers keeping several domains accessible during the outage~\cite{MouraIMC2018}. Also, for some organizations the short term cost of moving to another provider or adding redundancy may not justify benefits.

\textbf{The number of domains that became non-exclusive is not significantly different from the number of domains that unsubscribed.}
\textit{Re-active} domains showed two types of movement in terms of their decision to become non-exclusive or to unsubscribe from Dyn (Fig.~\ref{fig:macro_flowchart}). 
Among 3,197 re-active domains, 1,361 became non-exclusive and 1,836 unsubscribed.
There is no clear preference in the type of movement among domains. This observation motivates us to zoom into domains with similar characteristics, i.e., popularity or industry sectors, to discover specific preferences in the resilience strategy among similar Dyn customers.


\subsection{Popularity Influence on Decision to Re-act}
\label{sec:domain_popularity}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/reactive_by_alexa_rank_bin2.pdf}
    \caption{
        Reactions of Dyn customers -- re-active or non-reactive -- among different Alexa popularity groups. For example, among \textit{top100} Alexa customers, 42.9\% re-acted to the attack. (Note that larger groups are supersets, i.e., the \textit{top100} are included in the \textit{top1k})
    }
    \label{fig:by_popularity}
\end{figure}


We then incorporate Alexa rank data into our data set to indicate how popular each domain is. Out of $\sim$106K domains, we manage to retrieve popularity ranks of $\sim$5K domains that belong to the Top 1M Alexa list and ignore the ones which do not. We observe that domains with higher Alexa rank have a higher proportion of re-active domains (e.g., 42.9\% in top100) compared to those with lower rank (e.g., 14.3\% in top1m) as shown in Fig.~\ref{fig:by_popularity}:\ the percentage of re-active domains decreases as more domains with lower rank are included.
Popularity is thus one factor that appears to influence the decision to re-act.
A higher rank means higher traffic to these domains which may result in a higher revenue~\cite{truong_relationships_2018}.
Hence, owners of domains with higher rank will prefer minimizing downtime of their domains to avoid revenue loss. Meanwhile, owners of domains with lower rank may not be sensitive to short-term downtime.
Some reactions involve an extra cost, e.g., using multiple DNS service providers, which may not be worthwhile for businesses with smaller revenue.



\ 

\noindent
\textit{\textbf{Key takeaway}: We observe that customers running domains for more popular websites (based on Alexa rank) reacted to the attack with higher probability.}

\

\subsection{Industry Sector Influence on Re-action}
\label{sec:stat_analysis}

%We obtain nearly 106K labeled domains with 94 unique categories from the categorization process. 
We discuss in more detail the Industry Sectors that had a significant impact on the resilience strategy adopted by the domain managers. 

To determine the impact of individual industry sectors on domain reactions, we model the resilience strategy adopted by the domains as a function of their industry sector using a multivariate logistic regression analysis. We model the binary decision of domains to re-act (re-act: \textbf{R1}/\textbf{R2}/\textbf{R3} or not react: \textbf{R0}) as a dependent variable (\ref{eq:logit_decision}). 

\begin{equation}
\label{eq:logit_decision}
    \text{\textit{logit}}(\pi_{b})=\log[\frac{\pi_{b}}{1-\pi_{b}}],
\end{equation}

\noindent where $\pi_{b} \in [0,1]$ represents the probability of a domain reacting and can be estimated using (\ref{eq_logit_estimation}).

\begin{equation}
    \label{eq_logit_estimation}
    \pi_{b}=\frac{\beta_{0}+\sum_{i}^{}\beta_{i}x_{i}}{1+(\beta_{0}+\sum_{i}^{}\beta_{i}x_{i})},
\end{equation}

\noindent where $x_{i} (i=1,2,3,....,94)$ represents each industry sector as a separate independent variable. $x_{i}$ has a value of 1 if a domain belongs to this industry sector, otherwise it has a value of 0. $\beta_{i}$ is the odds ratio and signifies the strength of correlation between this independent variable and the dependent variable. To implement logistic regression, we use \texttt{statsmodels} package in python~ \cite{seabold2010statsmodels}.
% In this analysis, $\beta_{i}$ shows the factor with which an industry sector $i$ will increase the probability of a domain to re-act.

The regression model outputs three main metrics to indicate the influence of each category (shown in Table~\ref{tab:stat_result}).
\textit{Coefficient} ($\beta_{i}$) is used to calculate the factor by which the probability of a domain re-acting to the attack increases, if this domain belongs to Industry Sector $i$,  i.e., if the regression coefficient is estimated as $\beta_{i}$ then the probability of post-attack domain re-action increases by $e^{\beta_i}$ times as compared to the base case.


\begin{table}[t]
    \centering
    \caption{GLM coefficients for domains showing most prominent industry sectors that had a statistically significant influence on domain reactions (ordered by the number of domains in each industry sector).
    }
    \label{tab:stat_result}
    
   \begin{tabular}{lrr}
\toprule
Industry Sector&    Coefficient\textsuperscript{*} &       z-value \\
\midrule
Internet Services                    &  0.47 &   6.80 \\
Travel                               &  1.25 &  14.61 \\
Content Server                       &  1.26 &  11.00 \\
Motor Vehicles                       &  0.78 &   6.26 \\
General News                         &  2.17 &  24.05 \\
Job Search                           &  1.30 &   9.40 \\
Streaming Media                      &  2.15 &   6.57 \\
Gambling                             &  1.60 &   8.97 \\
Portal Sites                         &  1.74 &   6.51 \\
PUPs (potentially unwanted programs) &  2.83 &  12.28 \\
Malicious Sites                      &  2.61 &   8.91 \\
Social Networking                    &  2.47 &   7.75 \\
Personal Pages                       &  1.87 &   5.37 \\
Provocative Attire                   &  2.71 &   4.86 \\
For Kids                             &  3.07 &   4.93 \\
Interactive Web Applications         &  2.61 &   7.97 \\
Weapons                              &  1.98 &   5.32 \\
Professional Networking              &  3.58 &   9.34 \\
Visual Search Engine                 &  4.12 &   7.42 \\
Instant Messaging                    &  4.03 &   5.32 \\
        \bottomrule
        \textit{\textsuperscript{*}p$<$0.001}
    \end{tabular}
\end{table}

For example, domains in the \textit{Professional Networking} with a coefficient value 3.58 are 16 times (i.e.\ $\dfrac{e^{3.58}}{e^{0.78}}$) more likely to re-act than domains in the \textit{Motor Vehicles}, such as web sites of car manufacturers and sales, with a coefficient value 0.78.
Hence, we expect the proportion of re-active domains is higher in the former than the latter.
\textit{p-value} indicates if the coefficient of a domain is statistically significant or not. 
\textit{z-value} is calculated as the number of standard deviations the average decision of a certain industry sector is away from the average decision of the whole data set~\cite{mcleod_z-score_2019}. It indicates the reliability of the coefficient computed by the logistic regression model.

We discuss the type of reactions observed for domains that belong to any of the top 20 industry sectors whose coefficient was both highly reliable (greater than the median \textit{z-value} as shown in Fig.~\ref{fig:z_hist}) and statistically significant (\textit{p-value} $<0.05$).

The results indicate that some categories have more significant correlation to the resilience strategy than others.
Domains in industry sectors with higher coefficient have a higher probability to re-act following outages, such as \textit{General News} and \textit{Streaming Media}. 
DNS providers should anticipate the reaction from customers in these industry sectors more than other sectors.


\ 

\noindent
\textit{\textbf{Key takeaway:} By using a multivariate logistic regression model, we were able to calculate and reveal that for 34 out of 94 industry sectors, there is statistically significant influence on the post-attack reaction.}

\ 


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/z_value.png}
    \caption{Distribution of z-values (signifies reliability) for industry sector coefficients in the linear regression model. We discuss in more detail the reactions of domains that belong to 20 industry sectors with the largest z-values, indicated by the shaded area.
    % which, according to the logistic regression model, had a reliable and statistically significant impact on the reactions.
    }
    \label{fig:z_hist}
\end{figure}

We also observe a number of industry sectors which \textbf{do not} have statistically significant influence on the decision to re-act such as \textit{Religion}, \textit{Ideologies}, and \textit{Politics}.
Religion and Ideologies sectors include web pages that discuss spirituality and beliefs while Politics domains host discussions of political parties, views, and opinions. We suspect that domains in these sectors do not require high resilience.

\ 

\noindent
\textit{\textbf{Key takeaway:} Some industry sectors do not seem to have a statistically significant influence on the decision to re-act after the attack.}

\

We zoom into a number of significantly influential industry sectors (Table~\ref{tab:stat_result}).
Fig.~\ref{fig:reactions_by_category} shows how domains in these industry sectors reacted.
The \textit{top plot} shows proportions of re-active domains in each industry sector, characterized by their decision to become non-exclusive or to unsubscribe after the attack.
The diminishing line in the top plot indicates the size, i.e., number of domains, of each industry sector on a $log_{10}$ scale.
We observe that sector size does not directly correlate with the proportion of re-active domains in the sector.
However, we demonstrate that reactions vary among industry sectors in two ways: the proportion of \textit{re-active} domains and the dominant type of reactions.

From the \textit{top plot} in Fig.~\ref{fig:reactions_by_category}, we show that most domains in some industry sectors \textit{became non-exclusive} following the incident, i.e., used additional DNS providers, such as domains in \textit{General News}, \textit{Potentially Unwanted Programs (PUPs)}, \textit{Malicious Sites}, and \textit{Visual Search Engine}.
Domains in \textit{PUPs} and \textit{Malicious Sites} categories are made with an intention to infect user's computer with software or other malicious activity, e.g., Trojan horses and viruses.
Domains in \textit{Visual Search Engine} include web pages that provide searching functionality with image-specific results.
The reaction to use multiple DNS services might indicate that these domains have a high -- most probably financial -- value for the owners, hence, it is important to keep them up at all times.
After the attack, these domains used back-up services to be more resilient against future outages. Therefore, we assume that the revenue from the domains is large enough to compensate for the cost of using an additional DNS service, if present.

Meanwhile, domains in some industry sectors showed a significant preference to \textbf{unsubscribe}, i.e., they stopped using Dyn service, after the attack (Fig.~\ref{fig:reactions_by_category}).
Among them, we observe domains intended for adult audiences -- \textit{Gambling} sites, web pages about \textit{Weapons}, and sites showing \textit{Provocative Attires} -- and the domains intended for more general audiences such as \textit{Motor Vehicles} sites, \textit{Streaming Media}, and \textit{Social Networking} sites.
The reaction to unsubscribe after the attack might also indicate that domain owners value their domains and find it necessary to re-act after the attack.
However, we suspect that the cost of using a secondary DNS service is not worth the revenue from the domain, or the owner considers Dyn no longer reliable.

\begin{figure*}[]
    \centering
    \includegraphics[width=\linewidth]{figure/plot_sector_v5-2.pdf}
    \caption{
        Behaviors of domains in selected industry sectors.
        \textbf{Top Plot} shows the proportions of domains with different reactions in each sector along with the sector sizes.
        \textbf{Middle Plot} shows the proportions of unsubscribed domains that did not return.
        % \textbf{Bottom Plot} shows the mean and variation of Alexa rank of domains in each sector.
        \textbf{Bottom Plot} shows the distribution of Alexa ranks among domains that belong to a certain industry sector.
    }
    \label{fig:reactions_by_category}
\end{figure*}
\

\noindent
\textit{\textbf{Key takeaway:} We see a difference in the type of reaction based on the industry sector. In some sectors, domains for the most part became non-exclusive following the attack (e.g., \textit{General News}), while for others, customers largely unsubscribed (e.g., \textit{Gambling}).}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} We analyse the type of reactions observed for the domains in selected industry sectors (Fig.~\ref{fig:reactions_by_category}). We see a difference in the type of reaction based on the industry sector: In some sectors such as \textit{General News}, domains predominantly became non-exclusive following the attack, while some others such as \textit{Gambling} domains tend to unsubscribe.} 
   % \end{minipage}}
% [DELETE] This number reflects the relative importance of keeping the domain operational from the perspective of domain owners. 
% [DELETE] A higher proportion in certain type of decision might reflects the risk appetite of the domain owners, especially because each type of reaction has different risk level (\S\ref{sec:key_concepts}). 

\ 

The \textit{middle plot} shows the proportion of return among domains that unsubscribed in each sector.
This metric is important to measure the business impact of an outage incident as it indicates how many customers the provider loses for a longer term.
In some industry sectors such as \textit{Travel} (e.g., ticketing sites), \textit{Motor Vehicles}, and \textit{Personal Pages} (e.g., blogs), more domains \textbf{did not return} than those did return.
On the contrary, the behavior was quite the opposite in \textit{Gambling}, \textit{PUPs}, and \textit{Malicious Sites} sectors, i.e., most unsubscribed domains \textbf{returned} later.
In \textit{Visual Search Engine} sector, there is no domain that unsubscribed, hence, no data is shown in the plot for that sector.
% This number might reflect the relative tolerance of domain owners against service failure by the provider.
% High proportion of domains which did not return might indicate low tolerance among the domain owners e.g., due to trust loss. 
% On the other hand, domains that returned might still consider Dyn as a trustworthy provider or already have a good relationship with Dyn.

\ 

\noindent
\textit{\textbf{Key takeaway:} In some industry sectors, domains that unsubscribed mostly did not return (e.g., \textit{Travel}), while in others, a higher proportion of domains unsubscribed and returned (e.g., \textit{Gambling}). This suggests that the industry sector affects decision-making.}

%\noindent \fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} In some industry sectors, such as Travel, most domains that unsubscribed after the attack did not return, while in some other sectors, such as \textit{Gambling}, a higher proportion of domains returned. This shows that for some sectors, the chance of customers leaving for a longer term is higher. Domains belonging to \textit{visual search engine} category only used becoming non-exclusive as a resilience strategy.} 
   % \end{minipage}}

\ 

% [Still working] 
The \textit{bottom plot} in Fig.~\ref{fig:reactions_by_category} shows the distribution of Alexa ranks of the domain names -- where present -- within each industry sector categorized by their responses after the attack i.e., re-active or non-reactive. 
This plot reveals insights into the influence of popularity on the choice of resilience strategy adopted by domains in each industry sector.
% 
%\textcolor{red}{There are a number of domain categories that are in Fig 4 but we never talk about in the text. Why?}
% The latter metric indicates how diverse the Alexa ranks are within that category.
% For example, most domains in \textit{Job Search} sector have higher Alexa ranks i.e., more popular, than domains in \textit{General News}, but more uniform i.e., have similar popularity.
%For example, in \textit{Job Search} and \textit{Gambling} categories, Alexa ranks of domains that reacted (dark box plot and light dots) are more concentrated in the lower plot (shorter box), indicating a higher popularity, compared to those which did not re-act (light box plot and dark dots) which are more dispersed (longer box) and, in majority, less popular.
For most industry sectors shown in Fig.~\ref{fig:reactions_by_category}, the average popularity of \textit{re-active} domains was higher than the average popularity of non-reactive domains. This is consistent with our previous findings in \S\ref{sec:domain_popularity} that higher popularity influences the domain decision to react.
However, we see that popularity was a more significant factor for some industry sectors than the others. \textbf{Non-overlapping inter quartile ranges (IQR)} for the box plots in \textit{Job Search} and \textit{Gambling} sectors indicate a strong correlation between popularity and the decision to react.
Meanwhile, in some industry sectors such as \textit{Internet Service}, domain popularity does not seem to have a strong correlation with the decisions to react, considering the substantial \textbf{overlap in the IQR} for the box plots of re-active and non-reactive domains.
% Therefore, a \textit{high mean} of Alexa rank with \textit{low coefficient of variation} indicates that the domain popularity plays significant role in the decisions to react such as domains in \textit{Weapons}, \textit{Provocative Attires}, and \textit{For Kids}.

\ 

\noindent\textit{\textbf{Key takeaway:} In some industry sectors (e.g., Job Search), the influence of popularity on the decision to re-act is stronger than in others (e.g., Internet Service).}
%\noindent \fbox{%
    %\begin{minipage}{0.95\linewidth}
%    \textit{\textbf{Key takeaway:} The popularity of domains in some industry sectors with high and similar Alexa ranks such as Job Search might have a significant influence on the decisions to react after the attack.} 
%    \end{minipage}}
% 
% We make a couple of further observations regarding domains in the selected categories.  
% % Figure~\ref{fig:reactions_by_category}.
% % 1
% Domains in \textit{Potentially Unwanted Programs (PUPs)} and \textit{Malicious Sites} categories predominantly became non-exclusive following the incident, and none of unsubscribed ones that did not return.
% In addition, we could see that none of domains in these two categories belong to Top 1M Alexa list. This is predictable since malicious websites are rarely found in top Alexa list~\cite{kim_malicious_2018}.
% % domain examples
% Domains in these categories are made with intention to infect user's computer with software or script to hijack or alter security and privacy, e.g., Trojan horses and viruses.
% % 2
% % 3
% Domains for adult audience i.e., \textit{Gambling}, \textit{Weapons}, and \textit{Provocative Attire}, predominantly unsubscribed after the incident. 
% However, in \textit{Gambling} sector, only 20\% that did not return.
% In addition, Alexa rank mean and variation for the other two sectors indicate that domains in these sectors are homogeneously quite popular and suggest a strong influence on the reaction.
% % example
% Domains in Gambling sector include web pages that allow users to place bets online.
% Domains in Weapon sector include web pages that provide every information about weapons, including buying, for either personal or military use.
% Meanwhile, domains in Provocative Attire sector include web pages showing non-nudity revealing attires intended to provoke the viewers. 
% \newline \newline \textit{\textbf{Key takeaway:}} \newline
% 
% % 4
% Domains in \textit{General News} predominantly became non-exclusive but more than 82\% of unsubscribed ones did not return.
% Furthermore, this behavior is less likely to be influenced by domain popularity due to a high diversity in their Alexa rank.
% % domain example
% Domains that belong in this category include news portals, both regional and international.
% % 
% Domains in \textit{Professional Networking} and \textit{Social Networking} show a similar behavior.
% Most of them unsubscribed then did not return which might indicate low tolerance against violation in service fulfillment.
% % example
% Domains in this category include social networking for professional use and friendship focus. 
% % 5
% Lastly, domains in \textit{Visual Search Engine} sector only reacted by becoming non-exclusive, hence, no data about their return behavior.
% % example
% This category includes web pages that provide searching functionality with image-specific results.


% \begin{observation}
%     Majority of reactive domains in Sport sector unsubscribed from Dyn but majority of them returned.\textcolor[red]{Too anecdotal. Maybe for most observations it is better to talk in terms of how Industry sector as a factor explains the decision taken by domain owners.}
% \end{observation}

% Discussion here.

% \begin{observation}
%     In Marketing/Advertising, Online Shopping, and Entertainment sectors, there were more reactive domains that unsubscribed than those which stayed. More than 80\% of those which unsubscribed did not return.
% \end{observation}

% Discussion here.






% \textbf{Reactive or Not reactive:\ }

% \textbf{Become Non Exclusive or Unsubscribe:\ }
% There are two likely reactions that a domain owner could take following the outage incident: to become non-exclusive or to unsubscribe. We observe that the proportion of these two reactions varies among different types of domain. 
% For example, domains in Finance, e.g., banks and loans, mostly chose to leave Dyn while domains in Business e.g., trading companies, mostly chose to keep using Dyn but became non-exclusive i.e., use managed DNS service from other providers following the incident (Figure~\ref{fig:first_reaction_industry}). 
% % One possible explanation is that domains in Finance are easier to lose trust following the incident. 
% This behavior is consistent with the fact that finance-related domains are more trust sensitive.
% It is likely that they require highly reliable partners to support their operation and less tolerant with service failure.

% In contrast, the intended use of the domains did not correlate with its reaction, as shown in Figure~\ref{fig:reaction_by_purpose}. Most domains reacted by stop using the service regardless their intended uses.

% \todo[inline]{MJ: Does proportion mean ratio/fraction? Does it mean numbers? The table 2 caption mentioned the word proportions before, but table 2 only tabulates numbers. The numerical metrics speak of proportions and there it seems to be about fractions. Here you are not giving fractions, but you do seem to compare absolute numbers from two reactivity classes (nonex and noncust). Please be consistent/avoid ambiguity.}

% 
% \begin{figure}%[ht]
%      \centering
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/first_reaction_by_purpose2.png}
%          \caption{ }
%          \label{fig:reaction_by_purpose}
%      \end{subfigure}
%      \hspace{1em}
%     %  \hfill
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/windowed_departing_domains_by_purpose.png}
%          \caption{ }
%          \label{fig:returning_by_purpose}
%      \end{subfigure}
%         \caption{Reaction (a) and return movement (b) by intended use }
%         \label{fig:by_purpose}
% \end{figure}

%\subsubsection{React Immediately or Later.}
% \textbf{React Immediately or Later:\ }
% Another aspect that reflects the importance of DNS service availability for businesses is immediacy of the reaction. 
% % As discussed in \S\ref{sec:mdns_business}, DNS service could be a key service in certain digital businesses, especially those who rely on Internet-based systems. Each second of downtime could cost them millions of dollar. For these type of businesses, they need to react immediately to return the availability of their systems. On the other hand, other businesses could react later because every second of downtime does not cost them much. 
% From the data, we observed that most domains in Finance reacted later than most domains in Business and News Portal. 
% Figure~\ref{fig:finance_late_response} shows that most domains in the financial sector reacted after the end of the month, while domains in more general categories mostly reacted immediately i.e., the next day following the incident. Despite the late reaction, almost all domains in the financial sector reacted by leaving Dyn. Meanwhile, we observe that domains in News category which left Dyn reacted immediately, but those which became non-exclusive reacted later in similar number. Hence, we may conclude that most domains in Finance sector might not suffer a great loss for each second of DNS unavailability but still lost their trust with the provider. Another possible explanation regarding this behavior is because the contract ended at the end of the month. Therefore, it is more efficient to wait until the previous contract ends before starting to use and pay for another service.

% Based on intended uses, similar proportions of domains that mainly provide service reacted on two specific days: day +1 and day +12. Further analysis is required to discover what type of services these domains provide to explain the difference. Domains that provide information and network reacted similarly i.e., immediately left after the incident, as shown in Figure~\ref{fig:reaction_time_by_purpose}.

%\subsubsection{Return or Leave for Good.}
% \textbf{Return or Not:\ }
% The third aspect that we analysed is the return movement among domains in different industry sectors. 
% % Previously, we have discussed that most domains in Finance chose to left Dyn, despite their late response.  
% We found out that most domains in Finance not only leave Dyn but almost all of them left for good. 
% Compared to other industry sectors, the proportion of Finance domains that left for good is much higher (Figure~\ref{fig:departing_by_industry}). 
% This fact supports our belief that domains in Finance are less tolerant of service failure thus prefer to leave and switch to other service providers. Based on intended use, we found no obvious difference in the proportion of domains that returned after they left, as shown in Figure~\ref{fig:returning_by_purpose}.  

% \begin{figure}[p]
%     \centering
%     \begin{subfigure}[b]{0.85\textwidth}%[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_time_to_react_finance.png}
%     \caption{\textbf{Time to react by industry sector.} Despite the tendency to leave instead of becoming non-exclusive, most domains in Finance (top) left Dyn after end of the month (a), while most domains in Business (middle) and News, Portal, and Search categories (bottom) left Dyn immediately i.e., the next day after the attack (b and c).}
%     \label{fig:finance_late_response}
% \end{subfigure}
% % 
% \begin{subfigure}[b]{0.85\textwidth}%[H]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_time_to_react_by_purpose.png}
%     \caption{\textbf{Time to react by intended use.} Most domains that provide service reacted by leaving Dyn. Many domains in this category left after end of the month (a), while in the other two categories, only a few left later.}
%     \label{fig:reaction_time_by_purpose}
% \end{subfigure}
% % 
% \begin{subfigure}[b]{0.85\textwidth}%[H]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_departing_domains_by_industry.png}
%     \caption{\textbf{Behavior of leaving domains by industry sector}. Majority of leaving domains in the Finance category did not return.}
%     \label{fig:departing_by_industry}
% \end{subfigure}
% \caption{Behaviour of domains for selected industry sectors.}
% \label{fig: behaviour of domains}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=.5\textwidth]{figure/plot3_behavior_by_functional_type.png}
%     \caption{Domain behaviors by different reactions across functional types.}
%     \label{fig:reactions_by_functional}
% \end{figure}

% \begin{observation}
%     Among reactive domains with Information/Communication function, there were more domains that stayed (4.2\%) than those which unsubscribed (2.2\%). Nevertheless, 81.8\% of those which left did not return.
% \end{observation}

% Information/Communication e.g. general news, search engine, and online forum.

\subsection{Risk Level Influence on Decision to React}
\label{sec:domain_risk_level}

%\textcolor{red}{Number of unverified, medium and high risk level websites are very low. Do comment on the aggregate numbers of these websites. How many are these?}

% Explain briefly about methodology to determine risk level.
% \textcolor{red}{
%     Discuss:
%     \begin{itemize}
%         \item DONE Only a few domains in unverified, medium, and high risk $\xrightarrow{}$ most Dyn consumers are legitimate domains
%         \item DONE Discuss med and hi risk domains, why use Dyn? why use redundancy? why return? $\xrightarrow{}$ premium crimes which needs hi availability.
%         \item DONE Discuss med hi risk domains with domains in PUPs and Malicious. compare behavior $\xrightarrow{}$ what it means?
%         \item In risk group, compare domains in security risk with domains in med and hi risks
%     \end{itemize}
% }

% Join two plots together using shared y axis!
We analyze how risk level of the domains influences their reaction following the attack. Fig.~\ref{fig:reaction_by_risk_type} shows the behavior of domains with different risk categories, characterized by risk level and risk group.
Recall that McAfee categorizes domains based on the reputation score into four risk levels as shown in \S\ref{sec:methodology}.
% \textit{Risk Level} is individually measured for each domain based on its reputation score~\footnote{See \url{https://trustedsource.org/download/ts_wd_reference_guide.pdf}}. 
% \textit{Unverified} refers to the level of risk which lies between minimal and medium risk.
Most domains using Dyn services are categorized as `Minimal Risk'. Out of 106K domains of Dyn customers, 104K are in Minimal Risk while domains in Unverified, Medium Risk, and High Risk categories only account for 2K domains (Fig.~\ref{fig:reaction_by_risk_type}).
% \textcolor{red}{add the exact number DONE}
%This indicates that majority of Dyn customer domains were relatively safe to use.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/plot_risk_combined3-4-4.pdf}
    \caption{
    Behaviors of domains with different \textit{Risk Levels} and \textit{Risk Groups}. 
    \textbf{Top Plot} shows the proportions of domains with different reactions in each group along with the group sizes. 
    \textbf{Middle Plot} shows the proportions of unsubscribed domains that did not return. 
    \textbf{Bottom Plot} shows the comparison in the distribution of Alexa ranks of re-active and non-reactive domains within each category.
    % Domain behaviors by different reactions across different \textit{Risk Levels} and \textit{Risk Groups}.
    % \textcolor{red}{Risk Type -- Risk Group}
    }
    \label{fig:reaction_by_risk_type}
\end{figure*}

Some domains with higher risk levels also need high availability, hence, using the managed DNS service from Dyn.
As illustrated by the \textit{top plot} in Fig.~\ref{fig:reaction_by_risk_type}, some Dyn customers are domains in \textit{medium} and \textit{high risk} levels and they show a similar preference to become non-exclusive after the attack, i.e., use redundant DNS services.
Moreover, most domains with medium and high risks returned if they unsubscribed, (the \textit{middle plot}).
% This observation reflects the resilience strategy of some malicious domains -- most probably with high revenue -- which demand higher availability from premium and redundant DNS services.
We also observed this behavior among domains intended to victimize the users, e.g., PUPs and Malicious Sites (\S\ref{sec:stat_analysis}).
% 
% We make a couple of observations with regards to Risk Level influence on the domains reactions.
% 1
% Domains with \textit{medium} and \textit{high risk} level show a similar behavior, namely, they predominantly became non-exclusive. Furthermore, none of those which unsubscribed did not return. 

% 2
We see a significant \textbf{overlap in the IQR} in the box plots of Alexa ranks for domains categorized as minimal risk (see:\ \textit{bottom plot} of Fig.~\ref{fig:reaction_by_risk_type}). This shows that popularity (for this aggregate set of domains) does not play a major role in deciding the post-attack reactions. The number of re-active domains categorized as unverified or medium risk are too low to derive any conclusions about the influence of popularity on the observed reaction. Meanwhile, no domain categorized as a high risk belonged to Alexa Top 1M list. This observation is again consistent with our result in \S\ref{sec:stat_analysis} with domains categorized as \textit{malicious domains}.

%Domains classified as medium risk are relatively quite popular (concentrated in the lower area) reflecting that some visitors unknowingly risk their security by regularly accessing the domains.

\

\noindent
\textit{\textbf{Key takeaway:} Customers with higher risk levels mostly became non-exclusive after the attack and the majority of those who unsubscribed instead also later returned.} 
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} Domains with higher risk levels mostly became non-exclusive after the attack and majority of those who unsubscribed returned later.} 
   % \end{minipage}}

\ 

% Moreover, there is another conclusion we could infer about domains with minimal risk from Figure~\ref{fig:reaction_by_risk_type}.
% 3
%\textcolor{red}{The word "active" needs to be removed everywhere.}
In addition, considering the \textit{top} and \textit{middle plots} in Fig.~\ref{fig:reaction_by_risk_type}, we observe that majority of the domains with minimal risk stopped using Dyn services permanently following the attack, i.e.\ nearly 1K domains or 71.4\% of those that unsubscribed did not return.
This shows that once customers of DNS service providers unsubscribe there is less chance for them to re-subscribe to the service. Other DNS providers may use similar heuristics to estimate customer loss following an outage.
%\newline \newline \textit{\textbf{Key takeaway:} Legitimate domains have a relatively high tendency not to return once they unsubscribe from the DNS service after an outage.}

\ 

\noindent
\textit{\textbf{Key takeaway:} Our results show that if domains in the minimal risk category unsubscribe, the probability that they stay away for a longer time is higher.}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth} \textit{\textbf{Key takeaway:} There is a greater probability for domains in the minimal risk category to stop using Dyn for a longer term if they unsubscribe.}
  %  \end{minipage}}
    
\subsection{
% [Still working] 
Risk Group Influence on Decision to React}
\label{sec:domain_risk_type}

%\textcolor{red}{Structure suggestion:Recall definition of a category and discuss the types of websites that will fall in the category. Discuss how different is the reaction to other risk groups (See top plot). Discuss return behaviour (second plot). Do only popular websites move; or do all websites have similar likelihood of moving? Repeat for the next category. Note that in the documentation, it is "risk group" not "risk type".[DONE]}

% Category labels from the URL categorization service indicates the functionalities of the domains based on their content (if present).
% When used improperly, domains with certain functionalities might lead to unintended situations and negatively impact businesses or individuals.
% McAfee classifies URL categories into \textit{Risk Groups} based on which main aspect is the most at risk when this unintended situation happens.
% According to the documentation,
% \textit{Risk Group} refers to the main aspect which domains in certain category i.e., industry sector, might risk.
% For example, domains with \textit{Productivity} risk are non-business related which might reduce one's productivity at work e.g., social media and entertainment portal.
% Another example, domains with \textit{Bandwidth} risk are mainly web pages whose contents require a large amount of bandwidth to retrieve e.g., video streaming portal, hence, might disrupt business related communication over the network. 

Fig.~\ref{fig:reaction_by_risk_type} shows the re-actions among domains that belong to different Risk Groups.
% 4
According to the \textit{top plot}, domains with \textit{Liability}, \textit{Bandwidth}, and \textit{Propriety} risks show a slight preference to unsubscribe after the attack. More than 60\% of the unsubscribed domains in these categories did not return. %Re

% 3
Meanwhile, as shown in the \textit{middle plot}, we observe similar return behaviors of domains in different risk groups, i.e., more than half of them did not return after they unsubscribed, except for domains in \textit{Security} risk group.

% 5
% Regarding domain popularity illustrated by the \textit{bottom plot}, even though the mean Alexa rank of each risk group is similarly high, but popularity of domains in \textit{Productivity, Information,} and \textit{Liability} risk groups are more uniform.
% This implies that popularity of domains in these 3 risk groups might have a significant influence on the reactions after the attack.

%We observe in the \textit{bottom plot} of Fig.~\ref{fig:reaction_by_risk_type} that Alexa ranks of re-active domains are more concentrated in the lower area, i.e., more popular, in every risk group. 
As shown in the \textit{bottom plot} of Fig.~\ref{fig:reaction_by_risk_type}, the popularity of re-active domains in all risk groups (except Security) is higher than the popularity of the domains that do not re-act. For 5 of the 7 risk groups, we observe that the re-active domains are concentrated in relatively higher Alexa ranks. This indicates that for these domains (i.e.\ \textit{Liability, Security, Propriety, Bandwidth}, and \textit{Communications}), popularity played an important role in the decision of domain owners to re-act. Interestingly, these domains also include websites providing streaming and messaging services.    

%\textit{Security} group includes websites which can be used for phishing credentials, 

This result is consistent with our observation in \S\ref{sec:domain_popularity} that higher popularity shows a correlation with the decision to re-act after the attack.
In \textit{Productivity} and \textit{Information} risk groups (eg.\ social media websites), we see a substantial \textbf{overlap in the IQR} of the re-active and non-reactive box plots, which indicates a weaker correlation of the domain popularity with the decision to react.

%\textcolor{red}{The domains popularity in some risk groups such as Productivity might have a strong influence, why? What about information and liability?}
% 

\

\noindent\textit{\textbf{Key takeaway:} Domains in some risk groups (e.g., Liability) mostly unsubscribed after the attack.}

\

% \noindent\fbox{%
%     \begin{minipage}{0.95\linewidth}
%     \textit{\textbf{Key takeaway:} Domains in some risk groups such as \textit{Liability} (recall: may serve pirated material) mostly unsubscribed after the attack. 
%     \textcolor{red}{
%     The domains popularity in some risk groups such as Productivity might have a strong influence on the domain reactions after the attack. Popularity of websites have a lower impact on post-attack reactions for the domains that consume greater \textit{Bandwidth} or can be used for \textit{Communication}.}
%     }
%     \end{minipage}}

% Lower variation in these risk types indicate that the domains are relatively more homogeneous in terms of popularity, i.e., similarly quite popular (Figure~\ref{fig:reaction_by_risk_type}).

% \begin{figure}[t]
%      \centering
%      \begin{subfig}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/plot_risk_level_v2.pdf}
%         \caption{By risk level}
%         \label{fig:by_risk_level}
%      \end{subfig}
%      \hfill
%      \begin{subfig}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/plot_risk_type_v2.pdf}
%         \caption{By risk type}
%         \label{fig:by_risk_type}
%      \end{subfig}
%         \caption{Behavior by risk profile.}
%         \label{fig:by_risk_profile}
% \end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=.25\textwidth]{figure/plot_risk_level_v2.pdf}
%    \caption{Domain behaviors by different reactions across risk levels [make subfigure]}
%    \label{fig:reaction_by_risk_level}
%\end{figure}

\subsection{Analysis on Domain Autonomous Systems}
\label{sec:domain_as}

A single party can operate multiple domains that rely on Dyn for DNS. For example, Alphabet Inc. operates, among others, google.com and gmail.com. So far we have not considered the potential effects of a single party making decisions (i.e., driving domain reactions) for multiple domains. 
As a first step towards exploring if multiple re-actions can be correlated with decisions made by a single party, we measure the variety of reactions of Dyn customers within each Autonomous System (AS).

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/AS-and-Rank-histogram-2.pdf}
    \caption{Distribution of variety in re-actions among Domains mapped to an AS.}
    \label{fig:AS_Size_Histogram}
\end{figure}

We associate domains to their hosting network at the time of the Dyn attack by mapping IP addresses (i.e., \texttt{A} records) to AS numbers, using IP-prefix-to-AS data from CAIDA~\cite{the_caida_ucsd_routeviews_2008}. 
% We then calculate the number of IP addresses per AS that are used to host domains that react and compare it with the total number of IP addresses in each AS used to host Dyn customers. 
We then calculate the percentage of re-active domains that re-acted in each AS. In other words, if two domains (both Dyn customers) mapped to a single AS and one re-acted, the percentage of re-active domains for that AS is 50\%.
Fig.~\ref{fig:AS_Size_Histogram} shows the resulting distribution. We only include ASes that were mapped to at-least 1 re-active domain in this plot. Nearly 1.6K different ASes, each in which on average 14 domains were hosted, showed no re-active domains at all.
We observe that in the case of about 200 smaller ASes (one to only a few domains hosted), the domains all showed the same behavior (i.e., 100\% re-acted). This suggests that parties that operated several domains drove the reaction for multiple domains, but on the order of a few hundred domains in total based on our initial view. This approach of course does not account for cases where a single party hosts their domains in multiple networks, which we leave for future work.

\

\noindent\textit{\textbf{Key takeaway:} Domains mapped to the same AS showed different re-actions.}

\
%In some cases, multiple domains can be operated by a single party. For example, an enterprise such as Alphabet Inc. can operate multiple domains such as google.com and gmail.com.\ Currently, we do not view the impact that the concentration of domains among the parties that operate them has on our results. However, to further explore if there are multiple parties responsible for the reactions we observe, we measure the variety of reactions observed within each AS. 
% \textcolor{red}{
%To do so, we extract the type of hosting that a domain was using during the incident by mapping IP address from domain's \texttt{A} record to its corresponding Autonomous System (AS) using IP prefix to AS dataset~\cite{the_caida_ucsd_routeviews_2008}
% } 
%Using this data we calculate the percentage of IPs that react out of the total number of IPs related to the domains using Dyn name servers. Fig.~\ref{fig:AS_Size_Histogram} shows the distribution for the percentage of \texttt{IP} addresses within each AS that react. We observe that in the case of only the smaller ASes, all domains show the same behaviour. For, larger ASes, we see only a small fraction of domains showing reactions. This shows that the resilience strategy chosen by domains within each AS was not the same, except when these ASes were relatively small.






%\textcolor{red}{A subsection on what kind of diversity in decisions do we notice per AS would be nice to argue that not all IPs in an AS reacted the same way.}


% \subsection{Hypothesis Testing}

% To test whether the differences in behavior across industry sectors and intended use are statistically significant, we did a statistical test. We compared the daily number of domains from two categories as two related-pair samples. Because most data are not normally distributed according to the Shapiro-Wilk test \cite{shapiro_analysis_1965}, we could not do a simple paired t-test. Instead, we did the Wilcoxon signed-rank test \cite{wilcoxon_individual_1945} for all possible pairs of industry sectors and intended uses. We repeated the test for three daily variables: number of domains that become non-exclusive, left, and returned. 
% The test shows variation in results between categories: some pairs are significantly different and some others are not. 
% A complete result of this test is presented in Table~\ref{tab:ttest_by_industry1}, Table~\ref{fig:returning_ttest_by_industry}, and Table~\ref{tab:ttest_by_purpose} in Appendix, alongside the complete metrics calculation in Table~\ref{tab:metrics_by_industry} and Table~\ref{tab:metric_by_purpose}.
% 


==> WTMC2022 - No Time for Downtime/section/result.tex <==
 \section{Result and Discussion}
\label{sec:Result_and_Discussion}
% 
%We next present our results and discuss the implications for various stakeholders. %Third, we discuss the limitation of this research and possible further studies in the future.
% 
%\subsection{Descriptive Statistics}
%As discussed in Section~\ref{sec:key_concepts}, all active domains which used Dyn service a day before the incident can be categorised into reactive and non-reactive domains. They can also be categorised based on their statuses i.e., exclusive or non-exclusive. Figure~\ref{fig:domain_count} summarises the number of domains according to these categorisation.
% 
%In the previous section, we introduce the key concepts and state a step-by-step methodology. Here, we present our findings.
We identify nearly 168K domain names that were Dyn customers on the day prior to the DDoS attack. 

%discuss the results of each step we performed in more detail. 

% start with initial finding
% We start by explaining some initial findings and summary of our data set that are important to note, including URL categorization results and the distributions of domains by their initial status and reactions.
% influence of each aspect
% Then, we discuss the influence of each aspect of domains characteristics to the domains post-attack reactions.
% key takeaway
% We also attach key takeaways preceding discussions in this section in bold format.


%
% \begin{table}[]
%     \caption{Summary of domains.}
%     \setlength{\tabcolsep}{3pt}
%     \renewcommand{\arraystretch}{1}
%     \resizebox{.48\textwidth}{!}{%
%         \centering
%         % \tiny
%         \begin{tabular}{ l r r }
%             % \hline
%             \toprule
%             {\textbf{Description}} & {\textbf{Unique Count}} & {\textbf{\% of Total}} \\
%             % \hline
%             \midrule
%             Initial Set of Domains* & 168,577 & 100.00\% \\
%             \quad Uncategorized Domains** & 62,408 & 37.02\% \\
%             \quad Categorized Domains & 106,169 & 62.98\% \\
%             \quad \quad Non-reactive Domains (\textbf{R0}) & 102,972 & 61.08\% \\
%             \quad \quad Reactive Domains (\textbf{R1,R2 \& R3}) & 3,197 & 1.90\% \\
%             % \quad \quad \quad Became Non Exclusive \quad \quad \quad & 1,361 & 0.81\% \\
%             % \quad \quad \quad Unsubscribed & 1,836 & 1.09\% \\
%             % \quad \quad \quad \quad Did Not Return & 1,315 & 0.78\% \\
%             % \quad \quad \quad \quad Returned & 521 & 0.31\% \\
%             % \hline
%             \bottomrule
%             \textit{*Active domains as per 20 October 2016.} & & \\
%             \textit{**Excluded from further analysis.} & & \\
%             \hline
%         \end{tabular}
%     }
%     \label{tab:domain_summary}
% \end{table}

% \begin{table}[]
%     \caption{Count of categorized domains by initial response.}
%     \setlength{\tabcolsep}{1pt}
%     \renewcommand{\arraystretch}{1.1}
%     \resizebox{.48\textwidth}{!}{%
%         \centering
%         \tiny
%         \begin{tabular}{lrrrr}
%             % \hline
%             \toprule
            
%             {Initial Status} &  Not reactive &  Became non exclusive &  Unsubscribed &   Total \\
%             % \hline
%             \midrule
%             Exclusive     &         85,449 &                  1,361 &          1,791 &   88,601 \\
%             Non Exclusive &         17,523 &                     0 &            45 &   17,568 \\
            
%             % \hline
%             \bottomrule
%             Total         &        102,972 &                  1,361 &          1,836 &  106,169 \\
%         \end{tabular}
%     }
%     \label{tab:domain_initial_response}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
%     \caption{Categorized domains by initial status and behavior.}
%     \setlength{\tabcolsep}{2pt}
%     \renewcommand{\arraystretch}{1.5}
%     \centering
%     \resizebox{.48\textwidth}{!}{%
%     \begin{tabular}{llrrrrrlr}
%     \hline
%     \multirow{3}{*}{\textbf{Initial Status}} & \multicolumn{6}{c}{\textbf{First Response}}                          & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Total}}} \\ \cline{2-7}
%      &
%       \multicolumn{2}{l}{\textbf{Not Reactive}} &
%       \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}To Non Exclusive\end{tabular}}} &
%       \multicolumn{2}{l}{\textbf{Unsubscribed}} &
%       \multicolumn{2}{l}{} \\ \cline{2-9} 
%      &
%       \textbf{\#Unique} &
%       \multicolumn{1}{l}{\textbf{\#Row}} &
%       \multicolumn{1}{l}{\textbf{\#Unique}} &
%       \multicolumn{1}{l}{\textbf{\#Row}} &
%       \multicolumn{1}{l}{\textbf{\#Unique}} &
%       \multicolumn{1}{l}{\textbf{\#Row}} &
%       \textbf{\#Unique} &
%       \multicolumn{1}{l}{\textbf{\#Row}} \\ \hline
%     Exclusive                                & \multicolumn{1}{r}{85,449}  & 89,277  & 1,361 & 1,471 & 1,791 & 1,915     & \multicolumn{1}{r}{88,601}         & 92,663         \\
%     Non Exclusive                            & \multicolumn{1}{r}{17,523}  & 18,198  & -     & -     & 45    & 50    & \multicolumn{1}{r}{17,568}         & 18,248         \\ \hline
%     Total                                    & \multicolumn{1}{r}{102,972} & 107,475 & 1,361 & 1,471 & 1,836 & 1,965 & \multicolumn{1}{r}{106,169}        & 110,911        \\ \hline
%         \multicolumn{9}{l}{\textit{\#Unique: number of unique domains; \#Row: total row after splitting multilabels;}} \\
%         % \multicolumn{9}{l}{\#Row: total row after splitting multilabels} \\
%         \hline
%     \end{tabular}%
%     }
    
%     \label{tab:categorized_domain_by_status}
% \end{table}



%
% \noindent
% \begin{minipage}[t]{\textwidth}
% \begin{minipage}[b]{0.49\textwidth}
% %\begin{figure}%[h]
%     \centering
%     \includegraphics[width=\linewidth]{figure/general_statistic.png}
%     \captionof{figure}{Number of active domains, the type of reaction, and the initial status per reaction type. Only a small fraction of non-exclusive domains reacted to the attack. A possible cause is the presence of backup service.}
%     \label{fig:domain_count}
% %\end{figure}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.49\textwidth}
% %\begin{figure}%[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figure/unreachable_statistic.png}
%     \vspace{0.5em}
%     \captionof{figure}{Number of reachable and unreachable domains by Zvelo. Some of the reachable domains are labelled with multiple categories. Hence, the number of unique domains are smaller than the number of rows in the dataset.}
%     \label{fig:unreachable_domains}
% %\end{figure}
% \end{minipage}
% \end{minipage}

% \todo[inline]{MJ: I think `unreachable' may confuse readers. In the paper's context, unreachable as the result of the attack is probably the first thing to come mind. Unreachable from a categorization lookup point of view is less obvious. Discuss with Abhishta, but if redoing the figures and rebranding these as `still existing' or `categorizable' or reasonable and still possible, I think it's worth considering.}
% \todo[inline]{MJ: what currently feels unresolved is the fact that the Zvelo lookups were done recently and for this reason some names are more likely to be not be categorizable 5 years after the fact.}

% \begin{table}[t]
%     \setlength{\tabcolsep}{3pt}
%     \renewcommand{\arraystretch}{1.5}
%     \centering
%     \resizebox{.7\textwidth}{!}{%
%         \begin{tabular}{llrrrr}
%             \hline
%             \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Domain \\ Status\end{tabular}}} &
%               \multicolumn{5}{l}{\textbf{Company Type}} \\ \cline{2-6} 
%              &
%               \textbf{Business} &
%               \multicolumn{1}{l}{\textbf{Hosting}} &
%               \multicolumn{1}{l}{\textbf{ISP}} &
%               \multicolumn{1}{l}{\textbf{Education}} &
%               \multicolumn{1}{l}{\textbf{Unknown}} \\ \hline
%             Exclusive     & \multicolumn{1}{r}{17,986} & 6,890 & 2,944 & 72 & 121 \\
%             Non Exclusive & \multicolumn{1}{r}{8,074}  & 1,970 & 559   & 12 & 15  \\ \hline
%         \end{tabular}%
%     }
%     \caption{Number of non-reactive domains by domain status and company type.}
%     \label{tab:non_reactive_domains}
% \end{table}

\subsection{Categorization of Dyn Customers}
%We identify nearly 168K domain names that were Dyn customers on the day prior to the DDoS attack.
%We obtain nearly 168K domain names which used at least one Dyn name server from the measurement data on the given day.
%We refer to this set of domain names as the initial set of domains (Table~\ref{tab:domain_summary}). 

We query category labels and reputation scores of the initial set of domains using a publicly available URL categorization service provided by McAfee ``Real-Time Database"~\cite{vallina_mis-shapes_2020}. % \textcolor{red}{Reference}. 
%We query the categories associated to these 168K domains at a non-intensive average rate lower than 40 reques. %We observe two findings from the domains categorization process: 
\noindent \textbf{$\approx$ 62\% of the domains were categorized by McAfee.} 
Some domain names are not yet categorized by McAfee, these are domains that are either no longer in operation or do not have enough features available for McAfee's classifier to make a deterministic classification.
%we did not obtain any category label from the service.
% Domain names which are no longer in operation or are not yet listed for categorization by McAfee could not be categorised. 
We refer to these domains as \textit{Un-categorized domains}. In this paper, we limit our analysis only to the domain names which were successfully categorized by McAfee, i.e., around 106K unique domains or nearly 62\% of all unique domains that used Dyn services one day prior to the attack (Fig.~\ref{fig:macro_flowchart}). 
% Among them, around 102K unique domains are non-reactive and only around 3K unique domains reacted.
% Table~\ref{tab:categorized_domain_by_status} presents a more detailed summary with additional information of their initial status and first response.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/Flowchart Domains.drawio.pdf}
    \caption{Dyn customer subdivision in category, domain status and reaction. We identify 169K customers and categorize per our methodology. We distinguish exclusive and non-exclusive domains and subdivide into reactions. For example, out of $\sim$17K non-exclusive domains, 45 unsubscribed following the attack, and 24 out of 45 did not return to Dyn later.}
    \label{fig:macro_flowchart}
\end{figure}

%\subsubsection{Multiple Category Labels}
%  \textbf{Domain names can be related to multiple categories.}
Some domain names are mapped to multiple industry sectors and risk groups by McAfee. We consider all retrieved category labels for our analysis. 
% \textcolor{red}{This approach aligns with our objective to focus on the relationship between sectors and post-incident responses.\textbf{, why?}} 
Hence, the total number of category labels retrieved for the domains are more than the total number of unique domains.%, as shown in Figure~\ref{fig:macro_flowchart}.

% \subsection{Summary of Domains Reactions}
% Our dataset now contains around 106K of categorized domains. 
We retrieve daily \textit{Domain Status} for all categorized domains from the measurement data for 20 days after the attack to observe status changes which can be used to capture \textit{Domain Movements} as discussed in Section~\ref{sec:methodology}.
%We identify two initial observations:

\noindent \textbf{The number of \textit{Non-reactive Domains} is significantly higher than \textit{Reactive Domains}.}
The number of \textit{Non-reactive Domains} is significantly higher than \textit{Reactive Domains} by a ratio of 32:1 (Fig.~\ref{fig:macro_flowchart}). 
%For \textit{Exclusive Domains}, this movement is particularly unusual since they were more probably to have a period of downtime when the incident happened.
We observe more \textit{Exclusive Domains} either becoming non-exclusive or unsubscribing to Dyn services as they have a greater probability of experiencing downtime due to the lack of redundancy in authoritative name servers.Whereas among non-exclusive domains, only 45 out of nearly 17K domains reacted. 
This is predictable since they had redundancy, hence, did not need to react.  
More than 85K out of $\approx$88K of \textit{Exclusive Domains} did not show any reaction (Fig.~\ref{fig:macro_flowchart}). This can be explained by the presence of cached \texttt{NS} records on DNS resolvers might keep several domains accessible during the outage~\cite{MouraIMC2018}.
% We expect to explain this behavior with additional data on domain characteristics in the next sections.


\noindent \textbf{The number of domains that became non-exclusive is not significantly different with the number of domains that unsubscribed.}
Reactive domains showed two types of movement in terms of their decision to become non-exclusive or to unsubscribe from Dyn (Fig.~\ref{fig:macro_flowchart}). 
Among 3,197 reactive domains, 1,361 became non-exclusive and 1,836 unsubscribed.
We observe that there is no clear preference in the type of movement among domains since the numbers are not significantly different.
This observation motivates us to zoom into domains with similar characteristics, i.e., in terms of popularity, expecting to discover specific preferences in the resilience strategy among similar Dyn customers.
% All 45 reactive \textit{Non-exclusive Domains} chose to unsubscribe from Dyn.
% We further discuss in the next sections the return behavior of these unsubscribed domains.

\subsection{Popularity Influence on Decision to React}
\label{sec:domain_popularity}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/reactive_by_alexa_rank_bin2.pdf}
    \caption{
        % Domains reactions in different groups of popularity. 
        % Groups indicate cumulative classification. 
        % For example, \textit{top1k} includes domains in \textit{top100}. 
        % The percentages represent the proportion of \textit{reactive} and \textit{non-reactive} domains in each group. 
        Reactions of Dyn customers -- reactive or non-reactive -- among different Alexa popularity groups. For example, among \textit{top100} Alexa customers, 42.9\% react to the attack. (Note that larger groups are supersets, i.e., the \textit{top100} are included in the \textit{top1k})
    }
    \label{fig:by_popularity}
\end{figure}


% \textcolor{red}{How many domains have an Alexa rank? [DONE]}
We then incorporate Alexa rank data into our data set to indicate how popular each domain is.
Out of $\approx$106K domains, we manage to retrieve popularity ranks of $\approx$5K domains that belong to the Top 1M Alexa list and ignore the ones which do not.  
% \textcolor{red}{get numbers for categorized only, change to active voice [DONE]}
% We ignore domains outside the Top 1M Alexa lists.
We observe that domains with higher Alexa rank have a higher proportion of reactive domains (e.g., 42.9\% in top100) compared to those with lower rank (e.g., 14.3\% in top1m) as shown in Fig.~\ref{fig:by_popularity}:
the percentage of reactive domains decreases as more domains with lower rank are included.
Popularity of the domains is thus one factor that might influence the decision to react.

A higher rank means a higher traffic to these domains which may result in a higher revenue~\cite{truong_relationships_2018}.
Hence, owners of domains with higher rank will prefer minimizing downtime of their domains to avoid revenue loss. Meanwhile, owners of domains with lower rank may not very sensitive to short-term downtime.
Some reactions involve an extra cost, e.g., using multiple DNS service providers, which may not be worthwhile for businesses with smaller revenue.



%To describe how popularity may affect the domains reactions, we include Alexa rank data of the domains in our further analysis.
%We attach \textit{mean Alexa rank} of domains in a certain group to indicate \textit{how popular the domains are on average}.
% We also compute the \textit{coefficient of variation} as the ratio between the sample standard deviation and mean~\cite{everitt_cambridge_1998} for ranks of domains within each industry sector to analyze the impact of website popularity on the decision of domains to chose a resilience strategy.
% 

\ 

\noindent
\textit{\textbf{Key takeaway}: We observe that customers running domains for more popular websites (based on Alexa rank) reacted to the attack with higher probability.}
%\noindent\fbox{%
    %\begin{minipage}{0.95\linewidth}
    %\textit{\textbf{Key takeaway}: Comparing the Alexa ranks of the domains that react and do not react to the %attack, we observe that those with a higher website popularity (lower Alexa ranks) have a greater probability %of reacting to the outage.}
    %\end{minipage}}
% These two metrics assist in determining whether the behavior is strongly influenced by popularity of domains.

% How domains with higher Alexa rank behave differently with domains with lower Alexa rank. Mention how many domains with rank and without rank. 

% Plot: histogram of popularity index

% Plot: bar chart behaviors by binning




% We later discuss in depth the behaviors of domains in these selected categories in Section~\ref{sec:domain_sector}.
% Each category has various number of domains labeled with. 

% \textcolor{red}{The following discussion section needs updating of structure and content}
% 
% 
% 
% \textcolor{red}{A paragraph on methodology will be nice to manage expectations.It will make it clear why statistical test is used to select important industry sectors.}
% 
% 

% We now discuss the behavior of categorized domains from three perspectives: 1) to react or not, 2) to become non-exclusive or to unsubscribe; 3) to return after unsubscribing or not.

% \subsection{Overall Behavior}
% 
% First we discuss about the overall behavior of the active domains which were using Dyn DNS service during the incident as summarized in Table~\ref{tab:categorized_domain_by_status}. 
% 
% \begin{observation}
%     The proportion of reactive domains are relatively small ($\approx$3K domains) compared to non-reactive domains ($\approx$102K domains), despite many of them ($\approx$85K domains) were critically dependent on Dyn DNS service.
% \end{observation}
% 
% \begin{observation}
%     Only a tiny fraction (45 domains) of $\approx$17K non exclusive domains reacted by unsubscribing from Dyn.
% \end{observation}
% 
% 
% 
\subsection{Industry Sector Influence on Decision to React}
\label{sec:stat_analysis}
% Content:
% \begin{itemize}
%     \item Define dependent variables: 4 types of reactions @ 1 model
%     \item Define independent variables: 4 aspect of domain characteristics
%     \item Explain why choose logistic regression
%     \item Present the result in a table
%     \item Mention selection for industry sector selection
%     \item Explain how to interpret the result using example
% \end{itemize}


% \textcolor{red}{How? There are 106K unique domains? We should only talk about unique domains throughout the paper.}
% This result shows that each category is significantly different in terms of the number of domains.
% Considering the space limitation, we cannot discuss all 94 categories in depth.
%\textcolor{red}{Even if we had space we would not have talked about 94 categories.} 
 

%We make use of a multivariate logistic regression model to determine the impact of individual industry sectors on domain reactions (\textbf{R0} vs \textbf{R1}, \textbf{R2} \& \textbf{R3}).
%We then perform a regression analysis to measure correlations between each category to domain reaction.

We obtain nearly 106K labeled domains with 94 unique categories from the categorization process. We discuss in more detail the Industry Sectors that had a significant impact on the resilience strategy adopted by the domain managers. 

To determine the impact of individual industry sectors on domain reactions, we model the resilience strategy adopted by the domains as a function of their industry sector using a multivariate logistic regression analysis. We model the binary decision of domains to react (react: \textbf{R1}/\textbf{R2}/\textbf{R3} or not react: \textbf{R0}) as a dependent variable (\ref{eq:logit_decision}). 

\begin{equation}
\label{eq:logit_decision}
    \text{\textit{logit}}(\pi_{b})=\log[\frac{\pi_{b}}{1-\pi_{b}}],
\end{equation}

\noindent where $\pi_{b} \in [0,1]$ represents the probability of a domain reacting and can be estimated using (\ref{eq_logit_estimation}).

\begin{equation}
    \label{eq_logit_estimation}
    \pi_{b}=\frac{\beta_{0}+\sum_{i}^{}\beta_{i}x_{i}}{1+(\beta_{0}+\sum_{i}^{}\beta_{i}x_{i})},
\end{equation}

\noindent where $x_{i} (i=1,2,3,....,94)$ represents each industry sector as a separate independent variable. $x_{i}$ has a value of 1 if a domain belongs to this industry sector, otherwise it has a value of 0. $\beta_{i}$ is the odds ratio and signifies the strength of correlation between this independent variable and the dependent variable. In this analysis, $\beta_{i}$ shows the factor with which an industry sector $i$ will increase the probability of a domain to react. To implement logistic regression, we use \texttt{statsmodels} package in python~ \cite{seabold2010statsmodels}.
% Explain the motivation of GLM use


%The reason of this specific choice of model is due to the binary identity of the dependent variable i.e., react or not react, and the independence between domain decisions to react.
%\textcolor{red}{[OPTIONAL] The predicted value of the regression model is the probability of a domain labeled with certain categories to react after the attack.}
% option A
%We define $Y_d$ as the decision of domain $d \in D$ after the attack with $D$ being all categorized domain names of Dyn customers.
%$Y_d$ is 1 if domain name $d$ changes its Domain Status at least once after the attack and 0 if otherwise.
% We transform the category labels given to each domain using one-hot-encoding resulting in dummy variables that we use as our independent variables ($X$).
% Option B
%Our independent variables, $X$, are a set of $X_c$, which equals to 1 if a domain is labeled by category $c \in C$ with $C$ being 94 unique categories, and 0 if otherwise.
% 
%For the regression model to converge, we eliminate categories that have only 1 domain due to low variance.




The regression model outputs three main metrics to indicate the influence of each category as Table~\ref{tab:stat_result} shows.
\textit{Coefficient} ($\beta_{i}$) indicates the fraction by which the probability of a domain reacting to the attack increases, if this domain belongs to Industry Sector $i$  i.e., the more positive the coefficient is, the higher the influence.


\begin{table}[t]
    \centering
    \caption{GLM coefficients for domains showing most prominent industry sectors that had a statistically significant influence on domain reactions (ordered by the number of domains in each industry sector).
    %\textcolor{red}{The selected categories changed. So we need to change the plot too?(DONE)}
    }
    \label{tab:stat_result}
    
   \begin{tabular}{lrr}
\toprule
Industry Sector&    Coefficient\textsuperscript{*} &       z-value \\
\midrule
Internet Services                    &  0.47 &   6.80 \\
Travel                               &  1.25 &  14.61 \\
Content Server                       &  1.26 &  11.00 \\
Motor Vehicles                       &  0.78 &   6.26 \\
General News                         &  2.17 &  24.05 \\
Job Search                           &  1.30 &   9.40 \\
Streaming Media                      &  2.15 &   6.57 \\
Gambling                             &  1.60 &   8.97 \\
Portal Sites                         &  1.74 &   6.51 \\
PUPs (potentially unwanted programs) &  2.83 &  12.28 \\
Malicious Sites                      &  2.61 &   8.91 \\
Social Networking                    &  2.47 &   7.75 \\
Personal Pages                       &  1.87 &   5.37 \\
Provocative Attire                   &  2.71 &   4.86 \\
For Kids                             &  3.07 &   4.93 \\
Interactive Web Applications         &  2.61 &   7.97 \\
Weapons                              &  1.98 &   5.32 \\
Professional Networking              &  3.58 &   9.34 \\
Visual Search Engine                 &  4.12 &   7.42 \\
Instant Messaging                    &  4.03 &   5.32 \\
        \bottomrule
        \textit{\textsuperscript{*}p$<$0.001}
    \end{tabular}
\end{table}
%We compare industry sectors to  one is more likely to react following an outage incident.
For example, domains in the \textit{Professional Networking} with coefficient value 3.58 are more likely to react than domains in the \textit{Motor Vehicles}, such as web sites of car manufacturers and sales, with coefficient value 0.78.
Hence, we expect the proportion of reactive domains is higher in the former than the latter.
\textit{p-value} indicates if the coefficient of a domain is statistically significant or not. 
% A \textit{p-value} lower than 0.01 means that ...
\textit{z-value} tells us how many standard deviation the average decision of a certain industry sector is away from the average decision of the whole data set~\cite{mcleod_z-score_2019}. It indicates the reliability of the coefficient computed by the logistic regression model.
% The larger the z-value is, the more distinct the behavior of domains with certain industry sector is, compared to the behavior of all domains. 
%Domains in a category with a higher \textit{z-value} are more concentrated on a specific decision, compared to those with a lower \textit{z-value.} 



We discuss the type of reactions observed of those domains that belong to any of the top 20 industry sectors whose coefficient was both highly reliable (greater than the median \textit{z-value} as shown in Fig.~\ref{fig:z_hist}) and statistically significant (\textit{p-value} $<0.05$).

% In Section~\ref{sec:domain_sector}, we show how domains in these selected industry sectors reacted after the incident.
% 
% \textcolor{red}{To add: cdf of p and z value, negative significant influence}
% 

% \begin{figure}[hbp]
%     \centering
%     \includegraphics[width=\linewidth]{figure/z_value.png}
%     \caption{Distribution of z-values (signifies reliability) for industry sector coefficients in the linear regression model. We discuss in more detail the reactions of domains that belong to industry sectors, which according to the logistic regression model had a reliable and statistically significant impact on the reactions.}
%     \label{fig:z_hist}
% \end{figure}
The results indicate that a number of categories have more significant correlation to the resilience strategy than the others.
Domains in industry sectors with higher coefficient have a higher probability to react following outages, such as \textit{General News} and \textit{Streaming Media}. 
DNS providers should anticipate the reaction from their customers in these industry sectors more than other sectors.
% We then particularly discuss a number of industry sectors with statistically significant positive influence on the decision to react to be discussed further.
% % \textcolor{red}{Our results show $>$20 sectors with coef$>$0 and p-value$<$0.01. We select only top 20 due to space limitation?}
% We retrieve sectors with significant p-values and choose the top 20 sectors with the highest z-values as shown in Table~\ref{tab:stat_result}.
% We limit our industry sector analysis to selected categories with statistically significant influence on the decision to react.
% 

\ 

\noindent
\textit{\textbf{Key takeaway:} By using a multivariate logistic regression model, we were able to calculate and reveal that for 34 out of 94 industry sectors, there is statistically significant influence on the post-attack reaction.}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} Using a multivariate logistic regression model, we calculate the impact of industry sectors on the reactions of domains to the attack. 34 out of 94 industry sectors (20 of which are shown in Table~\ref{tab:stat_result}), have some statistical influence on the post-attack reaction of the domains.}
   % \end{minipage}}

\ 

% \textcolor{red}{See my comment on teams.}
% \todo{see my comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/z_value.png}
    \caption{Distribution of z-values (signifies reliability) for industry sector coefficients in the linear regression model. We discuss in more detail the reactions of domains that belong to industry sectors, which according to the logistic regression model had a reliable and statistically significant impact on the reactions.}
    \label{fig:z_hist}
\end{figure}

We also observe a number of industry sectors which \textbf{do not} have statistically significant influence on the decision to react such as \textit{Religion}, \textit{Ideologies}, and \textit{Politics}.
Religion and Ideologies sectors include web pages that discuss spirituality and beliefs while Politics domains discuss about political parties, views, and opinions.
We might indicate that domains in these sectors do not require high resilience.

\ 

\noindent
\textit{\textbf{Key takeaway:} Some industry sectors do not seem to have a statistically significant influence on the decision to react after the attack.}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} Some industry sectors such as Religions and Politics do not seem to have a statistically significant influence on the decision to react after the attack. Hence, in these cases the likelihood of domains reacting is equal to random.} 
   % \end{minipage}}

\



% \subsection{Domain Behaviors by Industry Sectors}
%\label{sec:domain_sector}
%We define domain reaction as \textit{the first movement following the incident}. Moreover, we define returning movement as \textit{the first returning movement after it stopped using Dyn service} i.e., the status changed from not customer to customer, either as exclusive or non-exclusive.



We zoom into a number of significantly influential industry sectors (Table~\ref{tab:stat_result}).
Fig.~\ref{fig:reactions_by_category} shows how domains in these industry sectors reacted.
The \textit{top plot} shows proportions of reactive domains in each industry sector, characterized by their decision to become non-exclusive or to unsubscribe after the attack.
The diminishing line in the top plot indicates the size, i.e., number of domains, of each industry sector on a $log_{10}$ scale.
We observe that sector size do not indicate a direct correlation with the proportion of reactive domains in the sector.
However, we demonstrate that the reactions vary among industry sectors in two ways: proportion of the reactive domains and the dominant type of reactions.



% 1
From the \textit{top plot} in Fig.~\ref{fig:reactions_by_category}, we show that majority of domains in some industry sectors \textbf{became non-exclusive} following the incident, i.e., used additional DNS providers, such as domains in \textit{General News}, \textit{Potentially Unwanted Programs (PUPs)}, \textit{Malicious Sites}, and \textit{Visual Search Engine}.
Domains in \textit{PUPs} and \textit{Malicious Sites} categories are made with intention to infect user's computer with software or script to hijack or alter security and privacy, e.g., Trojan horses and viruses.
Domains in \textit{Visual Search Engine} include web pages that provide searching functionality with image-specific results.
The reaction to use multiple DNS services might indicate that these domains have a high -- most probably financial -- value for the owners, hence, it is important to keep them up at all times.
After the attack, they used back-up services to make their domains more resilient against future outages.
Therefore, we assume that the revenue from the domains is large enough to compensate the cost of using extra DNS service, if present.

% 2
Meanwhile, domains in some industry sectors show a significant preference to \textbf{unsubscribe}, i.e., stop using Dyn service, after the attack (Fig.~\ref{fig:reactions_by_category}).
% We group industry sectors with such preference into two groups.
Among them, we observe domains intended for adult audience
% 1
% First, domains with content for adult audience 
such as \textit{Gambling} sites, web pages about \textit{Weapons}, and sites showing \textit{Provocative Attires}, 
and domains intended for 
% 2
% Second, domains for 
more general audience such as \textit{Motor Vehicles} sites, \textit{Streaming Media}, and \textit{Social Networking} sites.
The reaction to unsubscribe after the attack might also indicate that domain owners value their domains and find it necessary to react after the attack.
However, we suspect that the cost of using a secondary DNS service is not worth the revenue from the domain or the owner considers Dyn no longer reliable.

\begin{figure}[]
    % \centering
    \includegraphics[width=\linewidth]{figure/plot_sector_v5_with_swarm.pdf}
    \caption{
        Behaviors of domains in selected industry sectors.
        \textbf{Top Plot} shows the proportions of domains with different reactions in each sector along with the sector sizes.
        \textbf{Middle Plot} shows the proportions of unsubscribed domains that did not return.
        % \textbf{Bottom Plot} shows the mean and variation of Alexa rank of domains in each sector.
        \textbf{Bottom Plot} shows the distribution of Alexa ranks among domains that belong to a certain industry sector.
    }
    \label{fig:reactions_by_category}
\end{figure}
\

\noindent
\textit{\textbf{Key takeaway:} We see a difference in the type of reaction based on the industry sector. In some sectors, domains for the most part became non-exclusive following the attack (e.g., \textit{General News}), while for others, customers largely unsubscribed (e.g., \textit{Gambling}).}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} We analyse the type of reactions observed for the domains in selected industry sectors (Fig.~\ref{fig:reactions_by_category}). We see a difference in the type of reaction based on the industry sector: In some sectors such as \textit{General News}, domains predominantly became non-exclusive following the attack, while some others such as \textit{Gambling} domains tend to unsubscribe.} 
   % \end{minipage}}
% [DELETE] This number reflects the relative importance of keeping the domain operational from the perspective of domain owners. 
% [DELETE] A higher proportion in certain type of decision might reflects the risk appetite of the domain owners, especially because each type of reaction has different risk level (Section~\ref{sec:key_concepts}). 

\ 

In the \textit{middle plot}, we show the proportion of return among domains that unsubscribed in each sector.
This metric is particularly important to measure business impact of an outage incident as it indicates how many customers that the provider loses for a longer term.
In some industry sectors such as \textit{Travel} (e.g., ticketing sites), \textit{Motor Vehicles}, and \textit{Personal Pages} (e.g., blogs), domains that \textbf{did not return} are significantly more than those which \textit{returned}.
On the contrary, the behavior is quite the opposite in \textit{Gambling}, \textit{PUPs}, and \textit{Malicious Sites} sectors, i.e., most of unsubscribed domains returned later.
In \textit{Visual Search Engine} sector, there is no domain that unsubscribed, hence, no data shown in the plot.
% This number might reflect the relative tolerance of domain owners against service failure by the provider.
% High proportion of domains which did not return might indicate low tolerance among the domain owners e.g., due to trust loss. 
% On the other hand, domains that returned might still consider Dyn as a trustworthy provider or already have a good relationship with Dyn.

\ 

\noindent
\textit{\textbf{Key takeaway:} In some industry sectors, domains that unsubscribed mostly did not return (e.g., \textit{Travel}), while in others, a higher proportion of domains unsubscribed and returned (e.g., \textit{Gambling}). This suggests that the industry sector affects decision-making.}

%\noindent \fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} In some industry sectors, such as Travel, most domains that unsubscribed after the attack did not return, while in some other sectors, such as \textit{Gambling}, a higher proportion of domains returned. This shows that for some sectors, the chance of customers leaving for a longer term is higher. Domains belonging to \textit{visual search engine} category only used becoming non-exclusive as a resilience strategy.} 
   % \end{minipage}}

\ 

% [Still working] 
The \textit{bottom plot} in Fig.~\ref{fig:reactions_by_category} shows the distribution of Alexa ranks -- where present -- among all domains in each industry sector characterized by their responses after the attack i.e., reactive or non-reactive. 
This plot provides insight into the influence of popularity on the choice of resilience strategy adopted by domains in each industry sector.
% 
%\textcolor{red}{There are a number of domain categories that are in Fig 4 but we never talk about in the text. Why?}
% The latter metric indicates how diverse the Alexa ranks are within that category.
% For example, most domains in \textit{Job Search} sector have higher Alexa ranks i.e., more popular, than domains in \textit{General News}, but more uniform i.e., have similar popularity.
%For example, in \textit{Job Search} and \textit{Gambling} categories, Alexa ranks of domains that reacted (dark box plot and light dots) are more concentrated in the lower plot (shorter box), indicating a higher popularity, compared to those which did not react (light box plot and dark dots) which are more dispersed (longer box) and, in majority, less popular.
For most industry sectors shown in Fig.~\ref{fig:reactions_by_category}, we observe that the average popularity of reactive domains is higher than the average popularity of non-reactive domains. This is consistent with our previous discussion in Section~\ref{sec:domain_popularity} that higher popularity influences the domain decision to react.
However, we see that popularity was a more significant factor for some industry sectors than the others. \textbf{Non-overlapping} boxes in \textit{Job Search} and \textit{Gambling} sectors indicate a strong correlation between popularity and the decision to react.
Meanwhile, in some industry sectors such as \textit{Internet Service}, domain popularity does not seem to have a strong correlation with the decisions to react, considering that the distributions of Alexa ranks are rather similar between reactive and non-reactive domains, indicated by \textbf{overlapping} boxes.
% Therefore, a \textit{high mean} of Alexa rank with \textit{low coefficient of variation} indicates that the domain popularity plays significant role in the decisions to react such as domains in \textit{Weapons}, \textit{Provocative Attires}, and \textit{For Kids}.

\ 

\noindent\textit{\textbf{Key takeaway:} In some industry sectors (e.g., Job Search), the influence of popularity on the decision to react is stronger than the others (e.g., Internet Service).}
%\noindent \fbox{%
    %\begin{minipage}{0.95\linewidth}
%    \textit{\textbf{Key takeaway:} The popularity of domains in some industry sectors with high and similar Alexa ranks such as Job Search might have a significant influence on the decisions to react after the attack.} 
%    \end{minipage}}
% 
% We make a couple of further observations regarding domains in the selected categories.  
% % Figure~\ref{fig:reactions_by_category}.
% % 1
% Domains in \textit{Potentially Unwanted Programs (PUPs)} and \textit{Malicious Sites} categories predominantly became non-exclusive following the incident, and none of unsubscribed ones that did not return.
% In addition, we could see that none of domains in these two categories belong to Top 1M Alexa list. This is predictable since malicious websites are rarely found in top Alexa list~\cite{kim_malicious_2018}.
% % domain examples
% Domains in these categories are made with intention to infect user's computer with software or script to hijack or alter security and privacy, e.g., Trojan horses and viruses.
% % 2
% % 3
% Domains for adult audience i.e., \textit{Gambling}, \textit{Weapons}, and \textit{Provocative Attire}, predominantly unsubscribed after the incident. 
% However, in \textit{Gambling} sector, only 20\% that did not return.
% In addition, Alexa rank mean and variation for the other two sectors indicate that domains in these sectors are homogeneously quite popular and suggest a strong influence on the reaction.
% % example
% Domains in Gambling sector include web pages that allow users to place bets online.
% Domains in Weapon sector include web pages that provide every information about weapons, including buying, for either personal or military use.
% Meanwhile, domains in Provocative Attire sector include web pages showing non-nudity revealing attires intended to provoke the viewers. 
% \newline \newline \textit{\textbf{Key takeaway:}} \newline
% 
% % 4
% Domains in \textit{General News} predominantly became non-exclusive but more than 82\% of unsubscribed ones did not return.
% Furthermore, this behavior is less likely to be influenced by domain popularity due to a high diversity in their Alexa rank.
% % domain example
% Domains that belong in this category include news portals, both regional and international.
% % 
% Domains in \textit{Professional Networking} and \textit{Social Networking} show a similar behavior.
% Most of them unsubscribed then did not return which might indicate low tolerance against violation in service fulfillment.
% % example
% Domains in this category include social networking for professional use and friendship focus. 
% % 5
% Lastly, domains in \textit{Visual Search Engine} sector only reacted by becoming non-exclusive, hence, no data about their return behavior.
% % example
% This category includes web pages that provide searching functionality with image-specific results.


% \begin{observation}
%     Majority of reactive domains in Sport sector unsubscribed from Dyn but majority of them returned.\textcolor[red]{Too anecdotal. Maybe for most observations it is better to talk in terms of how Industry sector as a factor explains the decision taken by domain owners.}
% \end{observation}

% Discussion here.

% \begin{observation}
%     In Marketing/Advertising, Online Shopping, and Entertainment sectors, there were more reactive domains that unsubscribed than those which stayed. More than 80\% of those which unsubscribed did not return.
% \end{observation}

% Discussion here.






% \textbf{Reactive or Not reactive:\ }

% \textbf{Become Non Exclusive or Unsubscribe:\ }
% There are two likely reactions that a domain owner could take following the outage incident: to become non-exclusive or to unsubscribe. We observe that the proportion of these two reactions varies among different types of domain. 
% For example, domains in Finance, e.g., banks and loans, mostly chose to leave Dyn while domains in Business e.g., trading companies, mostly chose to keep using Dyn but became non-exclusive i.e., use managed DNS service from other providers following the incident (Figure~\ref{fig:first_reaction_industry}). 
% % One possible explanation is that domains in Finance are easier to lose trust following the incident. 
% This behavior is consistent with the fact that finance-related domains are more trust sensitive.
% It is likely that they require highly reliable partners to support their operation and less tolerant with service failure.

% In contrast, the intended use of the domains did not correlate with its reaction, as shown in Figure~\ref{fig:reaction_by_purpose}. Most domains reacted by stop using the service regardless their intended uses.

% \todo[inline]{MJ: Does proportion mean ratio/fraction? Does it mean numbers? The table 2 caption mentioned the word proportions before, but table 2 only tabulates numbers. The numerical metrics speak of proportions and there it seems to be about fractions. Here you are not giving fractions, but you do seem to compare absolute numbers from two reactivity classes (nonex and noncust). Please be consistent/avoid ambiguity.}

% 
% \begin{figure}%[ht]
%      \centering
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/first_reaction_by_purpose2.png}
%          \caption{ }
%          \label{fig:reaction_by_purpose}
%      \end{subfigure}
%      \hspace{1em}
%     %  \hfill
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/windowed_departing_domains_by_purpose.png}
%          \caption{ }
%          \label{fig:returning_by_purpose}
%      \end{subfigure}
%         \caption{Reaction (a) and return movement (b) by intended use }
%         \label{fig:by_purpose}
% \end{figure}

%\subsubsection{React Immediately or Later.}
% \textbf{React Immediately or Later:\ }
% Another aspect that reflects the importance of DNS service availability for businesses is immediacy of the reaction. 
% % As discussed in Section~\ref{sec:mdns_business}, DNS service could be a key service in certain digital businesses, especially those who rely on Internet-based systems. Each second of downtime could cost them millions of dollar. For these type of businesses, they need to react immediately to return the availability of their systems. On the other hand, other businesses could react later because every second of downtime does not cost them much. 
% From the data, we observed that most domains in Finance reacted later than most domains in Business and News Portal. 
% Figure~\ref{fig:finance_late_response} shows that most domains in the financial sector reacted after the end of the month, while domains in more general categories mostly reacted immediately i.e., the next day following the incident. Despite the late reaction, almost all domains in the financial sector reacted by leaving Dyn. Meanwhile, we observe that domains in News category which left Dyn reacted immediately, but those which became non-exclusive reacted later in similar number. Hence, we may conclude that most domains in Finance sector might not suffer a great loss for each second of DNS unavailability but still lost their trust with the provider. Another possible explanation regarding this behavior is because the contract ended at the end of the month. Therefore, it is more efficient to wait until the previous contract ends before starting to use and pay for another service.

% Based on intended uses, similar proportions of domains that mainly provide service reacted on two specific days: day +1 and day +12. Further analysis is required to discover what type of services these domains provide to explain the difference. Domains that provide information and network reacted similarly i.e., immediately left after the incident, as shown in Figure~\ref{fig:reaction_time_by_purpose}.

%\subsubsection{Return or Leave for Good.}
% \textbf{Return or Not:\ }
% The third aspect that we analysed is the return movement among domains in different industry sectors. 
% % Previously, we have discussed that most domains in Finance chose to left Dyn, despite their late response.  
% We found out that most domains in Finance not only leave Dyn but almost all of them left for good. 
% Compared to other industry sectors, the proportion of Finance domains that left for good is much higher (Figure~\ref{fig:departing_by_industry}). 
% This fact supports our belief that domains in Finance are less tolerant of service failure thus prefer to leave and switch to other service providers. Based on intended use, we found no obvious difference in the proportion of domains that returned after they left, as shown in Figure~\ref{fig:returning_by_purpose}.  

% \begin{figure}[p]
%     \centering
%     \begin{subfigure}[b]{0.85\textwidth}%[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_time_to_react_finance.png}
%     \caption{\textbf{Time to react by industry sector.} Despite the tendency to leave instead of becoming non-exclusive, most domains in Finance (top) left Dyn after end of the month (a), while most domains in Business (middle) and News, Portal, and Search categories (bottom) left Dyn immediately i.e., the next day after the attack (b and c).}
%     \label{fig:finance_late_response}
% \end{subfigure}
% % 
% \begin{subfigure}[b]{0.85\textwidth}%[H]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_time_to_react_by_purpose.png}
%     \caption{\textbf{Time to react by intended use.} Most domains that provide service reacted by leaving Dyn. Many domains in this category left after end of the month (a), while in the other two categories, only a few left later.}
%     \label{fig:reaction_time_by_purpose}
% \end{subfigure}
% % 
% \begin{subfigure}[b]{0.85\textwidth}%[H]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_departing_domains_by_industry.png}
%     \caption{\textbf{Behavior of leaving domains by industry sector}. Majority of leaving domains in the Finance category did not return.}
%     \label{fig:departing_by_industry}
% \end{subfigure}
% \caption{Behaviour of domains for selected industry sectors.}
% \label{fig: behaviour of domains}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=.5\textwidth]{figure/plot3_behavior_by_functional_type.png}
%     \caption{Domain behaviors by different reactions across functional types.}
%     \label{fig:reactions_by_functional}
% \end{figure}

% \begin{observation}
%     Among reactive domains with Information/Communication function, there were more domains that stayed (4.2\%) than those which unsubscribed (2.2\%). Nevertheless, 81.8\% of those which left did not return.
% \end{observation}

% Information/Communication e.g. general news, search engine, and online forum.

\subsection{Risk Level Influence on Decision to React}
\label{sec:domain_risk_level}

%\textcolor{red}{Number of unverified, medium and high risk level websites are very low. Do comment on the aggregate numbers of these websites. How many are these?}

% Explain briefly about methodology to determine risk level.
% \textcolor{red}{
%     Discuss:
%     \begin{itemize}
%         \item DONE Only a few domains in unverified, medium, and high risk $\xrightarrow{}$ most Dyn consumers are legitimate domains
%         \item DONE Discuss med and hi risk domains, why use Dyn? why use redundancy? why return? $\xrightarrow{}$ premium crimes which needs hi availability.
%         \item DONE Discuss med hi risk domains with domains in PUPs and Malicious. compare behavior $\xrightarrow{}$ what it means?
%         \item In risk group, compare domains in security risk with domains in med and hi risks
%     \end{itemize}
% }

% Join two plots together using shared y axis!
We then analyze how risk level of the domains influence their reaction following the attack.
Fig.~\ref{fig:reaction_by_risk_type} shows behavior of domains with different risk profile, characterized by risk level and risk group.
Recall that McAfee categorizes domains based on the reputation score into four risk levels as shown in Section~\ref{sec:methodology}.
% \textit{Risk Level} is individually measured for each domain based on its reputation score~\footnote{See \url{https://trustedsource.org/download/ts_wd_reference_guide.pdf}}. 
% \textit{Unverified} refers to the level of risk which lies between minimal and medium risk.
We show that domains in Minimal Risk significantly outnumber domains in other risk levels. Out of 106K domains of Dyn customers, 104K are in Minimal Risk while domains in Unverified, Medium Risk, and High Risk categories only account for 2K domains (Fig.~\ref{fig:reaction_by_risk_type}).
% \textcolor{red}{add the exact number DONE}
This indicates that majority of Dyn customer domains were relatively safe to visit.

\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{figure/plot_risk_combined3.3_with_swarm.pdf}
    \caption{
    Behaviors of domains with different \textit{Risk Levels} and \textit{Risk Groups}. 
    \textbf{Top Plot} shows the proportions of domains with different reactions in each group along with the group sizes. 
    \textbf{Middle Plot} shows the proportions of unsubscribed domains that did not return. 
    \textbf{Bottom Plot} shows the distribution of Alexa ranks among domains that belong to a certain group.
    % Domain behaviors by different reactions across different \textit{Risk Levels} and \textit{Risk Groups}.
    % \textcolor{red}{Risk Type -- Risk Group}
    }
    \label{fig:reaction_by_risk_type}
\end{figure}

Some domains with higher risk levels also need high availability, hence, using the managed DNS service from Dyn.
As illustrated by the \textit{top plot} in Fig.~\ref{fig:reaction_by_risk_type}, some Dyn customers are domains in \textit{medium} and \textit{high risk} levels and they show a similar preference, namely, to become non-exclusive after the attack, i.e., use redundant DNS services.
Moreover, majority of the domains with medium and high risks returned if they unsubscribed, (the \textit{middle plot}).
% This observation reflects the resilience strategy of some malicious domains -- most probably with high revenue -- which demand higher availability from premium and redundant DNS services.
We also observed this \textit{exact} behavior among domains intended to victimize the users, e.g., PUPs and Malicious Sites, as discussed in Section~\ref{sec:stat_analysis}.
% 
% We make a couple of observations with regards to Risk Level influence on the domains reactions.
% 1
% Domains with \textit{medium} and \textit{high risk} level show a similar behavior, namely, they predominantly became non-exclusive. Furthermore, none of those which unsubscribed did not return. 

% 2
With regards to domain popularity, we indicate no domain with high risk belonged to Alexa Top 1M list as the \textit{bottom plot} in Fig.~\ref{fig:reaction_by_risk_type} shows.
This observation is again consistent with our result in Section~\ref{sec:stat_analysis} about malicious domains.
We demonstrate that some domains with medium risk are relatively quite popular (concentrated in the lower area) reflecting that some visitors unknowingly risk their security by regularly accessing the domains.

\

\noindent
\textit{\textbf{Key takeaway:} Customers with higher risk levels mostly became non-exclusive after the attack and the majority of those who unsubscribed instead also later returned.} 
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} Domains with higher risk levels mostly became non-exclusive after the attack and majority of those who unsubscribed returned later.} 
   % \end{minipage}}

\ 

% Moreover, there is another conclusion we could infer about domains with minimal risk from Figure~\ref{fig:reaction_by_risk_type}.
% 3
%\textcolor{red}{The word "active" needs to be removed everywhere.}
In addition, considering the \textit{top} and \textit{middle plots} in Fig.~\ref{fig:reaction_by_risk_type}, we observe that majority of the domains with minimal risk stopped using Dyn service permanently following the attack, namely, nearly 1K domains or 71.4\% of those which unsubscribed did not return.
This number indicates a relatively major business impact (i.e., losing nearly 1K customers) that Dyn suffered following the outage.
Other DNS providers could use this proportion to help estimate customer loss following an outage.
%\newline \newline \textit{\textbf{Key takeaway:} Legitimate domains have a relatively high tendency not to return once they unsubscribe from the DNS service after an outage.}

\ 

\noindent
\textit{\textbf{Key takeaway:} Our results show that if domains in the minimal risk category unsubscribe, the probability that they stay away for a longer time is higher.}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth} \textit{\textbf{Key takeaway:} There is a greater probability for domains in the minimal risk category to stop using Dyn for a longer term if they unsubscribe.}
  %  \end{minipage}}
    
\subsection{
% [Still working] 
Risk Group Influence on Decision to React}
\label{sec:domain_risk_type}

%\textcolor{red}{Structure suggestion:Recall definition of a category and discuss the types of websites that will fall in the category. Discuss how different is the reaction to other risk groups (See top plot). Discuss return behaviour (second plot). Do only popular websites move; or do all websites have similar likelihood of moving? Repeat for the next category. Note that in the documentation, it is "risk group" not "risk type".[DONE]}

% Category labels from the URL categorization service indicates the functionalities of the domains based on their content (if present).
% When used improperly, domains with certain functionalities might lead to unintended situations and negatively impact businesses or individuals.
% McAfee classifies URL categories into \textit{Risk Groups} based on which main aspect is the most at risk when this unintended situation happens.
% According to the documentation,
% \textit{Risk Group} refers to the main aspect which domains in certain category i.e., industry sector, might risk.
% For example, domains with \textit{Productivity} risk are non-business related which might reduce one's productivity at work e.g., social media and entertainment portal.
% Another example, domains with \textit{Bandwidth} risk are mainly web pages whose contents require a large amount of bandwidth to retrieve e.g., video streaming portal, hence, might disrupt business related communication over the network. 

We make a couple of observations from Fig.~\ref{fig:reaction_by_risk_type} regarding reactions among domains in different Risk Groups.
% 4
According to the \textit{top plot}, domains with \textit{Liability}, \textit{Communications}, and \textit{Propriety} risks show preferences to unsubscribe after the attack.
% 3
Meanwhile, as shown in the \textit{middle plot}, we observe similar return behaviors of domains in different risk groups, namely, more than half of them did not return after they unsubscribed, except domains in \textit{Security} risk group.

% 5
% Regarding domain popularity illustrated by the \textit{bottom plot}, even though the mean Alexa rank of each risk group is similarly high, but popularity of domains in \textit{Productivity, Information,} and \textit{Liability} risk groups are more uniform.
% This implies that popularity of domains in these 3 risk groups might have a significant influence on the reactions after the attack.
We could observe in the \textit{bottom plot} of Fig.~\ref{fig:reaction_by_risk_type} that Alexa ranks of reactive domains are more concentrated in the lower area, i.e., more popular, in every risk group. 
This result is consistent with our observation in Section~\ref{sec:domain_popularity} that higher popularity shows a correlation with the decision to react after the attack.
However, there is a higher spread in the popularity of reactive domains in \textit{Productivity} and \textit{Information} risk groups, which indicates a weaker correlation of the domain popularity with the decision to react.

%\textcolor{red}{The domains popularity in some risk groups such as Productivity might have a strong influence, why? What about information and liability?}
% 

\

\noindent\textit{\textbf{Key takeaway:} Domains in some risk groups (e.g., Liability) mostly unsubscribed after the attack.}
% \noindent\fbox{%
%     \begin{minipage}{0.95\linewidth}
%     \textit{\textbf{Key takeaway:} Domains in some risk groups such as \textit{Liability} (recall: may serve pirated material) mostly unsubscribed after the attack. 
%     \textcolor{red}{
%     The domains popularity in some risk groups such as Productivity might have a strong influence on the domain reactions after the attack. Popularity of websites have a lower impact on post-attack reactions for the domains that consume greater \textit{Bandwidth} or can be used for \textit{Communication}.}
%     }
%     \end{minipage}}

% Lower variation in these risk types indicate that the domains are relatively more homogeneous in terms of popularity, i.e., similarly quite popular (Figure~\ref{fig:reaction_by_risk_type}).

% \begin{figure}[t]
%      \centering
%      \begin{subfig}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/plot_risk_level_v2.pdf}
%         \caption{By risk level}
%         \label{fig:by_risk_level}
%      \end{subfig}
%      \hfill
%      \begin{subfig}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/plot_risk_type_v2.pdf}
%         \caption{By risk type}
%         \label{fig:by_risk_type}
%      \end{subfig}
%         \caption{Behavior by risk profile.}
%         \label{fig:by_risk_profile}
% \end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=.25\textwidth]{figure/plot_risk_level_v2.pdf}
%    \caption{Domain behaviors by different reactions across risk levels [make subfigure]}
%    \label{fig:reaction_by_risk_level}
%\end{figure}

\subsection{Analysis on Domain Autonomous Systems}
\label{sec:domain_as}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/AS-and-Rank-histogram.pdf}
    \caption{Histogram showing the variability in decisions within each AS and the average size (number of IPs) of ASes.}
    \label{fig:AS_Size_Histogram}
\end{figure}

A single party can operate multiple domains. For example, Alphabet Inc. operates, among others, google.com and gmail.com. So far we have not considered the potential effects of a single party making decisions (i.e., driving domain reactions) for multiple domains. 
As a first step towards exploring if multiple reactions are correlated to a single party, we measure the variety of reactions of Dyn customers within each Autonomous System (AS).

We associate domains to their hosting network at the time of the Dyn attack by mapping IP addresses (i.e., \texttt{A} records) to AS numbers, using IP-prefix-to-AS data set from CAIDA~\cite{the_caida_ucsd_routeviews_2008}. 
% We then calculate the number of IP addresses per AS that are used to host domains that react and compare it with the total number of IP addresses in each AS used to host Dyn customers. 
We then compare the proportion of IP addresses that reacted in each AS, i.e., number of IP addresses associated with reactive domains to all IP addresses in each AS.
Fig.~\ref{fig:AS_Size_Histogram} shows the resulting distribution.
We observe that in the case of about 200 smaller ASes (one to a few domains hosted), the domains all show the same behaviour. This suggests that parties that operate several domains drive the reaction for multiple domains, but on the order of a few hundred domains in total based on this initial view. This approach of course does not account for cases where a single party hosts their domains in multiple networks, which we leave for future work.

%In some cases, multiple domains can be operated by a single party. For example, an enterprise such as Alphabet Inc. can operate multiple domains such as google.com and gmail.com.\ Currently, we do not view the impact that the concentration of domains among the parties that operate them has on our results. However, to further explore if there are multiple parties responsible for the reactions we observe, we measure the variety of reactions observed within each AS. 
% \textcolor{red}{
%To do so, we extract the type of hosting that a domain was using during the incident by mapping IP address from domain's \texttt{A} record to its corresponding Autonomous System (AS) using IP prefix to AS dataset~\cite{the_caida_ucsd_routeviews_2008}
% } 
%Using this data we calculate the percentage of IPs that react out of the total number of IPs related to the domains using Dyn name servers. Fig.~\ref{fig:AS_Size_Histogram} shows the distribution for the percentage of \texttt{IP} addresses within each AS that react. We observe that in the case of only the smaller ASes, all domains show the same behaviour. For, larger ASes, we see only a small fraction of domains showing reactions. This shows that the resilience strategy chosen by domains within each AS was not the same, except when these ASes were relatively small.






%\textcolor{red}{A subsection on what kind of diversity in decisions do we notice per AS would be nice to argue that not all IPs in an AS reacted the same way.}


% \subsection{Hypothesis Testing}

% To test whether the differences in behavior across industry sectors and intended use are statistically significant, we did a statistical test. We compared the daily number of domains from two categories as two related-pair samples. Because most data are not normally distributed according to the Shapiro-Wilk test \cite{shapiro_analysis_1965}, we could not do a simple paired t-test. Instead, we did the Wilcoxon signed-rank test \cite{wilcoxon_individual_1945} for all possible pairs of industry sectors and intended uses. We repeated the test for three daily variables: number of domains that become non-exclusive, left, and returned. 
% The test shows variation in results between categories: some pairs are significantly different and some others are not. 
% A complete result of this test is presented in Table~\ref{tab:ttest_by_industry1}, Table~\ref{fig:returning_ttest_by_industry}, and Table~\ref{tab:ttest_by_purpose} in Appendix, alongside the complete metrics calculation in Table~\ref{tab:metrics_by_industry} and Table~\ref{tab:metric_by_purpose}.
% 
\section{Implications of results for Stakeholders}
\label{sec: Implications}
%We present possible implications of the results for different stakeholders, especially in managed DNS business.
% 
%\subsubsection{For Managed DNS Service Providers}
%\textcolor{red}{This should be a separate section and part of Discussion. Implications are very generic, we need examples from results for making them stronger.}

We evaluate the impact of factors such as domain popularity, industry sectors, domain risk level and risk group on decision of domain managers in reaction to unavailability of Dyn services. We believe that our results can be insightful for both providers and users of network services. In this section, we discuss the implications of these results for four a number of stakeholders:

\noindent \textbf{Managed DNS Service Providers:}
The results of this work are most useful for managed DNS service providers, especially to develop resilient strategy related with their customer portfolios. 
\begin{itemize}
    \item 
        DNS providers could use this work to estimate the proportion of their existing customers which are more likely to stop using the service in case of an outage incident. 
        For example, they can start profiling their existing customers using URL categorization service and Alexa rank to indicate which of them have characteristics (e.g., industry sector and popularity) that suggest a higher probability to leave in case of an outage.
    \item
        Using data of their existing revenue, DNS providers can quantify financially the potential business impact of an unforeseen outage by calculating the potential revenue loss coming from the number of customers with higher probability to leave in case of an outage.
    \item 
        DNS providers could use this estimation of potential business impact to justify their strategy in outage prevention e.g., infrastructure redundancy, or to minimize the loss, e.g., use cyber insurance. 
    \item
        Moreover, using this method, DNS providers should consider to monitor their customer portfolio in order to minimize the proportion of customers with characteristics (e.g., domain popularity and industry sector) that reflect a high probability to react or leave in case of an outage to minimize the business impact.
    \item
        Further, DNS providers could base their marketing strategy on the results of this work, for example, to offer more premium DNS services, e.g., with more redundant PoP servers, to customers that are more probably to react since it indicates that the customers adopt a more resilient strategy.
        
\end{itemize}
% They could develop a formula to measure their current risk score based on the number and the industry sectors of their current customers. 
% \textit{Second}, 
% \textit{Third}, they 
% 
%\subsubsection{For Digital Businesses}

\noindent \textbf{Digital Businesses:\ }
\textcolor{red}{}
The results could be beneficial for businesses in terms of managing their risk of downtime.
\begin{itemize}
    \item 
        They could adjust their investment to prevent or to deal with downtime, e.g., insurance, SLA, or use of backup provider, by estimating the relative cost of downtime based on their characteristics.
    \item
        They could adjust their contingency plan in case of downtime, e.g., what reaction they could take based on most domains in similar sectors. However, it needs further study to evaluate the quality or the impact of different decisions taken by the Dyn customers, i.e., whether their reactions were appropriate.
\end{itemize}


%\subsubsection{}
\noindent \textbf{Cyber Insurance:\ }
The results can assist in cyber risk calculation for insurance purpose. 
\begin{itemize}
    \item 
        Insurers can use these results to find the optimum price and compensation, according to business characteristics of their (potential) customers and estimated business impact of downtime.
        For example, cyber insurers could estimate a higher business impact of downtime on customers with characteristics that suggest a higher likelihood to react.
    \item
        With this estimation, cyber insurers can adjust their strategy to offer more competitive pricing and compensation scheme, e.g., higher premiums for customers with high likelihood to react.
\end{itemize}

%\textcolor{red}{Example! DONE}

%\subsubsection{}
\noindent \textbf{Academic Researchers:\ }
The methodology and results presented in this paper have shown a novel direction for Internet measurement research to explore the Internet ecosystem resilience properties and dynamics. Rapid growth of digital business and use of Internet as business enabler requires more attention from the academic measurement community. 
\begin{itemize}
    \item 
        Our methodology provides business context on large-scale Internet network measurements. This approach can initiate ground breaking insights for academic research in both business and technical fields, such as digital business ecosystem, cyber risk, and centralization topic.
    \item
        Our methodology translates observations from measurement data into business insight which might accelerate strategic decision making related with digital resilience such as cyber security investment.
    \item
        The results from this work could help researchers analyze industry sectors regarding their concern about DNS service availability, and behavior against downtime in general, based on our statistical model.
        
\end{itemize}

==> section/introduction.tex <==
\section{Introduction}

% Elaborate problem statements and previous works

% Situation

% REMOVED DUE TO REVIEW
% Rapid development in cloud technology has led to a move from on-premise solution to outsourced services \cite{hsu2014examining}. 
% With the increase in the number of businesses that consume and provide services through Internet, quality of service stands out as one of the competitive advantages in this emerging market \cite{alkhater2018empirical}. 
% Service quality determines and influences selection of cloud service providers. 
% Service outage frequency is a key factor that can diminish the quality of service by making online resources unavailable for businesses and their consumers for a period of time. 
% Downtime in service availability causes disruption in business and leads to a loss \cite{abhishta2019blind}. 
% However, the financial loss experienced by businesses due to unavailability of online resources may depend on their business type. 
% Each industry sector has its own cost of downtime, according to the nature of the business and the importance of the unavailable service. 
% For some business types, every second of Internet unavailability may cost millions of dollars, while for others, the cost can be negligible \cite{florencio2013sex}.

% Complication
Cloud-based infrastructure as a service (IaaS) providers offer premium services (e.g., managed DNS and Content Delivery Network (CDN)) that promise high availability and performance of customer services~\cite{mell_nist_2011}.
Businesses purchase these services to hedge the risk of accumulating losses from network downtime. Unplanned outages of these cloud providers might significantly disrupt businesses that depend on their infrastructure/services~\cite{dubendorfer_economic_2004}. For some business types, every second of Internet unavailability may cost millions of dollars, while for others, the cost can be negligible \cite{florencio2013sex}. 

Businesses that use a managed DNS service often have the opportunity to adopt a more resilient strategy (i.e.,\ use multiple DNS service providers) that ensures higher availability even when that managed DNS service provider may be unavailable. Previous studies \cite{abhishta_measuring_2019,bates2018evidence} have shown that when services of Dyn, a large managed DNS service provider, became unavailable in 2016 \cite{bolstridge2016dyn}, a considerable number of domains adopted this more resilient strategy to counter the effects of downtime. The same studies have also shown that the domains that adopted the more resilient strategy were not in majority. Different businesses value high  availability differently, but it clearly sometimes directly induces loss of revenue~\cite{akamai2018}.

@@make roadmap of paper.
Section\ref{sec:related_work} reviews related work.
Section~\ref{sec:mdns_business} discusses the relationship between various industry sectors and importance of Internet availability to them.

%The technological impact of DNS unavailability and consequences of centralization in this market has been discussed in the literature at great lengths. We summarize these findings in Section~\ref{sec:related_work}. A study using survey-based methodology to understand the perception of unplanned unavailability of network services to its customers report that the largest loss is due to the unavailability of customer facing services~\cite{akamai2018}. \cite{florencio2013sex} have argued that most cybercrime surveys provide limited insights as they use restricted sample size and selection criteria. In this paper, using an empirical methodology, we evaluate the influence of factors such as industry sector and website popularity on the decision of Dyn customers to follow the previously discussed more resilient strategy.


% \textcolor{red}{something on the real life implication of this outage. Why should we still care? Maybe, a short comparison with recent outages and their impact on network availability world wide.} 

%Our aim is to be able to predict how cloud service consumers, such as managed DNS consumers, would react upon an outage incident, so that different stakeholders can anticipate the business impact of such events. 

% Answer
We perform an analysis of large-scale longitudinal active DNS measurement data to identify domains that responded to the outage. We then map these domains to their popularity rank (using historical Alexa ranks), industry sector and risk characteristics such as level of maliciousness \& risk type (using McAfee URL categorization service). We discuss the datasets used for this analysis and their characterstics in Section~\ref{sec:methodology}. Further in Section~\ref{sec:Result_and_Discussion}, we analyze this mapped data to understand the influence of various factors such as industry sector and website popularity on the decision of Dyn customers to use of more resilient DNS strategy.

% Conclusion
% 
% Brief about conclusion here, needs update...
% 
% \textcolor{red}{ 
% [Still Working][CONTRIBUTION] We show that all following aspects do influence post-outage decisions of customers of Dyn:
% \begin{itemize}
%     \item \textit{Popularity} of the domain names
%     \item \textit{Industry sector} of the domain names
%     \item \textit{Risk level} of the domain names
%     \item \textit{Risk type} of the domain names
% \end{itemize}
% }

% \textcolor{red}{AVOID USING TERMS THAT NEED FORMAL DEFINITIONS!}
\ 

Overall, we make the following contributions:
\begin{itemize}
    % methodology
    \item 
    We present a novel methodology to analyze longitudinal Internet measurement data.
    % to estimate business impact of cyber attacks on DNS providers based on customer portfolio.
    We characterize domains affected by the Dyn outage based on a number of aspects, including responses after the outage, popularity, industry sectors, and risk characteristics.
    % domain popularity influence on reaction
    \item 
    % \textit{We demonstrate in Section~\ref{sec:domain_popularity} how popularity of domains correlate with the reactions after the attack and} 
    We observe that domains with higher popularity, indicated by Alexa rank, have a higher chance to adopt a more resilient strategy.
    % Later in Section~\ref{sec:stat_analysis}, \ref{sec:domain_risk_level}, and \ref{sec:domain_risk_type}, 
    % We show how to identify whether the popularity plays an important role on the reactions.
    % quantitative measure of industry sector influence
    \item 
    % We statistically model the correlation between domain industry sectors and the probability of reacting to outage in Section~\ref{sec:stat_analysis}. 
    We observe that some industry sectors have a higher and significant influence on the post-attack response of the domain managers, while some others do not.
    % risk and reaction
    \item 
    % We discuss the correlation between risk characteristics of domains and the reactions after the attack.
    We show different post-attack responses across domains with different levels of maliciousness and risk types, according to McAfee URL categorization service.
    % using data to validate prior known premise about value of availability for businesses
    \item 
    Our results confirm the notion about availability that certain aspects, such as industry sector and popularity of domain names,
    % indicate a higher concern about availability among managed DNS customers thus 
    influence the resilience strategy adopted by the domain managers.
    % \item \textit{We propose an approach to evaluate possible business impact of cyber risk on Cloud providers \textbf{based on their customer portfolio} which existing frameworks do not take into account~\cite{akinrolabu_csccra_2019,akinrolabu_cyber_2019}}. PUT THE CITATIONS IN THE FIRST POINT.
\end{itemize}

We believe that our results can be useful, not only for manage DNS industry to understand the possible aftermath of unforeseen downtime, but also for other stakeholders, such as insurance service providers, who are interested in measuring the cost of unplanned network downtime. We discuss this topic in Section~\ref{sec: Implications}.
% 
% i.e., popularity, industry sector, risk level, and risk type of domains, do have an influence on post-outage decision. They influence, in different ways, the decision
% (1) \textit{to react or not}, 
% (2) \textit{to become non-exclusive or unsubscribe}, and 
% (3) \textit{to return or not}. 
% \\
% Include contribution here and summarize conclusion.
% }

  

%how different domain owners/managers take decisions following a major downtime incident forced by a large denial of service attack. 
%We use large-scale DNS measurement data to investigate the change in behaviour of customers (categorised by domain characteristics) of Dyn after the DDoS attack in 2016. 
%We classified all active domains that used Dyn managed DNS service prior to the incident into different domain statuses after the incident: those who keep using and those who stop using the service. 
%We further consider the status change in these domains as reactions of the domain owners in response to the incident.

%\begin{description}
   % \item[The attack] The day, Oct. 21, 2016 (\textit{day 0}), in which Dyn suffered an outage of its managed DNS service from a DDoS attack.
    %\item[Dyn customers] Domains under \texttt{.com}, \texttt{.net}, and \texttt{.org} that used at least one of Dyn name servers (\texttt{*.dynect.*}) \textit{one day before} the attack i.e., Oct. 20, 2016 (\textit{day -1}).
    %\item[Domain status] The relationship between a Dyn customer and Dyn on a certain day in terms of use of Dyn name servers.
  %  \item[Exclusive domain] Domain status that indicates the use of \textit{only} name servers from Dyn.
  %  \item[Non-exclusive domain] Domain status that indicates the use of name servers from Dyn \textit{and at least one} name server \textit{other} than Dyn name servers.
    %\item[Unsubscribed domain] Domain status that indicates the use of \textit{only} name servers \textit{other} than Dyn name servers.
    %\item[Domain movement] Changes in domain status between adjacent days.
    %\item[Observation period] A period of 20 consecutive days after the attack, from Oct. 22, 2016 (\textit{day +1}), to Nov. 10, 2016 (\textit{day +20}), in which the daily domain status of Dyn customers were observed.
    %\item[Do nothing] Domain response following the attack in which no single change in domain status is observed within the observation period.
   % \item[Non-reactive domain] Dyn customers which \textit{did nothing} in response to the attack.
%    \item[Reactive domain] Dyn customers whose domain status changed at least once within the observation period in response to the attack.
 %   \item[Become non-exclusive] Domain response following the attack by changing its domain status from exclusive to non-exclusive, i.e., use redundant services.
  %  \item[Unsubscribe] Domain response following the attack by changing its domain status from exclusive or non-exclusive to unsubscribed, i.e., stop using Dyn DNS service.
%\end{description}


%To understand more about factors influencing domain owners, we study the characteristics of these domains from different aspects.
%We use ranks from Alexa Top 1M list to measure domain popularity and
%a URL categorization service to classify these domains into different industry sectors, risk types, and risk levels.
% In addition, we enriched the data with information about the type of hosting which the domains used from their AS number.

%We employ two main research questions to guide this study. 
%\begin{itemize}
%    \item \textit{How does each domain characteristic influence the decision made by %    \item \textit{How do owners of domains in the same category behave?}
%\end{itemize}
% Methodology
% We use two types of analysis to answer these questions.
% \textit{First}, we conduct statistical analysis to study how significantly important industry sector of the domains are in making a decision towards a decision to react.
% \textit{Second}, we conduct graphical analysis using plots and diagrams to study the behavior of domains in the same category.



% \textcolor{red}{
% CONCLUSION.
% We show the difference in behavior across industry sectors using three perspectives. 
% \textit{First}, what type of reaction i.e., whether a domain chose to keep using Dyn but became non-exclusive, or to stop using Dyn service. 
% \textit{Second}, how delayed was the reaction i.e., whether a domain reacted immediately after the incident or later.
% \textit{Third}, returning movement i.e., whether a domain returned after it stopped using Dyn or left for good.
% We observe differences in the behaviour among industry sectors and intended uses. 
% Specifically, most domains in Finance sector showed a distinct behavior that suggests sensitivity to reliability of the DNS provider, as they permanently stopped using the services a few days after the incident.
% In addition, using the Wilcoxon signed-rank test we check whether the differences we observed are statistically significant.
% }
% 
% 
% 


==> section/mdns_business.tex <==
\section{Business of Managed DNS Service and Importance of Internet Availability for different Industry Sectors}
\label{sec:mdns_business}
% 
% DNS is one key component of Internet ecosystem.
% Its main role is to translate the domain name to its corresponding IP address. 
% The use of domain name is beneficial for multiple reasons, including ease of use and stable connectivity.
% Nowadays, almost all Internet-based services use domain name extensively and rely on it.

The domain name system (DNS) is a core component of the Internet. Its primary function is to translate human-readable domain names to IP addresses. Domain-destined communication (e.g., business website visits) may no longer be possible if the authoritative name servers for a domain name fail to function. 


A managed DNS service provider offers premium services to manage DNS traffic, especially for businesses which rely on it~\cite{abhishta_measuring_2019}. It offers better reliability and performance with better computing and network infrastructures, and may offer a DDoS protection. Domain name owners can delegate authority to managed DNS services, which, among others, can provide greater resilience against denial-of-service (DoS) attacks. If managed DNS services themselves however fall over, this can have adverse effects on many of the depending parties. The effects are not necessarily always earth-shattering: businesses will view unavailability based on its operational consequences.

%DNS resolves the domain name requested by the client through a DNS resolver into an IP address. 
%The resolver will locate the authoritative name server (ANS) for the domain name and query the ANS for the IP address of the domain name. 
%Once obtained, the IP address will be returned to the client, so the client can contact the corresponding machine using the IP address. 
% DNS makes use of caching mechanism in which a record is stored for a certain Time to Live (TTL) before it gets refreshed by a new record.


% Hence, their customers can expect higher availability for their online resource by using managed DNS service.


%\subsection{}
% 
% Explain why different business value and require availability differently and how managed DNS can be an important service
% 
% Reference: \cite{barua_empirical_2004}
% 
% Main idea: Availability as digital business capability and value \\
% 
% Main idea: Managed DNS offers premium service for higher availability \\
% 
% Historically businesses have been viewed either as brick \& mortar or as online or as a combination of the prior two based on the mode of delivery of service. 
Today, even most ``brick \& mortar" businesses have an online presence, either for e-commerce, marketing, or communication~\cite{pozzi2013effect}.
%The backbone services of the Internet such as the domain name system play a crucial role in making the digital business of firms available. 
% As discussed before managed DNS service providers offer additional resilience to availability as they are able to leverage their infrastructure to defend against attacks such as denial of service.
% Of-course, this resilience comes at an additional cost, hence, most 
Managed DNS providers charge a premium for using them as authoritative name servers. 
% As dependence of Industry varies per Industry sector, 
But, it is not profitable for all business types to bear this additional cost. It depends on the return on investment that is expected by the business by guaranteeing high up-times of their online services. To understand the influence of factors such as business sectors and website popularity on the willingness to spend additional cost to guarantee high availability of online services, we perform an analysis of Dyn customers (domains that use its services) that followed a resilience strategy of either using an additional DNS provider or switch to another provider after the attack. We empirically draw differences between the industry sectors that followed the above mentioned strategy and the one's that did not. Thus, giving us a peek into the the cost of unintended downtime anticipated by customers of Dyn.

%We hypothesise that industry sectors who value availability more are more likely to change their status. We observe the decisions taken by different industry sectors and empirically test the relationship between the type of business and the decision to change status.

%Importance of Internet for different firms.

%Dependence of industry sector on ICT.
% how mDNS affects it

% MIS Quarterly paper about An Empirical Investigation of Net-Enabled Business Value

% Digital Business Capability



==> section/result.tex <==
 \section{Result and Discussion}
\label{sec:Result_and_Discussion}
% 
%We next present our results and discuss the implications for various stakeholders. %Third, we discuss the limitation of this research and possible further studies in the future.
% 
%\subsection{Descriptive Statistics}
%As discussed in Section~\ref{sec:key_concepts}, all active domains which used Dyn service a day before the incident can be categorised into reactive and non-reactive domains. They can also be categorised based on their statuses i.e., exclusive or non-exclusive. Figure~\ref{fig:domain_count} summarises the number of domains according to these categorisation.
% 
%In the previous section, we introduce the key concepts and state a step-by-step methodology. Here, we present our findings.
We identify nearly 168K domain names that were Dyn customers on the day prior to the DDoS attack. 

%discuss the results of each step we performed in more detail. 

% start with initial finding
% We start by explaining some initial findings and summary of our data set that are important to note, including URL categorization results and the distributions of domains by their initial status and reactions.
% influence of each aspect
% Then, we discuss the influence of each aspect of domains characteristics to the domains post-attack reactions.
% key takeaway
% We also attach key takeaways preceding discussions in this section in bold format.


%
% \begin{table}[]
%     \caption{Summary of domains.}
%     \setlength{\tabcolsep}{3pt}
%     \renewcommand{\arraystretch}{1}
%     \resizebox{.48\textwidth}{!}{%
%         \centering
%         % \tiny
%         \begin{tabular}{ l r r }
%             % \hline
%             \toprule
%             {\textbf{Description}} & {\textbf{Unique Count}} & {\textbf{\% of Total}} \\
%             % \hline
%             \midrule
%             Initial Set of Domains* & 168,577 & 100.00\% \\
%             \quad Uncategorized Domains** & 62,408 & 37.02\% \\
%             \quad Categorized Domains & 106,169 & 62.98\% \\
%             \quad \quad Non-reactive Domains (\textbf{R0}) & 102,972 & 61.08\% \\
%             \quad \quad Reactive Domains (\textbf{R1,R2 \& R3}) & 3,197 & 1.90\% \\
%             % \quad \quad \quad Became Non Exclusive \quad \quad \quad & 1,361 & 0.81\% \\
%             % \quad \quad \quad Unsubscribed & 1,836 & 1.09\% \\
%             % \quad \quad \quad \quad Did Not Return & 1,315 & 0.78\% \\
%             % \quad \quad \quad \quad Returned & 521 & 0.31\% \\
%             % \hline
%             \bottomrule
%             \textit{*Active domains as per 20 October 2016.} & & \\
%             \textit{**Excluded from further analysis.} & & \\
%             \hline
%         \end{tabular}
%     }
%     \label{tab:domain_summary}
% \end{table}

% \begin{table}[]
%     \caption{Count of categorized domains by initial response.}
%     \setlength{\tabcolsep}{1pt}
%     \renewcommand{\arraystretch}{1.1}
%     \resizebox{.48\textwidth}{!}{%
%         \centering
%         \tiny
%         \begin{tabular}{lrrrr}
%             % \hline
%             \toprule
            
%             {Initial Status} &  Not reactive &  Became non exclusive &  Unsubscribed &   Total \\
%             % \hline
%             \midrule
%             Exclusive     &         85,449 &                  1,361 &          1,791 &   88,601 \\
%             Non Exclusive &         17,523 &                     0 &            45 &   17,568 \\
            
%             % \hline
%             \bottomrule
%             Total         &        102,972 &                  1,361 &          1,836 &  106,169 \\
%         \end{tabular}
%     }
%     \label{tab:domain_initial_response}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
%     \caption{Categorized domains by initial status and behavior.}
%     \setlength{\tabcolsep}{2pt}
%     \renewcommand{\arraystretch}{1.5}
%     \centering
%     \resizebox{.48\textwidth}{!}{%
%     \begin{tabular}{llrrrrrlr}
%     \hline
%     \multirow{3}{*}{\textbf{Initial Status}} & \multicolumn{6}{c}{\textbf{First Response}}                          & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Total}}} \\ \cline{2-7}
%      &
%       \multicolumn{2}{l}{\textbf{Not Reactive}} &
%       \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}To Non Exclusive\end{tabular}}} &
%       \multicolumn{2}{l}{\textbf{Unsubscribed}} &
%       \multicolumn{2}{l}{} \\ \cline{2-9} 
%      &
%       \textbf{\#Unique} &
%       \multicolumn{1}{l}{\textbf{\#Row}} &
%       \multicolumn{1}{l}{\textbf{\#Unique}} &
%       \multicolumn{1}{l}{\textbf{\#Row}} &
%       \multicolumn{1}{l}{\textbf{\#Unique}} &
%       \multicolumn{1}{l}{\textbf{\#Row}} &
%       \textbf{\#Unique} &
%       \multicolumn{1}{l}{\textbf{\#Row}} \\ \hline
%     Exclusive                                & \multicolumn{1}{r}{85,449}  & 89,277  & 1,361 & 1,471 & 1,791 & 1,915     & \multicolumn{1}{r}{88,601}         & 92,663         \\
%     Non Exclusive                            & \multicolumn{1}{r}{17,523}  & 18,198  & -     & -     & 45    & 50    & \multicolumn{1}{r}{17,568}         & 18,248         \\ \hline
%     Total                                    & \multicolumn{1}{r}{102,972} & 107,475 & 1,361 & 1,471 & 1,836 & 1,965 & \multicolumn{1}{r}{106,169}        & 110,911        \\ \hline
%         \multicolumn{9}{l}{\textit{\#Unique: number of unique domains; \#Row: total row after splitting multilabels;}} \\
%         % \multicolumn{9}{l}{\#Row: total row after splitting multilabels} \\
%         \hline
%     \end{tabular}%
%     }
    
%     \label{tab:categorized_domain_by_status}
% \end{table}



%
% \noindent
% \begin{minipage}[t]{\textwidth}
% \begin{minipage}[b]{0.49\textwidth}
% %\begin{figure}%[h]
%     \centering
%     \includegraphics[width=\linewidth]{figure/general_statistic.png}
%     \captionof{figure}{Number of active domains, the type of reaction, and the initial status per reaction type. Only a small fraction of non-exclusive domains reacted to the attack. A possible cause is the presence of backup service.}
%     \label{fig:domain_count}
% %\end{figure}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.49\textwidth}
% %\begin{figure}%[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figure/unreachable_statistic.png}
%     \vspace{0.5em}
%     \captionof{figure}{Number of reachable and unreachable domains by Zvelo. Some of the reachable domains are labelled with multiple categories. Hence, the number of unique domains are smaller than the number of rows in the dataset.}
%     \label{fig:unreachable_domains}
% %\end{figure}
% \end{minipage}
% \end{minipage}

% \todo[inline]{MJ: I think `unreachable' may confuse readers. In the paper's context, unreachable as the result of the attack is probably the first thing to come mind. Unreachable from a categorization lookup point of view is less obvious. Discuss with Abhishta, but if redoing the figures and rebranding these as `still existing' or `categorizable' or reasonable and still possible, I think it's worth considering.}
% \todo[inline]{MJ: what currently feels unresolved is the fact that the Zvelo lookups were done recently and for this reason some names are more likely to be not be categorizable 5 years after the fact.}

% \begin{table}[t]
%     \setlength{\tabcolsep}{3pt}
%     \renewcommand{\arraystretch}{1.5}
%     \centering
%     \resizebox{.7\textwidth}{!}{%
%         \begin{tabular}{llrrrr}
%             \hline
%             \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Domain \\ Status\end{tabular}}} &
%               \multicolumn{5}{l}{\textbf{Company Type}} \\ \cline{2-6} 
%              &
%               \textbf{Business} &
%               \multicolumn{1}{l}{\textbf{Hosting}} &
%               \multicolumn{1}{l}{\textbf{ISP}} &
%               \multicolumn{1}{l}{\textbf{Education}} &
%               \multicolumn{1}{l}{\textbf{Unknown}} \\ \hline
%             Exclusive     & \multicolumn{1}{r}{17,986} & 6,890 & 2,944 & 72 & 121 \\
%             Non Exclusive & \multicolumn{1}{r}{8,074}  & 1,970 & 559   & 12 & 15  \\ \hline
%         \end{tabular}%
%     }
%     \caption{Number of non-reactive domains by domain status and company type.}
%     \label{tab:non_reactive_domains}
% \end{table}

\subsection{Categorization of Dyn Customers}
%We identify nearly 168K domain names that were Dyn customers on the day prior to the DDoS attack.
%We obtain nearly 168K domain names which used at least one Dyn name server from the measurement data on the given day.
%We refer to this set of domain names as the initial set of domains (Table~\ref{tab:domain_summary}). 

We query category labels and reputation scores of the initial set of domains using a publicly available URL categorization service provided by McAfee ``Real-Time Database"~\cite{vallina_mis-shapes_2020}. % \textcolor{red}{Reference}. 
%We query the categories associated to these 168K domains at a non-intensive average rate lower than 40 reques. %We observe two findings from the domains categorization process: 
\noindent \textbf{$\approx$ 62\% of the domains were categorized by McAfee.} 
Some domain names are not yet categorized by McAfee, these are domains that are either no longer in operation or do not have enough features available for McAfee's classifier to make a deterministic classification.
%we did not obtain any category label from the service.
% Domain names which are no longer in operation or are not yet listed for categorization by McAfee could not be categorised. 
We refer to these domains as \textit{Un-categorized domains}. In this paper, we limit our analysis only to the domain names which were successfully categorized by McAfee, i.e., around 106K unique domains or nearly 62\% of all unique domains that used Dyn services one day prior to the attack (Fig.~\ref{fig:macro_flowchart}). 
% Among them, around 102K unique domains are non-reactive and only around 3K unique domains reacted.
% Table~\ref{tab:categorized_domain_by_status} presents a more detailed summary with additional information of their initial status and first response.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/Flowchart Domains.drawio.pdf}
    \caption{Dyn customer subdivision in category, domain status and reaction. We identify 169K customers and categorize per our methodology. We distinguish exclusive and non-exclusive domains and subdivide into reactions. For example, out of $\sim$17K non-exclusive domains, 45 unsubscribed following the attack, and 24 out of 45 did not return to Dyn later.}
    \label{fig:macro_flowchart}
\end{figure}

%\subsubsection{Multiple Category Labels}
%  \textbf{Domain names can be related to multiple categories.}
Some domain names are mapped to multiple industry sectors and risk groups by McAfee. We consider all retrieved category labels for our analysis. 
% \textcolor{red}{This approach aligns with our objective to focus on the relationship between sectors and post-incident responses.\textbf{, why?}} 
Hence, the total number of category labels retrieved for the domains are more than the total number of unique domains.%, as shown in Figure~\ref{fig:macro_flowchart}.

% \subsection{Summary of Domains Reactions}
% Our dataset now contains around 106K of categorized domains. 
We retrieve daily \textit{Domain Status} for all categorized domains from the measurement data for 20 days after the attack to observe status changes which can be used to capture \textit{Domain Movements} as discussed in Section~\ref{sec:methodology}.
%We identify two initial observations:

\noindent \textbf{The number of \textit{Non-reactive Domains} is significantly higher than \textit{Reactive Domains}.}
The number of \textit{Non-reactive Domains} is significantly higher than \textit{Reactive Domains} by a ratio of 32:1 (Fig.~\ref{fig:macro_flowchart}). 
%For \textit{Exclusive Domains}, this movement is particularly unusual since they were more probably to have a period of downtime when the incident happened.
We observe more \textit{Exclusive Domains} either becoming non-exclusive or unsubscribing to Dyn services as they have a greater probability of experiencing downtime due to the lack of redundancy in authoritative name servers.Whereas among non-exclusive domains, only 45 out of nearly 17K domains reacted. 
This is predictable since they had redundancy, hence, did not need to react.  
More than 85K out of $\approx$88K of \textit{Exclusive Domains} did not show any reaction (Fig.~\ref{fig:macro_flowchart}). This can be explained by the presence of cached \texttt{NS} records on DNS resolvers might keep several domains accessible during the outage~\cite{MouraIMC2018}.
% We expect to explain this behavior with additional data on domain characteristics in the next sections.


\noindent \textbf{The number of domains that became non-exclusive is not significantly different with the number of domains that unsubscribed.}
Reactive domains showed two types of movement in terms of their decision to become non-exclusive or to unsubscribe from Dyn (Fig.~\ref{fig:macro_flowchart}). 
Among 3,197 reactive domains, 1,361 became non-exclusive and 1,836 unsubscribed.
We observe that there is no clear preference in the type of movement among domains since the numbers are not significantly different.
This observation motivates us to zoom into domains with similar characteristics, i.e., in terms of popularity, expecting to discover specific preferences in the resilience strategy among similar Dyn customers.
% All 45 reactive \textit{Non-exclusive Domains} chose to unsubscribe from Dyn.
% We further discuss in the next sections the return behavior of these unsubscribed domains.

\subsection{Popularity Influence on Decision to React}
\label{sec:domain_popularity}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/reactive_by_alexa_rank_bin2.pdf}
    \caption{
        % Domains reactions in different groups of popularity. 
        % Groups indicate cumulative classification. 
        % For example, \textit{top1k} includes domains in \textit{top100}. 
        % The percentages represent the proportion of \textit{reactive} and \textit{non-reactive} domains in each group. 
        Reactions of Dyn customers -- reactive or non-reactive -- among different Alexa popularity groups. For example, among \textit{top100} Alexa customers, 42.9\% react to the attack. (Note that larger groups are supersets, i.e., the \textit{top100} are included in the \textit{top1k})
    }
    \label{fig:by_popularity}
\end{figure}


% \textcolor{red}{How many domains have an Alexa rank? [DONE]}
We then incorporate Alexa rank data into our data set to indicate how popular each domain is.
Out of $\approx$106K domains, we manage to retrieve popularity ranks of $\approx$5K domains that belong to the Top 1M Alexa list and ignore the ones which do not.  
% \textcolor{red}{get numbers for categorized only, change to active voice [DONE]}
% We ignore domains outside the Top 1M Alexa lists.
We observe that domains with higher Alexa rank have a higher proportion of reactive domains (e.g., 42.9\% in top100) compared to those with lower rank (e.g., 14.3\% in top1m) as shown in Fig.~\ref{fig:by_popularity}:
the percentage of reactive domains decreases as more domains with lower rank are included.
Popularity of the domains is thus one factor that might influence the decision to react.

A higher rank means a higher traffic to these domains which may result in a higher revenue~\cite{truong_relationships_2018}.
Hence, owners of domains with higher rank will prefer minimizing downtime of their domains to avoid revenue loss. Meanwhile, owners of domains with lower rank may not very sensitive to short-term downtime.
Some reactions involve an extra cost, e.g., using multiple DNS service providers, which may not be worthwhile for businesses with smaller revenue.



%To describe how popularity may affect the domains reactions, we include Alexa rank data of the domains in our further analysis.
%We attach \textit{mean Alexa rank} of domains in a certain group to indicate \textit{how popular the domains are on average}.
% We also compute the \textit{coefficient of variation} as the ratio between the sample standard deviation and mean~\cite{everitt_cambridge_1998} for ranks of domains within each industry sector to analyze the impact of website popularity on the decision of domains to chose a resilience strategy.
% 

\ 

\noindent
\textit{\textbf{Key takeaway}: We observe that customers running domains for more popular websites (based on Alexa rank) reacted to the attack with higher probability.}
%\noindent\fbox{%
    %\begin{minipage}{0.95\linewidth}
    %\textit{\textbf{Key takeaway}: Comparing the Alexa ranks of the domains that react and do not react to the %attack, we observe that those with a higher website popularity (lower Alexa ranks) have a greater probability %of reacting to the outage.}
    %\end{minipage}}
% These two metrics assist in determining whether the behavior is strongly influenced by popularity of domains.

% How domains with higher Alexa rank behave differently with domains with lower Alexa rank. Mention how many domains with rank and without rank. 

% Plot: histogram of popularity index

% Plot: bar chart behaviors by binning




% We later discuss in depth the behaviors of domains in these selected categories in Section~\ref{sec:domain_sector}.
% Each category has various number of domains labeled with. 

% \textcolor{red}{The following discussion section needs updating of structure and content}
% 
% 
% 
% \textcolor{red}{A paragraph on methodology will be nice to manage expectations.It will make it clear why statistical test is used to select important industry sectors.}
% 
% 

% We now discuss the behavior of categorized domains from three perspectives: 1) to react or not, 2) to become non-exclusive or to unsubscribe; 3) to return after unsubscribing or not.

% \subsection{Overall Behavior}
% 
% First we discuss about the overall behavior of the active domains which were using Dyn DNS service during the incident as summarized in Table~\ref{tab:categorized_domain_by_status}. 
% 
% \begin{observation}
%     The proportion of reactive domains are relatively small ($\approx$3K domains) compared to non-reactive domains ($\approx$102K domains), despite many of them ($\approx$85K domains) were critically dependent on Dyn DNS service.
% \end{observation}
% 
% \begin{observation}
%     Only a tiny fraction (45 domains) of $\approx$17K non exclusive domains reacted by unsubscribing from Dyn.
% \end{observation}
% 
% 
% 
\subsection{Industry Sector Influence on Decision to React}
\label{sec:stat_analysis}
% Content:
% \begin{itemize}
%     \item Define dependent variables: 4 types of reactions @ 1 model
%     \item Define independent variables: 4 aspect of domain characteristics
%     \item Explain why choose logistic regression
%     \item Present the result in a table
%     \item Mention selection for industry sector selection
%     \item Explain how to interpret the result using example
% \end{itemize}


% \textcolor{red}{How? There are 106K unique domains? We should only talk about unique domains throughout the paper.}
% This result shows that each category is significantly different in terms of the number of domains.
% Considering the space limitation, we cannot discuss all 94 categories in depth.
%\textcolor{red}{Even if we had space we would not have talked about 94 categories.} 
 

%We make use of a multivariate logistic regression model to determine the impact of individual industry sectors on domain reactions (\textbf{R0} vs \textbf{R1}, \textbf{R2} \& \textbf{R3}).
%We then perform a regression analysis to measure correlations between each category to domain reaction.

We obtain nearly 106K labeled domains with 94 unique categories from the categorization process. We discuss in more detail the Industry Sectors that had a significant impact on the resilience strategy adopted by the domain managers. 

To determine the impact of individual industry sectors on domain reactions, we model the resilience strategy adopted by the domains as a function of their industry sector using a multivariate logistic regression analysis. We model the binary decision of domains to react (react: \textbf{R1}/\textbf{R2}/\textbf{R3} or not react: \textbf{R0}) as a dependent variable (\ref{eq:logit_decision}). 

\begin{equation}
\label{eq:logit_decision}
    \text{\textit{logit}}(\pi_{b})=\log[\frac{\pi_{b}}{1-\pi_{b}}],
\end{equation}

\noindent where $\pi_{b} \in [0,1]$ represents the probability of a domain reacting and can be estimated using (\ref{eq_logit_estimation}).

\begin{equation}
    \label{eq_logit_estimation}
    \pi_{b}=\frac{\beta_{0}+\sum_{i}^{}\beta_{i}x_{i}}{1+(\beta_{0}+\sum_{i}^{}\beta_{i}x_{i})},
\end{equation}

\noindent where $x_{i} (i=1,2,3,....,94)$ represents each industry sector as a separate independent variable. $x_{i}$ has a value of 1 if a domain belongs to this industry sector, otherwise it has a value of 0. $\beta_{i}$ is the odds ratio and signifies the strength of correlation between this independent variable and the dependent variable. In this analysis, $\beta_{i}$ shows the factor with which an industry sector $i$ will increase the probability of a domain to react. To implement logistic regression, we use \texttt{statsmodels} package in python~ \cite{seabold2010statsmodels}.
% Explain the motivation of GLM use


%The reason of this specific choice of model is due to the binary identity of the dependent variable i.e., react or not react, and the independence between domain decisions to react.
%\textcolor{red}{[OPTIONAL] The predicted value of the regression model is the probability of a domain labeled with certain categories to react after the attack.}
% option A
%We define $Y_d$ as the decision of domain $d \in D$ after the attack with $D$ being all categorized domain names of Dyn customers.
%$Y_d$ is 1 if domain name $d$ changes its Domain Status at least once after the attack and 0 if otherwise.
% We transform the category labels given to each domain using one-hot-encoding resulting in dummy variables that we use as our independent variables ($X$).
% Option B
%Our independent variables, $X$, are a set of $X_c$, which equals to 1 if a domain is labeled by category $c \in C$ with $C$ being 94 unique categories, and 0 if otherwise.
% 
%For the regression model to converge, we eliminate categories that have only 1 domain due to low variance.




The regression model outputs three main metrics to indicate the influence of each category as Table~\ref{tab:stat_result} shows.
\textit{Coefficient} ($\beta_{i}$) indicates the fraction by which the probability of a domain reacting to the attack increases, if this domain belongs to Industry Sector $i$  i.e., the more positive the coefficient is, the higher the influence.


\begin{table}[t]
    \centering
    \caption{GLM coefficients for domains showing most prominent industry sectors that had a statistically significant influence on domain reactions (ordered by the number of domains in each industry sector).
    %\textcolor{red}{The selected categories changed. So we need to change the plot too?(DONE)}
    }
    \label{tab:stat_result}
    
   \begin{tabular}{lrr}
\toprule
Industry Sector&    Coefficient\textsuperscript{*} &       z-value \\
\midrule
Internet Services                    &  0.47 &   6.80 \\
Travel                               &  1.25 &  14.61 \\
Content Server                       &  1.26 &  11.00 \\
Motor Vehicles                       &  0.78 &   6.26 \\
General News                         &  2.17 &  24.05 \\
Job Search                           &  1.30 &   9.40 \\
Streaming Media                      &  2.15 &   6.57 \\
Gambling                             &  1.60 &   8.97 \\
Portal Sites                         &  1.74 &   6.51 \\
PUPs (potentially unwanted programs) &  2.83 &  12.28 \\
Malicious Sites                      &  2.61 &   8.91 \\
Social Networking                    &  2.47 &   7.75 \\
Personal Pages                       &  1.87 &   5.37 \\
Provocative Attire                   &  2.71 &   4.86 \\
For Kids                             &  3.07 &   4.93 \\
Interactive Web Applications         &  2.61 &   7.97 \\
Weapons                              &  1.98 &   5.32 \\
Professional Networking              &  3.58 &   9.34 \\
Visual Search Engine                 &  4.12 &   7.42 \\
Instant Messaging                    &  4.03 &   5.32 \\
        \bottomrule
        \textit{\textsuperscript{*}p$<$0.001}
    \end{tabular}
\end{table}
%We compare industry sectors to  one is more likely to react following an outage incident.
For example, domains in the \textit{Professional Networking} with coefficient value 3.58 are more likely to react than domains in the \textit{Motor Vehicles}, such as web sites of car manufacturers and sales, with coefficient value 0.78.
Hence, we expect the proportion of reactive domains is higher in the former than the latter.
\textit{p-value} indicates if the coefficient of a domain is statistically significant or not. 
% A \textit{p-value} lower than 0.01 means that ...
\textit{z-value} tells us how many standard deviation the average decision of a certain industry sector is away from the average decision of the whole data set~\cite{mcleod_z-score_2019}. It indicates the reliability of the coefficient computed by the logistic regression model.
% The larger the z-value is, the more distinct the behavior of domains with certain industry sector is, compared to the behavior of all domains. 
%Domains in a category with a higher \textit{z-value} are more concentrated on a specific decision, compared to those with a lower \textit{z-value.} 



We discuss the type of reactions observed of those domains that belong to any of the top 20 industry sectors whose coefficient was both highly reliable (greater than the median \textit{z-value} as shown in Fig.~\ref{fig:z_hist}) and statistically significant (\textit{p-value} $<0.05$).

% In Section~\ref{sec:domain_sector}, we show how domains in these selected industry sectors reacted after the incident.
% 
% \textcolor{red}{To add: cdf of p and z value, negative significant influence}
% 

% \begin{figure}[hbp]
%     \centering
%     \includegraphics[width=\linewidth]{figure/z_value.png}
%     \caption{Distribution of z-values (signifies reliability) for industry sector coefficients in the linear regression model. We discuss in more detail the reactions of domains that belong to industry sectors, which according to the logistic regression model had a reliable and statistically significant impact on the reactions.}
%     \label{fig:z_hist}
% \end{figure}
The results indicate that a number of categories have more significant correlation to the resilience strategy than the others.
Domains in industry sectors with higher coefficient have a higher probability to react following outages, such as \textit{General News} and \textit{Streaming Media}. 
DNS providers should anticipate the reaction from their customers in these industry sectors more than other sectors.
% We then particularly discuss a number of industry sectors with statistically significant positive influence on the decision to react to be discussed further.
% % \textcolor{red}{Our results show $>$20 sectors with coef$>$0 and p-value$<$0.01. We select only top 20 due to space limitation?}
% We retrieve sectors with significant p-values and choose the top 20 sectors with the highest z-values as shown in Table~\ref{tab:stat_result}.
% We limit our industry sector analysis to selected categories with statistically significant influence on the decision to react.
% 

\ 

\noindent
\textit{\textbf{Key takeaway:} By using a multivariate logistic regression model, we were able to calculate and reveal that for 34 out of 94 industry sectors, there is statistically significant influence on the post-attack reaction.}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} Using a multivariate logistic regression model, we calculate the impact of industry sectors on the reactions of domains to the attack. 34 out of 94 industry sectors (20 of which are shown in Table~\ref{tab:stat_result}), have some statistical influence on the post-attack reaction of the domains.}
   % \end{minipage}}

\ 

% \textcolor{red}{See my comment on teams.}
% \todo{see my comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/z_value.png}
    \caption{Distribution of z-values (signifies reliability) for industry sector coefficients in the linear regression model. We discuss in more detail the reactions of domains that belong to industry sectors, which according to the logistic regression model had a reliable and statistically significant impact on the reactions.}
    \label{fig:z_hist}
\end{figure}

We also observe a number of industry sectors which \textbf{do not} have statistically significant influence on the decision to react such as \textit{Religion}, \textit{Ideologies}, and \textit{Politics}.
Religion and Ideologies sectors include web pages that discuss spirituality and beliefs while Politics domains discuss about political parties, views, and opinions.
We might indicate that domains in these sectors do not require high resilience.

\ 

\noindent
\textit{\textbf{Key takeaway:} Some industry sectors do not seem to have a statistically significant influence on the decision to react after the attack.}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} Some industry sectors such as Religions and Politics do not seem to have a statistically significant influence on the decision to react after the attack. Hence, in these cases the likelihood of domains reacting is equal to random.} 
   % \end{minipage}}

\



% \subsection{Domain Behaviors by Industry Sectors}
%\label{sec:domain_sector}
%We define domain reaction as \textit{the first movement following the incident}. Moreover, we define returning movement as \textit{the first returning movement after it stopped using Dyn service} i.e., the status changed from not customer to customer, either as exclusive or non-exclusive.



We zoom into a number of significantly influential industry sectors (Table~\ref{tab:stat_result}).
Fig.~\ref{fig:reactions_by_category} shows how domains in these industry sectors reacted.
The \textit{top plot} shows proportions of reactive domains in each industry sector, characterized by their decision to become non-exclusive or to unsubscribe after the attack.
The diminishing line in the top plot indicates the size, i.e., number of domains, of each industry sector on a $log_{10}$ scale.
We observe that sector size do not indicate a direct correlation with the proportion of reactive domains in the sector.
However, we demonstrate that the reactions vary among industry sectors in two ways: proportion of the reactive domains and the dominant type of reactions.



% 1
From the \textit{top plot} in Fig.~\ref{fig:reactions_by_category}, we show that majority of domains in some industry sectors \textbf{became non-exclusive} following the incident, i.e., used additional DNS providers, such as domains in \textit{General News}, \textit{Potentially Unwanted Programs (PUPs)}, \textit{Malicious Sites}, and \textit{Visual Search Engine}.
Domains in \textit{PUPs} and \textit{Malicious Sites} categories are made with intention to infect user's computer with software or script to hijack or alter security and privacy, e.g., Trojan horses and viruses.
Domains in \textit{Visual Search Engine} include web pages that provide searching functionality with image-specific results.
The reaction to use multiple DNS services might indicate that these domains have a high -- most probably financial -- value for the owners, hence, it is important to keep them up at all times.
After the attack, they used back-up services to make their domains more resilient against future outages.
Therefore, we assume that the revenue from the domains is large enough to compensate the cost of using extra DNS service, if present.

% 2
Meanwhile, domains in some industry sectors show a significant preference to \textbf{unsubscribe}, i.e., stop using Dyn service, after the attack (Fig.~\ref{fig:reactions_by_category}).
% We group industry sectors with such preference into two groups.
Among them, we observe domains intended for adult audience
% 1
% First, domains with content for adult audience 
such as \textit{Gambling} sites, web pages about \textit{Weapons}, and sites showing \textit{Provocative Attires}, 
and domains intended for 
% 2
% Second, domains for 
more general audience such as \textit{Motor Vehicles} sites, \textit{Streaming Media}, and \textit{Social Networking} sites.
The reaction to unsubscribe after the attack might also indicate that domain owners value their domains and find it necessary to react after the attack.
However, we suspect that the cost of using a secondary DNS service is not worth the revenue from the domain or the owner considers Dyn no longer reliable.

\begin{figure}[]
    % \centering
    \includegraphics[width=\linewidth]{figure/plot_sector_v5_with_swarm.pdf}
    \caption{
        Behaviors of domains in selected industry sectors.
        \textbf{Top Plot} shows the proportions of domains with different reactions in each sector along with the sector sizes.
        \textbf{Middle Plot} shows the proportions of unsubscribed domains that did not return.
        % \textbf{Bottom Plot} shows the mean and variation of Alexa rank of domains in each sector.
        \textbf{Bottom Plot} shows the distribution of Alexa ranks among domains that belong to a certain industry sector.
    }
    \label{fig:reactions_by_category}
\end{figure}
\

\noindent
\textit{\textbf{Key takeaway:} We see a difference in the type of reaction based on the industry sector. In some sectors, domains for the most part became non-exclusive following the attack (e.g., \textit{General News}), while for others, customers largely unsubscribed (e.g., \textit{Gambling}).}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} We analyse the type of reactions observed for the domains in selected industry sectors (Fig.~\ref{fig:reactions_by_category}). We see a difference in the type of reaction based on the industry sector: In some sectors such as \textit{General News}, domains predominantly became non-exclusive following the attack, while some others such as \textit{Gambling} domains tend to unsubscribe.} 
   % \end{minipage}}
% [DELETE] This number reflects the relative importance of keeping the domain operational from the perspective of domain owners. 
% [DELETE] A higher proportion in certain type of decision might reflects the risk appetite of the domain owners, especially because each type of reaction has different risk level (Section~\ref{sec:key_concepts}). 

\ 

In the \textit{middle plot}, we show the proportion of return among domains that unsubscribed in each sector.
This metric is particularly important to measure business impact of an outage incident as it indicates how many customers that the provider loses for a longer term.
In some industry sectors such as \textit{Travel} (e.g., ticketing sites), \textit{Motor Vehicles}, and \textit{Personal Pages} (e.g., blogs), domains that \textbf{did not return} are significantly more than those which \textit{returned}.
On the contrary, the behavior is quite the opposite in \textit{Gambling}, \textit{PUPs}, and \textit{Malicious Sites} sectors, i.e., most of unsubscribed domains returned later.
In \textit{Visual Search Engine} sector, there is no domain that unsubscribed, hence, no data shown in the plot.
% This number might reflect the relative tolerance of domain owners against service failure by the provider.
% High proportion of domains which did not return might indicate low tolerance among the domain owners e.g., due to trust loss. 
% On the other hand, domains that returned might still consider Dyn as a trustworthy provider or already have a good relationship with Dyn.

\ 

\noindent
\textit{\textbf{Key takeaway:} In some industry sectors, domains that unsubscribed mostly did not return (e.g., \textit{Travel}), while in others, a higher proportion of domains unsubscribed and returned (e.g., \textit{Gambling}). This suggests that the industry sector affects decision-making.}

%\noindent \fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} In some industry sectors, such as Travel, most domains that unsubscribed after the attack did not return, while in some other sectors, such as \textit{Gambling}, a higher proportion of domains returned. This shows that for some sectors, the chance of customers leaving for a longer term is higher. Domains belonging to \textit{visual search engine} category only used becoming non-exclusive as a resilience strategy.} 
   % \end{minipage}}

\ 

% [Still working] 
The \textit{bottom plot} in Fig.~\ref{fig:reactions_by_category} shows the distribution of Alexa ranks -- where present -- among all domains in each industry sector characterized by their responses after the attack i.e., reactive or non-reactive. 
This plot provides insight into the influence of popularity on the choice of resilience strategy adopted by domains in each industry sector.
% 
%\textcolor{red}{There are a number of domain categories that are in Fig 4 but we never talk about in the text. Why?}
% The latter metric indicates how diverse the Alexa ranks are within that category.
% For example, most domains in \textit{Job Search} sector have higher Alexa ranks i.e., more popular, than domains in \textit{General News}, but more uniform i.e., have similar popularity.
%For example, in \textit{Job Search} and \textit{Gambling} categories, Alexa ranks of domains that reacted (dark box plot and light dots) are more concentrated in the lower plot (shorter box), indicating a higher popularity, compared to those which did not react (light box plot and dark dots) which are more dispersed (longer box) and, in majority, less popular.
For most industry sectors shown in Fig.~\ref{fig:reactions_by_category}, we observe that the average popularity of reactive domains is higher than the average popularity of non-reactive domains. This is consistent with our previous discussion in Section~\ref{sec:domain_popularity} that higher popularity influences the domain decision to react.
However, we see that popularity was a more significant factor for some industry sectors than the others. \textbf{Non-overlapping} boxes in \textit{Job Search} and \textit{Gambling} sectors indicate a strong correlation between popularity and the decision to react.
Meanwhile, in some industry sectors such as \textit{Internet Service}, domain popularity does not seem to have a strong correlation with the decisions to react, considering that the distributions of Alexa ranks are rather similar between reactive and non-reactive domains, indicated by \textbf{overlapping} boxes.
% Therefore, a \textit{high mean} of Alexa rank with \textit{low coefficient of variation} indicates that the domain popularity plays significant role in the decisions to react such as domains in \textit{Weapons}, \textit{Provocative Attires}, and \textit{For Kids}.

\ 

\noindent\textit{\textbf{Key takeaway:} In some industry sectors (e.g., Job Search), the influence of popularity on the decision to react is stronger than the others (e.g., Internet Service).}
%\noindent \fbox{%
    %\begin{minipage}{0.95\linewidth}
%    \textit{\textbf{Key takeaway:} The popularity of domains in some industry sectors with high and similar Alexa ranks such as Job Search might have a significant influence on the decisions to react after the attack.} 
%    \end{minipage}}
% 
% We make a couple of further observations regarding domains in the selected categories.  
% % Figure~\ref{fig:reactions_by_category}.
% % 1
% Domains in \textit{Potentially Unwanted Programs (PUPs)} and \textit{Malicious Sites} categories predominantly became non-exclusive following the incident, and none of unsubscribed ones that did not return.
% In addition, we could see that none of domains in these two categories belong to Top 1M Alexa list. This is predictable since malicious websites are rarely found in top Alexa list~\cite{kim_malicious_2018}.
% % domain examples
% Domains in these categories are made with intention to infect user's computer with software or script to hijack or alter security and privacy, e.g., Trojan horses and viruses.
% % 2
% % 3
% Domains for adult audience i.e., \textit{Gambling}, \textit{Weapons}, and \textit{Provocative Attire}, predominantly unsubscribed after the incident. 
% However, in \textit{Gambling} sector, only 20\% that did not return.
% In addition, Alexa rank mean and variation for the other two sectors indicate that domains in these sectors are homogeneously quite popular and suggest a strong influence on the reaction.
% % example
% Domains in Gambling sector include web pages that allow users to place bets online.
% Domains in Weapon sector include web pages that provide every information about weapons, including buying, for either personal or military use.
% Meanwhile, domains in Provocative Attire sector include web pages showing non-nudity revealing attires intended to provoke the viewers. 
% \newline \newline \textit{\textbf{Key takeaway:}} \newline
% 
% % 4
% Domains in \textit{General News} predominantly became non-exclusive but more than 82\% of unsubscribed ones did not return.
% Furthermore, this behavior is less likely to be influenced by domain popularity due to a high diversity in their Alexa rank.
% % domain example
% Domains that belong in this category include news portals, both regional and international.
% % 
% Domains in \textit{Professional Networking} and \textit{Social Networking} show a similar behavior.
% Most of them unsubscribed then did not return which might indicate low tolerance against violation in service fulfillment.
% % example
% Domains in this category include social networking for professional use and friendship focus. 
% % 5
% Lastly, domains in \textit{Visual Search Engine} sector only reacted by becoming non-exclusive, hence, no data about their return behavior.
% % example
% This category includes web pages that provide searching functionality with image-specific results.


% \begin{observation}
%     Majority of reactive domains in Sport sector unsubscribed from Dyn but majority of them returned.\textcolor[red]{Too anecdotal. Maybe for most observations it is better to talk in terms of how Industry sector as a factor explains the decision taken by domain owners.}
% \end{observation}

% Discussion here.

% \begin{observation}
%     In Marketing/Advertising, Online Shopping, and Entertainment sectors, there were more reactive domains that unsubscribed than those which stayed. More than 80\% of those which unsubscribed did not return.
% \end{observation}

% Discussion here.






% \textbf{Reactive or Not reactive:\ }

% \textbf{Become Non Exclusive or Unsubscribe:\ }
% There are two likely reactions that a domain owner could take following the outage incident: to become non-exclusive or to unsubscribe. We observe that the proportion of these two reactions varies among different types of domain. 
% For example, domains in Finance, e.g., banks and loans, mostly chose to leave Dyn while domains in Business e.g., trading companies, mostly chose to keep using Dyn but became non-exclusive i.e., use managed DNS service from other providers following the incident (Figure~\ref{fig:first_reaction_industry}). 
% % One possible explanation is that domains in Finance are easier to lose trust following the incident. 
% This behavior is consistent with the fact that finance-related domains are more trust sensitive.
% It is likely that they require highly reliable partners to support their operation and less tolerant with service failure.

% In contrast, the intended use of the domains did not correlate with its reaction, as shown in Figure~\ref{fig:reaction_by_purpose}. Most domains reacted by stop using the service regardless their intended uses.

% \todo[inline]{MJ: Does proportion mean ratio/fraction? Does it mean numbers? The table 2 caption mentioned the word proportions before, but table 2 only tabulates numbers. The numerical metrics speak of proportions and there it seems to be about fractions. Here you are not giving fractions, but you do seem to compare absolute numbers from two reactivity classes (nonex and noncust). Please be consistent/avoid ambiguity.}

% 
% \begin{figure}%[ht]
%      \centering
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/first_reaction_by_purpose2.png}
%          \caption{ }
%          \label{fig:reaction_by_purpose}
%      \end{subfigure}
%      \hspace{1em}
%     %  \hfill
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/windowed_departing_domains_by_purpose.png}
%          \caption{ }
%          \label{fig:returning_by_purpose}
%      \end{subfigure}
%         \caption{Reaction (a) and return movement (b) by intended use }
%         \label{fig:by_purpose}
% \end{figure}

%\subsubsection{React Immediately or Later.}
% \textbf{React Immediately or Later:\ }
% Another aspect that reflects the importance of DNS service availability for businesses is immediacy of the reaction. 
% % As discussed in Section~\ref{sec:mdns_business}, DNS service could be a key service in certain digital businesses, especially those who rely on Internet-based systems. Each second of downtime could cost them millions of dollar. For these type of businesses, they need to react immediately to return the availability of their systems. On the other hand, other businesses could react later because every second of downtime does not cost them much. 
% From the data, we observed that most domains in Finance reacted later than most domains in Business and News Portal. 
% Figure~\ref{fig:finance_late_response} shows that most domains in the financial sector reacted after the end of the month, while domains in more general categories mostly reacted immediately i.e., the next day following the incident. Despite the late reaction, almost all domains in the financial sector reacted by leaving Dyn. Meanwhile, we observe that domains in News category which left Dyn reacted immediately, but those which became non-exclusive reacted later in similar number. Hence, we may conclude that most domains in Finance sector might not suffer a great loss for each second of DNS unavailability but still lost their trust with the provider. Another possible explanation regarding this behavior is because the contract ended at the end of the month. Therefore, it is more efficient to wait until the previous contract ends before starting to use and pay for another service.

% Based on intended uses, similar proportions of domains that mainly provide service reacted on two specific days: day +1 and day +12. Further analysis is required to discover what type of services these domains provide to explain the difference. Domains that provide information and network reacted similarly i.e., immediately left after the incident, as shown in Figure~\ref{fig:reaction_time_by_purpose}.

%\subsubsection{Return or Leave for Good.}
% \textbf{Return or Not:\ }
% The third aspect that we analysed is the return movement among domains in different industry sectors. 
% % Previously, we have discussed that most domains in Finance chose to left Dyn, despite their late response.  
% We found out that most domains in Finance not only leave Dyn but almost all of them left for good. 
% Compared to other industry sectors, the proportion of Finance domains that left for good is much higher (Figure~\ref{fig:departing_by_industry}). 
% This fact supports our belief that domains in Finance are less tolerant of service failure thus prefer to leave and switch to other service providers. Based on intended use, we found no obvious difference in the proportion of domains that returned after they left, as shown in Figure~\ref{fig:returning_by_purpose}.  

% \begin{figure}[p]
%     \centering
%     \begin{subfigure}[b]{0.85\textwidth}%[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_time_to_react_finance.png}
%     \caption{\textbf{Time to react by industry sector.} Despite the tendency to leave instead of becoming non-exclusive, most domains in Finance (top) left Dyn after end of the month (a), while most domains in Business (middle) and News, Portal, and Search categories (bottom) left Dyn immediately i.e., the next day after the attack (b and c).}
%     \label{fig:finance_late_response}
% \end{subfigure}
% % 
% \begin{subfigure}[b]{0.85\textwidth}%[H]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_time_to_react_by_purpose.png}
%     \caption{\textbf{Time to react by intended use.} Most domains that provide service reacted by leaving Dyn. Many domains in this category left after end of the month (a), while in the other two categories, only a few left later.}
%     \label{fig:reaction_time_by_purpose}
% \end{subfigure}
% % 
% \begin{subfigure}[b]{0.85\textwidth}%[H]
%     \centering
%     \includegraphics[width=\linewidth]{figure/windowed_departing_domains_by_industry.png}
%     \caption{\textbf{Behavior of leaving domains by industry sector}. Majority of leaving domains in the Finance category did not return.}
%     \label{fig:departing_by_industry}
% \end{subfigure}
% \caption{Behaviour of domains for selected industry sectors.}
% \label{fig: behaviour of domains}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=.5\textwidth]{figure/plot3_behavior_by_functional_type.png}
%     \caption{Domain behaviors by different reactions across functional types.}
%     \label{fig:reactions_by_functional}
% \end{figure}

% \begin{observation}
%     Among reactive domains with Information/Communication function, there were more domains that stayed (4.2\%) than those which unsubscribed (2.2\%). Nevertheless, 81.8\% of those which left did not return.
% \end{observation}

% Information/Communication e.g. general news, search engine, and online forum.

\subsection{Risk Level Influence on Decision to React}
\label{sec:domain_risk_level}

%\textcolor{red}{Number of unverified, medium and high risk level websites are very low. Do comment on the aggregate numbers of these websites. How many are these?}

% Explain briefly about methodology to determine risk level.
% \textcolor{red}{
%     Discuss:
%     \begin{itemize}
%         \item DONE Only a few domains in unverified, medium, and high risk $\xrightarrow{}$ most Dyn consumers are legitimate domains
%         \item DONE Discuss med and hi risk domains, why use Dyn? why use redundancy? why return? $\xrightarrow{}$ premium crimes which needs hi availability.
%         \item DONE Discuss med hi risk domains with domains in PUPs and Malicious. compare behavior $\xrightarrow{}$ what it means?
%         \item In risk group, compare domains in security risk with domains in med and hi risks
%     \end{itemize}
% }

% Join two plots together using shared y axis!
We then analyze how risk level of the domains influence their reaction following the attack.
Fig.~\ref{fig:reaction_by_risk_type} shows behavior of domains with different risk profile, characterized by risk level and risk group.
Recall that McAfee categorizes domains based on the reputation score into four risk levels as shown in Section~\ref{sec:methodology}.
% \textit{Risk Level} is individually measured for each domain based on its reputation score~\footnote{See \url{https://trustedsource.org/download/ts_wd_reference_guide.pdf}}. 
% \textit{Unverified} refers to the level of risk which lies between minimal and medium risk.
We show that domains in Minimal Risk significantly outnumber domains in other risk levels. Out of 106K domains of Dyn customers, 104K are in Minimal Risk while domains in Unverified, Medium Risk, and High Risk categories only account for 2K domains (Fig.~\ref{fig:reaction_by_risk_type}).
% \textcolor{red}{add the exact number DONE}
This indicates that majority of Dyn customer domains were relatively safe to visit.

\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{figure/plot_risk_combined3.3_with_swarm.pdf}
    \caption{
    Behaviors of domains with different \textit{Risk Levels} and \textit{Risk Groups}. 
    \textbf{Top Plot} shows the proportions of domains with different reactions in each group along with the group sizes. 
    \textbf{Middle Plot} shows the proportions of unsubscribed domains that did not return. 
    \textbf{Bottom Plot} shows the distribution of Alexa ranks among domains that belong to a certain group.
    % Domain behaviors by different reactions across different \textit{Risk Levels} and \textit{Risk Groups}.
    % \textcolor{red}{Risk Type -- Risk Group}
    }
    \label{fig:reaction_by_risk_type}
\end{figure}

Some domains with higher risk levels also need high availability, hence, using the managed DNS service from Dyn.
As illustrated by the \textit{top plot} in Fig.~\ref{fig:reaction_by_risk_type}, some Dyn customers are domains in \textit{medium} and \textit{high risk} levels and they show a similar preference, namely, to become non-exclusive after the attack, i.e., use redundant DNS services.
Moreover, majority of the domains with medium and high risks returned if they unsubscribed, (the \textit{middle plot}).
% This observation reflects the resilience strategy of some malicious domains -- most probably with high revenue -- which demand higher availability from premium and redundant DNS services.
We also observed this \textit{exact} behavior among domains intended to victimize the users, e.g., PUPs and Malicious Sites, as discussed in Section~\ref{sec:stat_analysis}.
% 
% We make a couple of observations with regards to Risk Level influence on the domains reactions.
% 1
% Domains with \textit{medium} and \textit{high risk} level show a similar behavior, namely, they predominantly became non-exclusive. Furthermore, none of those which unsubscribed did not return. 

% 2
With regards to domain popularity, we indicate no domain with high risk belonged to Alexa Top 1M list as the \textit{bottom plot} in Fig.~\ref{fig:reaction_by_risk_type} shows.
This observation is again consistent with our result in Section~\ref{sec:stat_analysis} about malicious domains.
We demonstrate that some domains with medium risk are relatively quite popular (concentrated in the lower area) reflecting that some visitors unknowingly risk their security by regularly accessing the domains.

\

\noindent
\textit{\textbf{Key takeaway:} Customers with higher risk levels mostly became non-exclusive after the attack and the majority of those who unsubscribed instead also later returned.} 
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth}
  %  \textit{\textbf{Key takeaway:} Domains with higher risk levels mostly became non-exclusive after the attack and majority of those who unsubscribed returned later.} 
   % \end{minipage}}

\ 

% Moreover, there is another conclusion we could infer about domains with minimal risk from Figure~\ref{fig:reaction_by_risk_type}.
% 3
%\textcolor{red}{The word "active" needs to be removed everywhere.}
In addition, considering the \textit{top} and \textit{middle plots} in Fig.~\ref{fig:reaction_by_risk_type}, we observe that majority of the domains with minimal risk stopped using Dyn service permanently following the attack, namely, nearly 1K domains or 71.4\% of those which unsubscribed did not return.
This number indicates a relatively major business impact (i.e., losing nearly 1K customers) that Dyn suffered following the outage.
Other DNS providers could use this proportion to help estimate customer loss following an outage.
%\newline \newline \textit{\textbf{Key takeaway:} Legitimate domains have a relatively high tendency not to return once they unsubscribe from the DNS service after an outage.}

\ 

\noindent
\textit{\textbf{Key takeaway:} Our results show that if domains in the minimal risk category unsubscribe, the probability that they stay away for a longer time is higher.}
%\noindent\fbox{%
 %   \begin{minipage}{0.95\linewidth} \textit{\textbf{Key takeaway:} There is a greater probability for domains in the minimal risk category to stop using Dyn for a longer term if they unsubscribe.}
  %  \end{minipage}}
    
\subsection{
% [Still working] 
Risk Group Influence on Decision to React}
\label{sec:domain_risk_type}

%\textcolor{red}{Structure suggestion:Recall definition of a category and discuss the types of websites that will fall in the category. Discuss how different is the reaction to other risk groups (See top plot). Discuss return behaviour (second plot). Do only popular websites move; or do all websites have similar likelihood of moving? Repeat for the next category. Note that in the documentation, it is "risk group" not "risk type".[DONE]}

% Category labels from the URL categorization service indicates the functionalities of the domains based on their content (if present).
% When used improperly, domains with certain functionalities might lead to unintended situations and negatively impact businesses or individuals.
% McAfee classifies URL categories into \textit{Risk Groups} based on which main aspect is the most at risk when this unintended situation happens.
% According to the documentation,
% \textit{Risk Group} refers to the main aspect which domains in certain category i.e., industry sector, might risk.
% For example, domains with \textit{Productivity} risk are non-business related which might reduce one's productivity at work e.g., social media and entertainment portal.
% Another example, domains with \textit{Bandwidth} risk are mainly web pages whose contents require a large amount of bandwidth to retrieve e.g., video streaming portal, hence, might disrupt business related communication over the network. 

We make a couple of observations from Fig.~\ref{fig:reaction_by_risk_type} regarding reactions among domains in different Risk Groups.
% 4
According to the \textit{top plot}, domains with \textit{Liability}, \textit{Communications}, and \textit{Propriety} risks show preferences to unsubscribe after the attack.
% 3
Meanwhile, as shown in the \textit{middle plot}, we observe similar return behaviors of domains in different risk groups, namely, more than half of them did not return after they unsubscribed, except domains in \textit{Security} risk group.

% 5
% Regarding domain popularity illustrated by the \textit{bottom plot}, even though the mean Alexa rank of each risk group is similarly high, but popularity of domains in \textit{Productivity, Information,} and \textit{Liability} risk groups are more uniform.
% This implies that popularity of domains in these 3 risk groups might have a significant influence on the reactions after the attack.
We could observe in the \textit{bottom plot} of Fig.~\ref{fig:reaction_by_risk_type} that Alexa ranks of reactive domains are more concentrated in the lower area, i.e., more popular, in every risk group. 
This result is consistent with our observation in Section~\ref{sec:domain_popularity} that higher popularity shows a correlation with the decision to react after the attack.
However, there is a higher spread in the popularity of reactive domains in \textit{Productivity} and \textit{Information} risk groups, which indicates a weaker correlation of the domain popularity with the decision to react.

%\textcolor{red}{The domains popularity in some risk groups such as Productivity might have a strong influence, why? What about information and liability?}
% 

\

\noindent\textit{\textbf{Key takeaway:} Domains in some risk groups (e.g., Liability) mostly unsubscribed after the attack.}
% \noindent\fbox{%
%     \begin{minipage}{0.95\linewidth}
%     \textit{\textbf{Key takeaway:} Domains in some risk groups such as \textit{Liability} (recall: may serve pirated material) mostly unsubscribed after the attack. 
%     \textcolor{red}{
%     The domains popularity in some risk groups such as Productivity might have a strong influence on the domain reactions after the attack. Popularity of websites have a lower impact on post-attack reactions for the domains that consume greater \textit{Bandwidth} or can be used for \textit{Communication}.}
%     }
%     \end{minipage}}

% Lower variation in these risk types indicate that the domains are relatively more homogeneous in terms of popularity, i.e., similarly quite popular (Figure~\ref{fig:reaction_by_risk_type}).

% \begin{figure}[t]
%      \centering
%      \begin{subfig}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/plot_risk_level_v2.pdf}
%         \caption{By risk level}
%         \label{fig:by_risk_level}
%      \end{subfig}
%      \hfill
%      \begin{subfig}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/plot_risk_type_v2.pdf}
%         \caption{By risk type}
%         \label{fig:by_risk_type}
%      \end{subfig}
%         \caption{Behavior by risk profile.}
%         \label{fig:by_risk_profile}
% \end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=.25\textwidth]{figure/plot_risk_level_v2.pdf}
%    \caption{Domain behaviors by different reactions across risk levels [make subfigure]}
%    \label{fig:reaction_by_risk_level}
%\end{figure}

\subsection{Analysis on Domain Autonomous Systems}
\label{sec:domain_as}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/AS-and-Rank-histogram.pdf}
    \caption{Histogram showing the variability in decisions within each AS and the average size (number of IPs) of ASes.}
    \label{fig:AS_Size_Histogram}
\end{figure}

A single party can operate multiple domains. For example, Alphabet Inc. operates, among others, google.com and gmail.com. So far we have not considered the potential effects of a single party making decisions (i.e., driving domain reactions) for multiple domains. 
As a first step towards exploring if multiple reactions are correlated to a single party, we measure the variety of reactions of Dyn customers within each Autonomous System (AS).

We associate domains to their hosting network at the time of the Dyn attack by mapping IP addresses (i.e., \texttt{A} records) to AS numbers, using IP-prefix-to-AS data set from CAIDA~\cite{the_caida_ucsd_routeviews_2008}. 
% We then calculate the number of IP addresses per AS that are used to host domains that react and compare it with the total number of IP addresses in each AS used to host Dyn customers. 
We then compare the proportion of IP addresses that reacted in each AS, i.e., number of IP addresses associated with reactive domains to all IP addresses in each AS.
Fig.~\ref{fig:AS_Size_Histogram} shows the resulting distribution.
We observe that in the case of about 200 smaller ASes (one to a few domains hosted), the domains all show the same behaviour. This suggests that parties that operate several domains drive the reaction for multiple domains, but on the order of a few hundred domains in total based on this initial view. This approach of course does not account for cases where a single party hosts their domains in multiple networks, which we leave for future work.

%In some cases, multiple domains can be operated by a single party. For example, an enterprise such as Alphabet Inc. can operate multiple domains such as google.com and gmail.com.\ Currently, we do not view the impact that the concentration of domains among the parties that operate them has on our results. However, to further explore if there are multiple parties responsible for the reactions we observe, we measure the variety of reactions observed within each AS. 
% \textcolor{red}{
%To do so, we extract the type of hosting that a domain was using during the incident by mapping IP address from domain's \texttt{A} record to its corresponding Autonomous System (AS) using IP prefix to AS dataset~\cite{the_caida_ucsd_routeviews_2008}
% } 
%Using this data we calculate the percentage of IPs that react out of the total number of IPs related to the domains using Dyn name servers. Fig.~\ref{fig:AS_Size_Histogram} shows the distribution for the percentage of \texttt{IP} addresses within each AS that react. We observe that in the case of only the smaller ASes, all domains show the same behaviour. For, larger ASes, we see only a small fraction of domains showing reactions. This shows that the resilience strategy chosen by domains within each AS was not the same, except when these ASes were relatively small.






%\textcolor{red}{A subsection on what kind of diversity in decisions do we notice per AS would be nice to argue that not all IPs in an AS reacted the same way.}


% \subsection{Hypothesis Testing}

% To test whether the differences in behavior across industry sectors and intended use are statistically significant, we did a statistical test. We compared the daily number of domains from two categories as two related-pair samples. Because most data are not normally distributed according to the Shapiro-Wilk test \cite{shapiro_analysis_1965}, we could not do a simple paired t-test. Instead, we did the Wilcoxon signed-rank test \cite{wilcoxon_individual_1945} for all possible pairs of industry sectors and intended uses. We repeated the test for three daily variables: number of domains that become non-exclusive, left, and returned. 
% The test shows variation in results between categories: some pairs are significantly different and some others are not. 
% A complete result of this test is presented in Table~\ref{tab:ttest_by_industry1}, Table~\ref{fig:returning_ttest_by_industry}, and Table~\ref{tab:ttest_by_purpose} in Appendix, alongside the complete metrics calculation in Table~\ref{tab:metrics_by_industry} and Table~\ref{tab:metric_by_purpose}.
% 
\section{Implications of results for Stakeholders}
\label{sec: Implications}
%We present possible implications of the results for different stakeholders, especially in managed DNS business.
% 
%\subsubsection{For Managed DNS Service Providers}
%\textcolor{red}{This should be a separate section and part of Discussion. Implications are very generic, we need examples from results for making them stronger.}

We evaluate the impact of factors such as domain popularity, industry sectors, domain risk level and risk group on decision of domain managers in reaction to unavailability of Dyn services. We believe that our results can be insightful for both providers and users of network services. In this section, we discuss the implications of these results for four a number of stakeholders:

\noindent \textbf{Managed DNS Service Providers:}
The results of this work are most useful for managed DNS service providers, especially to develop resilient strategy related with their customer portfolios. 
\begin{itemize}
    \item 
        DNS providers could use this work to estimate the proportion of their existing customers which are more likely to stop using the service in case of an outage incident. 
        For example, they can start profiling their existing customers using URL categorization service and Alexa rank to indicate which of them have characteristics (e.g., industry sector and popularity) that suggest a higher probability to leave in case of an outage.
    \item
        Using data of their existing revenue, DNS providers can quantify financially the potential business impact of an unforeseen outage by calculating the potential revenue loss coming from the number of customers with higher probability to leave in case of an outage.
    \item 
        DNS providers could use this estimation of potential business impact to justify their strategy in outage prevention e.g., infrastructure redundancy, or to minimize the loss, e.g., use cyber insurance. 
    \item
        Moreover, using this method, DNS providers should consider to monitor their customer portfolio in order to minimize the proportion of customers with characteristics (e.g., domain popularity and industry sector) that reflect a high probability to react or leave in case of an outage to minimize the business impact.
    \item
        Further, DNS providers could base their marketing strategy on the results of this work, for example, to offer more premium DNS services, e.g., with more redundant PoP servers, to customers that are more probably to react since it indicates that the customers adopt a more resilient strategy.
        
\end{itemize}
% They could develop a formula to measure their current risk score based on the number and the industry sectors of their current customers. 
% \textit{Second}, 
% \textit{Third}, they 
% 
%\subsubsection{For Digital Businesses}

\noindent \textbf{Digital Businesses:\ }
\textcolor{red}{}
The results could be beneficial for businesses in terms of managing their risk of downtime.
\begin{itemize}
    \item 
        They could adjust their investment to prevent or to deal with downtime, e.g., insurance, SLA, or use of backup provider, by estimating the relative cost of downtime based on their characteristics.
    \item
        They could adjust their contingency plan in case of downtime, e.g., what reaction they could take based on most domains in similar sectors. However, it needs further study to evaluate the quality or the impact of different decisions taken by the Dyn customers, i.e., whether their reactions were appropriate.
\end{itemize}


%\subsubsection{}
\noindent \textbf{Cyber Insurance:\ }
The results can assist in cyber risk calculation for insurance purpose. 
\begin{itemize}
    \item 
        Insurers can use these results to find the optimum price and compensation, according to business characteristics of their (potential) customers and estimated business impact of downtime.
        For example, cyber insurers could estimate a higher business impact of downtime on customers with characteristics that suggest a higher likelihood to react.
    \item
        With this estimation, cyber insurers can adjust their strategy to offer more competitive pricing and compensation scheme, e.g., higher premiums for customers with high likelihood to react.
\end{itemize}

%\textcolor{red}{Example! DONE}

%\subsubsection{}
\noindent \textbf{Academic Researchers:\ }
The methodology and results presented in this paper have shown a novel direction for Internet measurement research to explore the Internet ecosystem resilience properties and dynamics. Rapid growth of digital business and use of Internet as business enabler requires more attention from the academic measurement community. 
\begin{itemize}
    \item 
        Our methodology provides business context on large-scale Internet network measurements. This approach can initiate ground breaking insights for academic research in both business and technical fields, such as digital business ecosystem, cyber risk, and centralization topic.
    \item
        Our methodology translates observations from measurement data into business insight which might accelerate strategic decision making related with digital resilience such as cyber security investment.
    \item
        The results from this work could help researchers analyze industry sectors regarding their concern about DNS service availability, and behavior against downtime in general, based on our statistical model.
        
\end{itemize}
